Hybrid Spiking Neural Networks for Low-Power Intra-Cortical Brain-Machine Interfaces

Intra-cortical brain-machine interfaces (iBMIs) have the potential to dramatically improve the lives of people with paraplegia by restoring their ability to perform daily activities. However, current iBMIs suffer from scalability and mobility limitations due to bulky hardware and wiring. Wireless iBMIs offer a solution but are constrained by a limited data rate. To overcome this challenge, we are investigating hybrid spiking neural networks for embedded neural decoding in wireless iBMIs. The networks consist of a temporal convolution-based compression followed by recurrent processing and a final interpolation back to the original sequence length. As recurrent units, we explore gated recurrent units (GRUs), leaky integrate-and-fire (LIF) neurons, and a combination of both - spiking GRUs (sGRUs) and analyze their differences in terms of accuracy, footprint, and activation sparsity. To that end, we train decoders on the "Nonhuman Primate Reaching with Multichannel Sensorimotor Cortex Electrophysiology" dataset and evaluate it using the NeuroBench framework, targeting both tracks of the IEEE BioCAS Grand Challenge on Neural Decoding. Our approach achieves high accuracy in predicting velocities of primate reaching movements from multichannel primary motor cortex recordings while maintaining a low number of synaptic operations, surpassing the current baseline models in the NeuroBench framework. This work highlights the potential of hybrid neural networks to facilitate wireless iBMIs with high decoding precision and a substantial increase in the number of monitored neurons, paving the way toward more advanced neuroprosthetic technologies.

==> chapters/entropicloss.tex <==
\section{Entropic Loss}

==> chapters/limitations.tex <==
\section{Limitations}

==> chapters/theory.tex <==
\section{Theoretical background}


==> data/gru_sample100.tex <==
-0.0412202906 0.0211917582
-0.0422213990 0.0197628467
-0.0432225074 0.0183339340
-0.0442236159 0.0169050214
-0.0452247243 0.0154761087
-0.0462258327 0.0140471960
-0.0472269411 0.0126182833
-0.0482280496 0.0111893707
-0.0480289652 0.0094587437
-0.0478298765 0.0077281167
-0.0476307877 0.0059974898
-0.0474316990 0.0042668631
-0.0472326102 0.0025362364
-0.0470335215 0.0008056098
-0.0468344327 -0.0009250169
-0.0466353439 -0.0026556436
-0.0450284303 -0.0039904073
-0.0434215167 -0.0053251713
-0.0418146031 -0.0066599352
-0.0402076895 -0.0079946992
-0.0386007759 -0.0093294632
-0.0369938622 -0.0106642266
-0.0353869486 -0.0119989900
-0.0337800350 -0.0133337534
-0.0341714970 -0.0145742830
-0.0345629591 -0.0158148126
-0.0349544211 -0.0170553422
-0.0353458831 -0.0182958717
-0.0357373452 -0.0195364002
-0.0361288072 -0.0207769298
-0.0365202693 -0.0220174593
-0.0369117313 -0.0232579889
-0.0381738026 -0.0237943501
-0.0394358740 -0.0243307112
-0.0406979453 -0.0248670724
-0.0419600167 -0.0254034335
-0.0432220880 -0.0259397947
-0.0444841593 -0.0264761559
-0.0457462307 -0.0270125170
-0.0470083020 -0.0275488782
-0.0477711371 -0.0275350159
-0.0485339721 -0.0275211535
-0.0492968072 -0.0275072912
-0.0500596422 -0.0274934289
-0.0508224773 -0.0274795665
-0.0515853123 -0.0274657042
-0.0523481474 -0.0274518419
-0.0531109825 -0.0274379796
-0.0521895546 -0.0263339508
-0.0512681267 -0.0252299221
-0.0503466988 -0.0241258934
-0.0494252709 -0.0230218647
-0.0485038430 -0.0219178360
-0.0475824151 -0.0208138073
-0.0466609872 -0.0197097785
-0.0457395594 -0.0186057498
-0.0434335701 -0.0176466000
-0.0411275809 -0.0166874503
-0.0388215917 -0.0157283005
-0.0365156046 -0.0147691507
-0.0342096176 -0.0138100009
-0.0319036306 -0.0128508511
-0.0295976436 -0.0118917013
-0.0272916565 -0.0109325515
-0.0254434827 -0.0103301650
-0.0235953088 -0.0097277785
-0.0217471350 -0.0091253925
-0.0198989611 -0.0085230065
-0.0180507873 -0.0079206206
-0.0162026135 -0.0073182346
-0.0143544396 -0.0067158486
-0.0125062658 -0.0061134627
-0.0119899262 -0.0057542296
-0.0114735867 -0.0053949966
-0.0109572471 -0.0050357636
-0.0104409076 -0.0046765305
-0.0099245681 -0.0043172975
-0.0094082285 -0.0039580645
-0.0088918890 -0.0035988315
-0.0083755494 -0.0032395984
-0.0079653820 -0.0032608388
-0.0075552145 -0.0032820792
-0.0071450471 -0.0033033195
-0.0067348796 -0.0033245599
-0.0063247122 -0.0033458003
-0.0059145448 -0.0033670406
-0.0055043773 -0.0033882810
-0.0050942099 -0.0034095214
-0.0048191024 -0.0033335114
-0.0045439949 -0.0032575015
-0.0042688875 -0.0031814916
-0.0039937800 -0.0031054816
-0.0037186726 -0.0030294717
-0.0034435651 -0.0029534618
-0.0031684577 -0.0028774519
-0.0028933502 -0.0028014419
-0.0030384276 -0.0023749825
-0.0031835051 -0.0019485230
-0.0033285825 -0.0015220635
-0.0034736600 -0.0010956041
-0.0036187375 -0.0006691447
-0.0037638149 -0.0002426852
-0.0039088924 0.0001837742
-0.0040539698 0.0006102336
-0.0043083006 0.0008964625
-0.0045626314 0.0011826914
-0.0048169622 0.0014689203
-0.0050712929 0.0017551491
-0.0053256237 0.0020413780
-0.0055799545 0.0023276068
-0.0058342853 0.0026138356
-0.0060886161 0.0029000645
-0.0065535675 0.0031043148
-0.0070185189 0.0033085651
-0.0074834703 0.0035128153
-0.0079484217 0.0037170656
-0.0084133731 0.0039213159
-0.0088783245 0.0041255662
-0.0093432759 0.0043298165
-0.0098082273 0.0045340668
-0.0101442193 0.0047099104
-0.0104802114 0.0048857540
-0.0108162035 0.0050615976
-0.0111521956 0.0052374413
-0.0114881876 0.0054132849
-0.0118241797 0.0055891285
-0.0121601718 0.0057649721
-0.0124961639 0.0059408157
-0.0123346482 0.0058980807
-0.0121731325 0.0058553457
-0.0120116168 0.0058126106
-0.0118501012 0.0057698756
-0.0116885855 0.0057271405
-0.0115270698 0.0056844055
-0.0113655541 0.0056416705
-0.0112040385 0.0055989354
-0.0108518979 0.0055664624
-0.0104997574 0.0055339893
-0.0101476168 0.0055015163
-0.0097954763 0.0054690432
-0.0094433357 0.0054365701
-0.0090911946 0.0054040971
-0.0087390535 0.0053716240
-0.0083869124 0.0053391510
-0.0084842211 0.0054301166
-0.0085815297 0.0055210822
-0.0086788384 0.0056120478
-0.0087761470 0.0057030134
-0.0088734556 0.0057939790
-0.0089707643 0.0058849446
-0.0090680729 0.0059759103
-0.0091653816 0.0060668759
-0.0093742991 0.0060497848
-0.0095832160 0.0060326937
-0.0097921329 0.0060156026
-0.0100010498 0.0059985115
-0.0102099667 0.0059814205
-0.0104188836 0.0059643294
-0.0106278006 0.0059472383
-0.0108367175 0.0059301472
-0.0108811650 0.0058444572
-0.0109256125 0.0057587672
-0.0109700600 0.0056730772
-0.0110145075 0.0055873872
-0.0110589549 0.0055016973
-0.0111034024 0.0054160073
-0.0111478499 0.0053303173
-0.0111922974 0.0052446273
-0.0112323309 0.0050777324
-0.0112723643 0.0049108375
-0.0113123977 0.0047439426
-0.0113524312 0.0045770477
-0.0113924646 0.0044101528
-0.0114324980 0.0042432579
-0.0114725315 0.0040763629
-0.0115125649 0.0039094680
-0.0115388230 0.0038399932
-0.0115650811 0.0037705183
-0.0115913392 0.0037010434
-0.0116175973 0.0036315685
-0.0116438554 0.0035620936
-0.0116701135 0.0034926187
-0.0116963716 0.0034231438
-0.0117226297 0.0033536689
-0.0117126007 0.0032826361
-0.0117025716 0.0032116032
-0.0116925426 0.0031405703
-0.0116825135 0.0030695374
-0.0116724845 0.0029985046
-0.0116624554 0.0029274717
-0.0116524264 0.0028564388
-0.0116423973 0.0027854059
-0.0115278513 0.0027076962
-0.0114133064 0.0026299865
-0.0112987615 0.0025522767
-0.0111842166 0.0024745670
-0.0110696717 0.0023968573
-0.0109551268 0.0023191475
-0.0108405818 0.0022414378
-0.0107260369 0.0021637281
-0.0106127691 0.0021434505
-0.0104995013 0.0021231730
-0.0103862335 0.0021028954
-0.0102729656 0.0020826179
-0.0101596978 0.0020623403
-0.0100464300 0.0020420628
-0.0099331622 0.0020217852
-0.0098198944 0.0020015077
-0.0094771802 0.0022189593
-0.0091344660 0.0024364109
-0.0087917519 0.0026538627
-0.0084490377 0.0028713141
-0.0081063235 0.0030887656
-0.0077636094 0.0033062171
-0.0074208952 0.0035236686
-0.0070781810 0.0037411200
-0.0073335433 0.0040361721
-0.0075889056 0.0043312242
-0.0078442679 0.0046262763
-0.0080996301 0.0049213284
-0.0083549924 0.0052163805
-0.0086103547 0.0055114326
-0.0088657170 0.0058064847
-0.0091210792 0.0061015368
-0.0098541163 0.0067149538
-0.0105871534 0.0073283709
-0.0113201905 0.0079417880
-0.0120532276 0.0085552051
-0.0127862647 0.0091686221
-0.0135193018 0.0097820387
-0.0142523388 0.0103954557
-0.0149853759 0.0110088728
-0.0145747443 0.0113153575
-0.0141641128 0.0116218422
-0.0137534812 0.0119283269
-0.0133428496 0.0122348115
-0.0129322180 0.0125412962
-0.0125215864 0.0128477809
-0.0121109548 0.0131542656
-0.0117003232 0.0134607503
-0.0130076953 0.0148725076
-0.0143150673 0.0162842649
-0.0156224394 0.0176960222
-0.0169298115 0.0191077783
-0.0182371835 0.0205195345
-0.0195445556 0.0219312907
-0.0208519288 0.0233430469
-0.0221593020 0.0247548031
-0.0239777463 0.0268648070
-0.0257961906 0.0289748108
-0.0276146349 0.0310848147
-0.0294330792 0.0331948186
-0.0312515235 0.0353048225
-0.0330699678 0.0374148264
-0.0348884121 0.0395248303
-0.0367068565 0.0416348320
-0.0416475994 0.0451253420
-0.0465883445 0.0486158521
-0.0515290896 0.0521063622
-0.0564698347 0.0555968722
-0.0614105798 0.0590873823
-0.0663513249 0.0625778923
-0.0712920701 0.0660684024
-0.0762328108 0.0695589125
-0.0823877050 0.0735480333
-0.0885425992 0.0775371542
-0.0946974934 0.0815262750
-0.1008523877 0.0855153959
-0.1070072819 0.0895045167
-0.1131621761 0.0934936376
-0.1193170703 0.0974827584
-0.1254719645 0.1014718793
-0.1299500486 0.1047746772
-0.1344281327 0.1080774752
-0.1389062168 0.1113802732
-0.1433843009 0.1146830712
-0.1478623850 0.1179858692
-0.1523404690 0.1212886671
-0.1568185443 0.1245914651
-0.1612966195 0.1278942631
-0.1633257248 0.1329155658
-0.1653548300 0.1379368686
-0.1673839352 0.1429581713
-0.1694130404 0.1479794740
-0.1714421456 0.1530007768
-0.1734712509 0.1580220705
-0.1755003561 0.1630433642
-0.1775294613 0.1680646579
-0.1745383440 0.1701779029
-0.1715472266 0.1722911480
-0.1685561093 0.1744043930
-0.1655649920 0.1765176381
-0.1625738746 0.1786308832
-0.1595827573 0.1807441282
-0.1565916400 0.1828573733
-0.1536005226 0.1849706183
-0.1483016323 0.1844933356
-0.1430027332 0.1840160529
-0.1377038341 0.1835387701
-0.1324049350 0.1830614874
-0.1271060359 0.1825842046
-0.1218071367 0.1821069219
-0.1165082376 0.1816296392
-0.1112093385 0.1811523564
-0.1061640378 0.1805345107
-0.1011187371 0.1799166649
-0.0960734364 0.1792988192
-0.0910281357 0.1786809734
-0.0859828349 0.1780631276
-0.0809375342 0.1774452819
-0.0758922335 0.1768274361
-0.0708469328 0.1762095904
-0.0690901728 0.1785211033
-0.0673334128 0.1808326162
-0.0655766528 0.1831441291
-0.0638198928 0.1854556420
-0.0620631328 0.1877671548
-0.0603063728 0.1900786677
-0.0585496128 0.1923901806
-0.0567928528 0.1947016935
-0.0576555457 0.2006735109
-0.0585182386 0.2066453282
-0.0593809315 0.2126171455
-0.0602436245 0.2185889628
-0.0611063174 0.2245607801
-0.0619690103 0.2305325975
-0.0628317032 0.2365044148
-0.0636943961 0.2424762321
-0.0623001479 0.2473556636
-0.0609058996 0.2522350951
-0.0595116514 0.2571145266
-0.0581174032 0.2619939582
-0.0567231550 0.2668733897
-0.0553289068 0.2717528212
-0.0539346585 0.2766322527
-0.0525404103 0.2815116842
-0.0526589399 0.2857464024
-0.0527774695 0.2899811206
-0.0528959991 0.2942158388
-0.0530145287 0.2984505570
-0.0531330583 0.3026852932
-0.0532515879 0.3069200114
-0.0533701175 0.3111547296
-0.0534886471 0.3153894478
-0.0541998203 0.3171609028
-0.0549109934 0.3189323577
-0.0556221666 0.3207038127
-0.0563333398 0.3224752677
-0.0570445130 0.3242467226
-0.0577556861 0.3260181776
-0.0584668593 0.3277896326
-0.0591780325 0.3295610875
-0.0587186166 0.3280815490
-0.0582592007 0.3266020104
-0.0577997848 0.3251224718
-0.0573403690 0.3236429332
-0.0568809531 0.3221633946
-0.0564215372 0.3206838560
-0.0559621213 0.3192043174
-0.0555027054 0.3177247788
-0.0551538453 0.3170201954
-0.0548049853 0.3163156120
-0.0544561252 0.3156110285
-0.0541072651 0.3149064451
-0.0537584050 0.3142018617
-0.0534095449 0.3134972782
-0.0530606849 0.3127926948
-0.0527118248 0.3120881114
-0.0548167826 0.3128264372
-0.0569217404 0.3135647629
-0.0590266982 0.3143030887
-0.0611316560 0.3150414145
-0.0632366138 0.3157797402
-0.0653415716 0.3165180660
-0.0674465294 0.3172563918
-0.0695514872 0.3179947176
-0.0685048275 0.3164145294
-0.0674581678 0.3148343411
-0.0664115081 0.3132541529
-0.0653648484 0.3116739647
-0.0643181887 0.3100937765
-0.0632715290 0.3085135883
-0.0622248693 0.3069334001
-0.0611782095 0.3053532119
-0.0580887179 0.3024893891
-0.0549992262 0.2996255664
-0.0519097345 0.2967617437
-0.0488202428 0.2938979210
-0.0457307511 0.2910340982
-0.0426412594 0.2881702755
-0.0395517677 0.2853064528
-0.0364622760 0.2824426301
-0.0326868615 0.2775833537
-0.0289114470 0.2727240774
-0.0251360325 0.2678648011
-0.0213606179 0.2630055247
-0.0175852045 0.2581462484
-0.0138097911 0.2532869721
-0.0100343777 0.2484276957
-0.0062589643 0.2435684194
0.0001336889 0.2375493809
0.0065263422 0.2315303423
0.0129189954 0.2255113037
0.0193116486 0.2194922652
0.0257043018 0.2134732266
0.0320969551 0.2074541881
0.0384896061 0.2014351495
0.0448822571 0.1954161110
0.0468383619 0.1900923812
0.0487944668 0.1847686515
0.0507505716 0.1794449217
0.0527066764 0.1741211919
0.0546627813 0.1687974622
0.0566188861 0.1634737324
0.0585749909 0.1581500027
0.0605310958 0.1528262729
0.0573347570 0.1496062609
0.0541384183 0.1463862490
0.0509420795 0.1431662370
0.0477457408 0.1399462251
0.0445494020 0.1367262131
0.0413530632 0.1335062012
0.0381567245 0.1302861892
0.0349603857 0.1270661773
0.0316930334 0.1232310803
0.0284256811 0.1193959833
0.0251583288 0.1155608863
0.0218909765 0.1117257894
0.0186236242 0.1078906924
0.0153562718 0.1040555954
0.0120889195 0.1002204984
0.0088215672 0.0963854015
0.0068062368 0.0920655606
0.0047909063 0.0877457196
0.0027755759 0.0834258787
0.0007602454 0.0791060378
-0.0012550850 0.0747861924
-0.0032704155 0.0704663469
-0.0052857459 0.0661465015
-0.0073010764 0.0618266561
-0.0074174216 0.0586539556
-0.0075337668 0.0554812551
-0.0076501120 0.0523085546
-0.0077664571 0.0491358541
-0.0078828023 0.0459631536
-0.0079991475 0.0427904531
-0.0081154927 0.0396177526
-0.0082318379 0.0364450521
-0.0078897904 0.0345497880
-0.0075477430 0.0326545239
-0.0072056955 0.0307592598
-0.0068636480 0.0288639957
-0.0065216005 0.0269687316
-0.0061795531 0.0250734675
-0.0058375056 0.0231782034
-0.0054954581 0.0212829392
-0.0057293268 0.0197358461
-0.0059631955 0.0181887529
-0.0061970642 0.0166416597
-0.0064309329 0.0150945665
-0.0066648016 0.0135474733
-0.0068986702 0.0120003801
-0.0071325389 0.0104532869
-0.0073664076 0.0089061937
-0.0064660500 0.0079958084
-0.0055656924 0.0070854232
-0.0046653351 0.0061750380
-0.0037649777 0.0052646528
-0.0028646204 0.0043542676
-0.0019642631 0.0034438823
-0.0010639058 0.0025334971
-0.0001635484 0.0016231119
0.0008146242 0.0009017073
0.0017927969 0.0001803028
0.0027709695 -0.0005411018
0.0037491422 -0.0012625063
0.0047273147 -0.0019839109
0.0057054874 -0.0027053154
0.0066836601 -0.0034267201
0.0076618329 -0.0041481246
0.0089823312 -0.0054739443
0.0103028296 -0.0067997641
0.0116233279 -0.0081255839
0.0129438263 -0.0094514037
0.0142643247 -0.0107772240
0.0155848230 -0.0121030432
0.0169053214 -0.0134288624
0.0182258197 -0.0147546816
0.0241125587 -0.0164975537
0.0299992977 -0.0182404258
0.0358860367 -0.0199832968
0.0417727779 -0.0217261700
0.0476595169 -0.0234690432
0.0535462559 -0.0252119164
0.0594329949 -0.0269547896
0.0653197339 -0.0286976629
0.0690928702 -0.0299182560
0.0728660065 -0.0311388492
0.0766391472 -0.0323594424
0.0804122879 -0.0335800356
0.0841854286 -0.0348006287
0.0879585694 -0.0360212219
0.0917317101 -0.0372418151
0.0955048508 -0.0384624083
0.0967586613 -0.0387394654
0.0980124719 -0.0390165225
0.0992662825 -0.0392935796
0.1005200930 -0.0395706367
0.1017739036 -0.0398476938
0.1030277141 -0.0401247510
0.1042815247 -0.0404018081
0.1055353353 -0.0406788652
0.1059945745 -0.0383464257
0.1064538138 -0.0360139863
0.1069130531 -0.0336815468
0.1073722924 -0.0313491073
0.1078315316 -0.0290166679
0.1082907709 -0.0266842284
0.1087500102 -0.0243517889
0.1092092495 -0.0220193495
0.1086021462 -0.0189509187
0.1079950430 -0.0158824879
0.1073879397 -0.0128140571
0.1067808365 -0.0097456263
0.1061737332 -0.0066771961
0.1055666300 -0.0036087658
0.1049595267 -0.0005403356
0.1043524235 0.0025280946
0.1055299399 0.0035794776
0.1067074564 0.0046308606
0.1078849728 0.0056822436
0.1090624893 0.0067336266
0.1102400058 0.0077850096
0.1114175222 0.0088363926
0.1125950387 0.0098877756
0.1137725551 0.0109391586
0.1079177952 0.0132961537
0.1020630353 0.0156531488
0.0962082753 0.0180101440
0.0903535154 0.0203671391
0.0844987555 0.0227241343
0.0786439955 0.0250811294
0.0727892400 0.0274381245
0.0669344845 0.0297951197
0.0550963905 0.0352131724
0.0432582965 0.0406312273
0.0314202025 0.0460492823
0.0195821086 0.0514673372
0.0077440135 0.0568853922
-0.0040940816 0.0623034471
-0.0159321767 0.0677215021
-0.0277702718 0.0731395570
-0.0313786782 0.0703238758
-0.0349870845 0.0675081945
-0.0385954909 0.0646925133
-0.0422038973 0.0618768320
-0.0458123037 0.0590611508
-0.0494207100 0.0562454695
-0.0530291164 0.0534297883
-0.0566375228 0.0506141070
-0.0508387163 0.0441844855
-0.0450399098 0.0377548640
-0.0392411033 0.0313252425
-0.0334422967 0.0248956210
-0.0276434902 0.0184659994
-0.0218446837 0.0120363779
-0.0160458783 0.0056067558
-0.0102470729 -0.0008228663
-0.0074104561 -0.0018265914
-0.0045738393 -0.0028303166
-0.0017372225 -0.0038340416
0.0010993943 -0.0048377670
0.0039360112 -0.0058414923
0.0067726280 -0.0068452176
0.0096092442 -0.0078489429
0.0124458616 -0.0088526682
0.0125821953 -0.0088821866
0.0127185291 -0.0089117049
0.0128548629 -0.0089412233
0.0129911966 -0.0089707416
0.0131275304 -0.0090002600
0.0132638642 -0.0090297783
0.0134001979 -0.0090592966
0.0135365317 -0.0090888150
0.0128314614 -0.0090277337
0.0121263911 -0.0089666524
0.0114213208 -0.0089055711
0.0107162504 -0.0088444898
0.0100111801 -0.0087834084
0.0093061098 -0.0087223271
0.0086010395 -0.0086612458
0.0078959692 -0.0086001645
0.0070079978 -0.0085836678
0.0061200264 -0.0085671710
0.0052320550 -0.0085506742
0.0043440836 -0.0085341775
0.0034561122 -0.0085176807
0.0025681408 -0.0085011840
0.0016801694 -0.0084846872
0.0007921980 -0.0084681905
-0.0000547684 -0.0085505874
-0.0009017347 -0.0086329844
-0.0017487011 -0.0087153813
-0.0025956674 -0.0087977783
-0.0034426338 -0.0088801752
-0.0042896001 -0.0089625722
-0.0051365668 -0.0090449691
-0.0059835329 -0.0091273661
-0.0051314341 -0.0089125620
-0.0042793354 -0.0086977579
-0.0034272367 -0.0084829539
-0.0025751380 -0.0082681498
-0.0017230393 -0.0080533457
-0.0008709406 -0.0078385416
-0.0000188419 -0.0076237376
0.0008332569 -0.0074089335
0.0008101721 -0.0072102563
0.0007870874 -0.0070115791
0.0007640027 -0.0068129018
0.0007409180 -0.0066142246
0.0007178333 -0.0064155474
0.0006947486 -0.0062168702
0.0006716639 -0.0060181930
0.0006485792 -0.0058195158
0.0005873651 -0.0059328943
0.0005261510 -0.0060462729
0.0004649369 -0.0061596514
0.0004037228 -0.0062730300
0.0003425087 -0.0063864086
0.0002812946 -0.0064997871
0.0002200805 -0.0066131657
0.0001588664 -0.0067265442
0.0006302485 -0.0070055896
0.0011016306 -0.0072846349
0.0015730127 -0.0075636803
0.0020443948 -0.0078427256
0.0025157769 -0.0081217709
0.0029871590 -0.0084008163
0.0034585411 -0.0086798616
0.0039299232 -0.0089589070
0.0047456255 -0.0093052334
0.0055613277 -0.0096515594
0.0063770300 -0.0099978853
0.0071927323 -0.0103442112
0.0080084346 -0.0106905371
0.0088241368 -0.0110368630
0.0096398391 -0.0113831889
0.0104555414 -0.0117295148
0.0104306873 -0.0119156108
0.0104058332 -0.0121017057
0.0103809791 -0.0122878006
0.0103561251 -0.0124738955
0.0103312710 -0.0126599903
0.0103064169 -0.0128460852
0.0102815628 -0.0130321801
0.0102567087 -0.0132182750
0.0101711472 -0.0129341503
0.0100855856 -0.0126500255
0.0100000241 -0.0123659008
0.0099144626 -0.0120817761
0.0098289010 -0.0117976513
0.0097433395 -0.0115135266
0.0096577780 -0.0112294018
0.0095722164 -0.0109452771
0.0092414000 -0.0108607487
0.0089105831 -0.0107762203
0.0085797661 -0.0106916919
0.0082489492 -0.0106071635
0.0079181322 -0.0105226351
0.0075873153 -0.0104381067
0.0072564984 -0.0103535783
0.0069256814 -0.0102690499
0.0071908156 -0.0108513275
0.0074559497 -0.0114336050
0.0077210839 -0.0120158826
0.0079862180 -0.0125981602
0.0082513521 -0.0131804378
0.0085164863 -0.0137627154
0.0087816204 -0.0143449930
0.0090467546 -0.0149272706
0.0102289594 -0.0155558717
0.0114111637 -0.0161844728
0.0125933679 -0.0168130739
0.0137755722 -0.0174416751
0.0149577765 -0.0180702762
0.0161399807 -0.0186988773
0.0173221850 -0.0193274773
0.0185043881 -0.0199560773
0.0217709457 -0.0206643350
0.0250375033 -0.0213725926
0.0283040609 -0.0220808503
0.0315706185 -0.0227891079
0.0348371761 -0.0234973656
0.0381037336 -0.0242056232
0.0413702912 -0.0249138809
0.0446368488 -0.0256221385
0.0501910550 -0.0281270857
0.0557452612 -0.0306320329
0.0612994674 -0.0331369801
0.0668536737 -0.0356419273
0.0724078799 -0.0381468722
0.0779620817 -0.0406518172
0.0835162835 -0.0431567621
0.0890704852 -0.0456617071
0.0968687756 -0.0507700226
0.1046670660 -0.0558783382
0.1124653564 -0.0609866538
0.1202636467 -0.0660949694
0.1280619371 -0.0712032849
0.1358602275 -0.0763116005
0.1436585179 -0.0814199116
0.1514568171 -0.0865282226
0.1625417319 -0.0937991201
0.1736266468 -0.1010700177
0.1847115617 -0.1083409152
0.1957964766 -0.1156118127
0.2068813915 -0.1228827103
0.2179663064 -0.1301536078
0.2290512213 -0.1374245053
0.2401361362 -0.1446954028
0.2547534857 -0.1523523074
0.2693708352 -0.1600092209
0.2839881846 -0.1676661344
0.2986055341 -0.1753230480
0.3132228836 -0.1829799615
0.3278402331 -0.1906368751
0.3424575826 -0.1982937886
0.3570749320 -0.2059507022
0.3755274730 -0.2142148516
0.3939800140 -0.2224790010
0.4124325549 -0.2307431504
0.4308850959 -0.2390072998
0.4493376368 -0.2472714492
0.4677901778 -0.2555355986
0.4862427187 -0.2637997480
0.5046952597 -0.2720638974
0.5217455786 -0.2794908939
0.5387958976 -0.2869178904
0.5558462165 -0.2943448868
0.5728965354 -0.3017718833
0.5899468544 -0.3091988617
0.6069971733 -0.3166258582
0.6240474923 -0.3240528546
0.6410978112 -0.3314798511
0.6452193175 -0.3318222908
0.6493408238 -0.3321647304
0.6534623301 -0.3325071701
0.6575838364 -0.3328496098
0.6617053427 -0.3331920495
0.6658268489 -0.3335344891
0.6699483552 -0.3338769288
0.6740698615 -0.3342193685
0.6759694434 -0.3350719130
0.6778690252 -0.3359244575
0.6797686071 -0.3367770020
0.6816681889 -0.3376295465
0.6835677708 -0.3384820910
0.6854673526 -0.3393346355
0.6873669345 -0.3401871800
0.6892665164 -0.3410397245
0.6875259512 -0.3414150043
0.6857853154 -0.3417902842
0.6840446796 -0.3421655640
0.6823040438 -0.3425408438
0.6805634080 -0.3429161236
0.6788227721 -0.3432914034
0.6770821363 -0.3436666832
0.6753415005 -0.3440419630
0.6714571417 -0.3442125152
0.6675727830 -0.3443830675
0.6636884242 -0.3445536197
0.6598040654 -0.3447241719
0.6559197066 -0.3448947241
0.6520353478 -0.3450652763
0.6481509890 -0.3452358285
0.6442666302 -0.3454063807
0.6340630005 -0.3445174594
0.6238593708 -0.3436285381
0.6136557411 -0.3427396169
0.6034521114 -0.3418506956
0.5932484817 -0.3409617743
0.5830448519 -0.3400728530
0.5728412222 -0.3391839317
0.5626375925 -0.3382950105
0.5494697603 -0.3339089389
0.5363019281 -0.3295228674
0.5231340960 -0.3251367958
0.5099662638 -0.3207507243
0.4967984316 -0.3163646527
0.4836305994 -0.3119785812
0.4704627672 -0.3075925096
0.4572949351 -0.3032064381
0.4426877581 -0.2946135264
0.4280805812 -0.2860206147
0.4134734043 -0.2774277030
0.3988662273 -0.2688347913
0.3842590504 -0.2602418796
0.3696518735 -0.2516489679
0.3550446965 -0.2430560562
0.3404375196 -0.2344631445
0.3234847229 -0.2219678135
0.3065319262 -0.2094724825
0.2895791118 -0.1969771516
0.2726262974 -0.1844818206
0.2556734831 -0.1719864896
0.2387206687 -0.1594911587
0.2217678543 -0.1469958367
0.2048150400 -0.1345005148
0.1883342424 -0.1244001503
0.1718534448 -0.1142997859
0.1553726472 -0.1041994215
0.1388918584 -0.0940990571
0.1224110696 -0.0839986927
0.1059302809 -0.0738983283
0.0894494921 -0.0637979639
0.0729687033 -0.0536975994
0.0592851354 -0.0453946960
0.0456015674 -0.0370917925
0.0319180017 -0.0287888890
0.0182344359 -0.0204859855
0.0045508702 -0.0121830832
-0.0091326955 -0.0038801808
-0.0228162613 0.0044227216
-0.0364998270 0.0127256239
-0.0432579745 0.0187764854
-0.0500161219 0.0248273468
-0.0567742694 0.0308782083
-0.0635324168 0.0369290698
-0.0702905643 0.0429799335
-0.0770487073 0.0490307972
-0.0838068548 0.0550816609
-0.0905650022 0.0611325246
-0.0951223650 0.0678136259
-0.0996797279 0.0744947271
-0.1042370907 0.0811758328
-0.1087944536 0.0878569340
-0.1133518164 0.0945380353
-0.1179091792 0.1012191365
-0.1224665421 0.1079002377
-0.1270239049 0.1145813389
-0.1286634687 0.1189465245
-0.1303030325 0.1233117010
-0.1319425963 0.1276768776
-0.1335821600 0.1320420542
-0.1352217238 0.1364072307
-0.1368612876 0.1407724073
-0.1385008514 0.1451375838
-0.1401404152 0.1495027604
-0.1353523598 0.1476697121
-0.1305643044 0.1458366638
-0.1257762491 0.1440036155
-0.1209881937 0.1421705673
-0.1162001384 0.1403375190
-0.1114120830 0.1385044707
-0.1066240276 0.1366714224
-0.1018359723 0.1348383741
-0.0970164721 0.1292075349
-0.0921969719 0.1235766957
-0.0873774717 0.1179458565
-0.0825579715 0.1123150173
-0.0777384713 0.1066841781
-0.0729189756 0.1010533389
-0.0680994798 0.0954224997
-0.0632799840 0.0897916604
-0.0613561982 0.0845377791
-0.0594324124 0.0792838978
-0.0575086266 0.0740300120
-0.0555848408 0.0687761262
-0.0536610550 0.0635222404
-0.0517372692 0.0582683546
-0.0498134834 0.0530144688
-0.0478896976 0.0477605829
-0.0467785543 0.0456636452
-0.0456674111 0.0435667074
-0.0445562679 0.0414697697
-0.0434451246 0.0393728319
-0.0423339814 0.0372758941
-0.0412228381 0.0351789564
-0.0401116949 0.0330820186
-0.0390005517 0.0309850809
-0.0374992047 0.0297741796
-0.0359978555 0.0285632783
-0.0344965064 0.0273523770
-0.0329951572 0.0261414758
-0.0314938081 0.0249305745
-0.0299924589 0.0237196732
-0.0284911098 0.0225087720
-0.0269897606 0.0212978707
-0.0256983173 0.0206689098
-0.0244068741 0.0200399489
-0.0231154309 0.0194109880
-0.0218239876 0.0187820283
-0.0205325444 0.0181530685
-0.0192411011 0.0175241088
-0.0179496568 0.0168951490
-0.0166582124 0.0162661893
-0.0165173079 0.0158800424
-0.0163764033 0.0154938956
-0.0162354987 0.0151077488
-0.0160945942 0.0147216019
-0.0159536896 0.0143354551
-0.0158127850 0.0139493083
-0.0156718805 0.0135631614
-0.0155309759 0.0131770146
-0.0161149955 0.0131605799
-0.0166990152 0.0131441451
-0.0172830349 0.0131277104
-0.0178670545 0.0131112757
-0.0184510742 0.0130948409
-0.0190350938 0.0130784062
-0.0196191123 0.0130619715
-0.0202031331 0.0130455367
-0.0197195618 0.0129257965
-0.0192359906 0.0128060563
-0.0187524193 0.0126863161
-0.0182688480 0.0125665759
-0.0177852768 0.0124468357
-0.0173017055 0.0123270955
-0.0168181342 0.0122073553
-0.0163345630 0.0120876151
-0.0157893913 0.0118813097
-0.0152442196 0.0116750033
-0.0146990479 0.0114686968
-0.0141538762 0.0112623904
-0.0136087045 0.0110560839
-0.0130635328 0.0108497774
-0.0125183611 0.0106434710
-0.0119731894 0.0104371645
-0.0119392224 0.0104568325
-0.0119052554 0.0104765005
-0.0118712884 0.0104961685
-0.0118373215 0.0105158365
-0.0118033545 0.0105355045
-0.0117693875 0.0105551725
-0.0117354205 0.0105748405
-0.0117014535 0.0105945085
-0.0116597566 0.0104985684
-0.0116180598 0.0104026282
-0.0115763630 0.0103066881
-0.0115346661 0.0102107480
-0.0114929693 0.0101148079
-0.0114512724 0.0100188677
-0.0114095756 0.0099229276
-0.0113678787 0.0098269875
-0.0112565414 0.0097505259
-0.0111452041 0.0096740643
-0.0110338669 0.0095976027
-0.0109225296 0.0095211411
-0.0108111923 0.0094446795
-0.0106998550 0.0093682179
-0.0105885177 0.0092917563
-0.0104771804 0.0092152947
-0.0105914251 0.0090131891
-0.0107056698 0.0088110836
-0.0108199144 0.0086089780
-0.0109341591 0.0084068724
-0.0110484038 0.0082047668
-0.0111626485 0.0080026612
-0.0112768932 0.0078005557
-0.0113911378 0.0075984501
-0.0115884693 0.0075021242
-0.0117858009 0.0074057984
-0.0119831324 0.0073094726
-0.0121804639 0.0072131468
-0.0123777954 0.0071168210
-0.0125751269 0.0070204952
-0.0127724584 0.0069241693
-0.0129697900 0.0068278435
-0.0130463744 0.0067145005
-0.0131229588 0.0066011575
-0.0131995432 0.0064878144
-0.0132761276 0.0063744714
-0.0133527120 0.0062611283
-0.0134292964 0.0061477853
-0.0135058808 0.0060344423
-0.0135824652 0.0059210992
-0.0132259061 0.0058319589
-0.0128693471 0.0057428186
-0.0125127881 0.0056536782
-0.0121562290 0.0055645379
-0.0117996700 0.0054753975
-0.0114431110 0.0053862572
-0.0110865520 0.0052971168
-0.0107299929 0.0052079765
-0.0104160359 0.0051489725
-0.0101020788 0.0050899685
-0.0097881217 0.0050309645
-0.0094741646 0.0049719605
-0.0091602076 0.0049129565
-0.0088462505 0.0048539525
-0.0085322934 0.0047949485
-0.0082183363 0.0047359446
-0.0081385791 0.0046087149
-0.0080588218 0.0044814853
-0.0079790646 0.0043542557
-0.0078993073 0.0042270261
-0.0078195501 0.0040997965
-0.0077397928 0.0039725669
-0.0076600356 0.0038453373
-0.0075802783 0.0037181077
-0.0075535235 0.0036434536
-0.0075267687 0.0035687995
-0.0075000139 0.0034941454
-0.0074732591 0.0034194913
-0.0074465043 0.0033448372
-0.0074197495 0.0032701831
-0.0073929946 0.0031955291
-0.0073662398 0.0031208750
-0.0072309911 0.0030975491
-0.0070957424 0.0030742232
-0.0069604936 0.0030508974
-0.0068252449 0.0030275715
-0.0066899962 0.0030042457
-0.0065547474 0.0029809198
-0.0064194987 0.0029575939
-0.0062842499 0.0029342681
-0.0061784278 0.0030713726
-0.0060726056 0.0032084771
-0.0059667834 0.0033455816
-0.0058609612 0.0034826860
-0.0057551390 0.0036197905
-0.0056493168 0.0037568950
-0.0055434946 0.0038939995
-0.0054376724 0.0040311040


==> data/gru_sample53.tex <==
-0.0074197478 0.0021975888
-0.0075798103 0.0021211041
-0.0077398729 0.0020446194
-0.0078999354 0.0019681347
-0.0080599979 0.0018916500
-0.0082200605 0.0018151653
-0.0083801230 0.0017386806
-0.0085401855 0.0016621958
-0.0083134115 0.0018189000
-0.0080866374 0.0019756041
-0.0078598633 0.0021323082
-0.0076330893 0.0022890123
-0.0074063152 0.0024457163
-0.0071795411 0.0026024203
-0.0069527671 0.0027591242
-0.0067259930 0.0029158282
-0.0063038958 0.0028594073
-0.0058817986 0.0028029865
-0.0054597013 0.0027465656
-0.0050376041 0.0026901447
-0.0046155069 0.0026337238
-0.0041934096 0.0025773030
-0.0037713124 0.0025208821
-0.0033492152 0.0024644612
-0.0029414628 0.0021043125
-0.0025337105 0.0017441637
-0.0021259580 0.0013840149
-0.0017182055 0.0010238662
-0.0013104530 0.0006637174
-0.0009027005 0.0003035686
-0.0004949480 -0.0000565801
-0.0000871956 -0.0004167289
0.0002698249 -0.0007528608
0.0006268453 -0.0010889926
0.0009838658 -0.0014251245
0.0013408862 -0.0017612564
0.0016979066 -0.0020973883
0.0020549271 -0.0024335201
0.0024119476 -0.0027696520
0.0027689680 -0.0031057839
0.0026041989 -0.0031412303
0.0024394298 -0.0031766766
0.0022746607 -0.0032121230
0.0021098916 -0.0032475694
0.0019451225 -0.0032830158
0.0017803534 -0.0033184621
0.0016155843 -0.0033539085
0.0014508152 -0.0033893549
0.0013307886 -0.0031792676
0.0012107620 -0.0029691804
0.0010907354 -0.0027590931
0.0009707088 -0.0025490059
0.0008506821 -0.0023389188
0.0007306555 -0.0021288317
0.0006106289 -0.0019187446
0.0004906023 -0.0017086575
0.0004277772 -0.0014490030
0.0003649521 -0.0011893485
0.0003021270 -0.0009296940
0.0002393020 -0.0006700395
0.0001764769 -0.0004103850
0.0001136518 -0.0001507305
0.0000508267 0.0001089240
-0.0000119984 0.0003685785
-0.0001801343 0.0004693010
-0.0003482702 0.0005700235
-0.0005164062 0.0006707460
-0.0006845421 0.0007714685
-0.0008526781 0.0008721910
-0.0010208140 0.0009729135
-0.0011889499 0.0010736360
-0.0013570859 0.0011743585
-0.0016036835 0.0010391124
-0.0018502811 0.0009038663
-0.0020968787 0.0007686202
-0.0023434764 0.0006333741
-0.0025900740 0.0004981280
-0.0028366716 0.0003628819
-0.0030832692 0.0002276359
-0.0033298668 0.0000923898
-0.0036231145 0.0000074924
-0.0039163623 -0.0000774050
-0.0042096100 -0.0001623024
-0.0045028577 -0.0002471998
-0.0047961055 -0.0003320972
-0.0050893532 -0.0004169946
-0.0053826009 -0.0005018920
-0.0056758486 -0.0005867894
-0.0055955422 -0.0006197103
-0.0055152359 -0.0006526312
-0.0054349295 -0.0006855520
-0.0053546231 -0.0007184729
-0.0052743167 -0.0007513938
-0.0051940103 -0.0007843146
-0.0051137039 -0.0008172355
-0.0050333975 -0.0008501563
-0.0049497373 -0.0008394164
-0.0048660770 -0.0008286764
-0.0047824168 -0.0008179365
-0.0046987565 -0.0008071966
-0.0046150963 -0.0007964566
-0.0045314360 -0.0007857167
-0.0044477757 -0.0007749768
-0.0043641155 -0.0007642368
-0.0041200422 -0.0007605704
-0.0038759690 -0.0007569040
-0.0036318958 -0.0007532376
-0.0033878225 -0.0007495713
-0.0031437493 -0.0007459049
-0.0028996760 -0.0007422385
-0.0026556028 -0.0007385721
-0.0024115295 -0.0007349057
-0.0023117785 -0.0007286554
-0.0022120274 -0.0007224051
-0.0021122764 -0.0007161548
-0.0020125253 -0.0007099045
-0.0019127742 -0.0007036543
-0.0018130232 -0.0006974040
-0.0017132721 -0.0006911537
-0.0016135211 -0.0006849034
-0.0017428187 -0.0006113983
-0.0018721163 -0.0005378932
-0.0020014140 -0.0004643881
-0.0021307116 -0.0003908830
-0.0022600093 -0.0003173779
-0.0023893069 -0.0002438729
-0.0025186045 -0.0001703678
-0.0026479022 -0.0000968627
-0.0032137184 -0.0001003060
-0.0037795346 -0.0001037493
-0.0043453507 -0.0001071925
-0.0049111669 -0.0001106358
-0.0054769828 -0.0001140791
-0.0060427988 -0.0001175223
-0.0066086147 -0.0001209656
-0.0071744306 -0.0001244089
-0.0074647582 -0.0000140341
-0.0077550859 0.0000963407
-0.0080454135 0.0002067155
-0.0083357412 0.0003170903
-0.0086260688 0.0004274651
-0.0089163965 0.0005378398
-0.0092067241 0.0006482146
-0.0094970518 0.0007585894
-0.0090300065 0.0009401197
-0.0085629612 0.0011216500
-0.0080959159 0.0013031803
-0.0076288706 0.0014847106
-0.0071618253 0.0016662410
-0.0066947800 0.0018477713
-0.0062277347 0.0020293016
-0.0057606894 0.0022108319
-0.0057734812 0.0022755608
-0.0057862731 0.0023402898
-0.0057990649 0.0024050188
-0.0058118568 0.0024697478
-0.0058246486 0.0025344769
-0.0058374405 0.0025992059
-0.0058502323 0.0026639349
-0.0058630242 0.0027286639
-0.0056692673 0.0026707629
-0.0054755104 0.0026128618
-0.0052817535 0.0025549608
-0.0050879966 0.0024970597
-0.0048942397 0.0024391587
-0.0047004828 0.0023812576
-0.0045067260 0.0023233566
-0.0043129691 0.0022654555
-0.0040500591 0.0021988467
-0.0037871491 0.0021322379
-0.0035242391 0.0020656290
-0.0032613291 0.0019990202
-0.0029984191 0.0019324113
-0.0027355090 0.0018658025
-0.0024725990 0.0017991936
-0.0022096892 0.0017325848
-0.0025060249 0.0015964640
-0.0028023608 0.0014603432
-0.0030986963 0.0013242224
-0.0033950319 0.0011881015
-0.0036913675 0.0010519807
-0.0039877031 0.0009158599
-0.0042840387 0.0007797391
-0.0045803743 0.0006436183
-0.0045166295 0.0005828440
-0.0044528846 0.0005220696
-0.0043891398 0.0004612953
-0.0043253950 0.0004005209
-0.0042616502 0.0003397466
-0.0041979054 0.0002789722
-0.0041341606 0.0002181979
-0.0040704158 0.0001574235
-0.0040396931 0.0000478830
-0.0040089704 -0.0000616576
-0.0039782477 -0.0001711982
-0.0039475251 -0.0002807388
-0.0039168024 -0.0003902793
-0.0038860797 -0.0004998199
-0.0038553571 -0.0006093605
-0.0038246344 -0.0007189010
-0.0038827700 -0.0007574419
-0.0039409056 -0.0007959828
-0.0039990413 -0.0008345236
-0.0040571769 -0.0008730645
-0.0041153125 -0.0009116053
-0.0041734481 -0.0009501462
-0.0042315837 -0.0009886871
-0.0042897194 -0.0010272279
-0.0041340082 -0.0010105363
-0.0039782971 -0.0009938446
-0.0038225860 -0.0009771530
-0.0036668749 -0.0009604613
-0.0035111638 -0.0009437697
-0.0033554527 -0.0009270780
-0.0031997416 -0.0009103864
-0.0030440305 -0.0008936947
-0.0029694693 -0.0008968880
-0.0028949082 -0.0009000813
-0.0028203470 -0.0009032746
-0.0027457859 -0.0009064679
-0.0026712248 -0.0009096612
-0.0025966636 -0.0009128545
-0.0025221025 -0.0009160478
-0.0024475413 -0.0009192411
-0.0022578008 -0.0009296842
-0.0020680604 -0.0009401272
-0.0018783199 -0.0009505703
-0.0016885795 -0.0009610134
-0.0014988390 -0.0009714564
-0.0013090985 -0.0009818995
-0.0011193581 -0.0009923425
-0.0009296177 -0.0010027856
-0.0011251866 -0.0010006254
-0.0013207554 -0.0009984653
-0.0015163242 -0.0009963052
-0.0017118929 -0.0009941450
-0.0019074617 -0.0009919849
-0.0021030304 -0.0009898247
-0.0022985992 -0.0009876646
-0.0024941680 -0.0009855045
-0.0025203891 -0.0010172016
-0.0025466102 -0.0010488988
-0.0025728314 -0.0010805960
-0.0025990525 -0.0011122931
-0.0026252736 -0.0011439903
-0.0026514947 -0.0011756875
-0.0026777159 -0.0012073846
-0.0027039370 -0.0012390818
-0.0028254750 -0.0012072816
-0.0029470130 -0.0011754815
-0.0030685510 -0.0011436814
-0.0031900889 -0.0011118812
-0.0033116269 -0.0010800811
-0.0034331649 -0.0010482809
-0.0035547029 -0.0010164808
-0.0036762409 -0.0009846806
-0.0036633618 -0.0009566000
-0.0036504828 -0.0009285193
-0.0036376037 -0.0009004386
-0.0036247247 -0.0008723579
-0.0036118457 -0.0008442773
-0.0035989666 -0.0008161966
-0.0035860876 -0.0007881159
-0.0035732085 -0.0007600352
-0.0035086726 -0.0007513907
-0.0034441366 -0.0007427462
-0.0033796006 -0.0007341017
-0.0033150647 -0.0007254572
-0.0032505287 -0.0007168127
-0.0031859928 -0.0007081682
-0.0031214568 -0.0006995237
-0.0030569209 -0.0006908792
-0.0027721638 -0.0006024207
-0.0024874067 -0.0005139621
-0.0022026496 -0.0004255036
-0.0019178925 -0.0003370450
-0.0016331354 -0.0002485865
-0.0013483783 -0.0001601280
-0.0010636213 -0.0000716695
-0.0007788642 0.0000167891
-0.0002381466 0.0000481902
0.0003025710 0.0000795914
0.0008432885 0.0001109925
0.0013840061 0.0001423937
0.0019247238 0.0001737948
0.0024654412 0.0002051959
0.0030061588 0.0002365971
0.0035468765 0.0002679982
0.0035448656 0.0001703280
0.0035428548 0.0000726579
0.0035408440 -0.0000250123
0.0035388331 -0.0001226825
0.0035368223 -0.0002203526
0.0035348115 -0.0003180228
0.0035328006 -0.0004156930
0.0035307898 -0.0005133632
0.0038573282 -0.0006079874
0.0041838665 -0.0007026117
0.0045104049 -0.0007972360
0.0048369433 -0.0008918603
0.0051634814 -0.0009864846
0.0054900195 -0.0010811089
0.0058165576 -0.0011757333
0.0061430957 -0.0012703576
0.0062300353 -0.0012644856
0.0063169749 -0.0012586136
0.0064039145 -0.0012527416
0.0064908542 -0.0012468696
0.0065777938 -0.0012409976
0.0066647334 -0.0012351256
0.0067516730 -0.0012292536
0.0068386126 -0.0012233816
0.0062711201 -0.0012796776
0.0057036275 -0.0013359736
0.0051361349 -0.0013922696
0.0045686424 -0.0014485655
0.0040011498 -0.0015048615
0.0034336572 -0.0015611575
0.0028661646 -0.0016174535
0.0022986721 -0.0016737494
0.0025139115 -0.0018029144
0.0027291509 -0.0019320794
0.0029443904 -0.0020612444
0.0031596298 -0.0021904093
0.0033748692 -0.0023195743
0.0035901087 -0.0024487393
0.0038053481 -0.0025779043
0.0040205876 -0.0027070691
0.0036846181 -0.0025321762
0.0033486487 -0.0023572834
0.0030126792 -0.0021823906
0.0026767098 -0.0020074978
0.0023407403 -0.0018326050
0.0020047708 -0.0016577122
0.0016688012 -0.0014828195
0.0013328316 -0.0013079267
0.0008675051 -0.0012747607
0.0004021786 -0.0012415947
-0.0000631479 -0.0012084287
-0.0005284744 -0.0011752627
-0.0009938008 -0.0011420967
-0.0014591273 -0.0011089307
-0.0019244537 -0.0010757647
-0.0023897801 -0.0010425987
-0.0028823236 -0.0009145741
-0.0033748670 -0.0007865495
-0.0038674105 -0.0006585249
-0.0043599539 -0.0005305003
-0.0048524976 -0.0004024757
-0.0053450411 -0.0002744511
-0.0058375845 -0.0001464265
-0.0063301280 -0.0000184019
-0.0063141329 0.0000776362
-0.0062981379 0.0001736744
-0.0062821428 0.0002697125
-0.0062661478 0.0003657506
-0.0062501527 0.0004617888
-0.0062341577 0.0005578269
-0.0062181626 0.0006538651
-0.0062021676 0.0007499032
-0.0062298705 0.0007949826
-0.0062575735 0.0008400620
-0.0062852765 0.0008851414
-0.0063129794 0.0009302209
-0.0063406824 0.0009753003
-0.0063683854 0.0010203797
-0.0063960884 0.0010654591
-0.0064237913 0.0011105386
-0.0070142836 0.0012903743
-0.0076047759 0.0014702100
-0.0081952682 0.0016500457
-0.0087857605 0.0018298814
-0.0093762528 0.0020097172
-0.0099667451 0.0021895529
-0.0105572373 0.0023693886
-0.0111477296 0.0025492245
-0.0111060769 0.0026624037
-0.0110644242 0.0027755826
-0.0110227715 0.0028887616
-0.0109811188 0.0030019405
-0.0109394662 0.0031151195
-0.0108978135 0.0032282984
-0.0108561608 0.0033414774
-0.0108145081 0.0034546563
-0.0108678124 0.0035258606
-0.0109211167 0.0035970649
-0.0109744210 0.0036682692
-0.0110277254 0.0037394735
-0.0110810297 0.0038106778
-0.0111343340 0.0038818821
-0.0111876383 0.0039530864
-0.0112409426 0.0040242907
-0.0112900172 0.0041522311
-0.0113390918 0.0042801714
-0.0113881664 0.0044081118
-0.0114372410 0.0045360522
-0.0114863156 0.0046639928
-0.0115353902 0.0047919329
-0.0115844648 0.0049198730
-0.0116335394 0.0050478131
-0.0117768204 0.0050424540
-0.0119201014 0.0050370950
-0.0120633825 0.0050317359
-0.0122066635 0.0050263768
-0.0123499445 0.0050210177
-0.0124932256 0.0050156587
-0.0126365066 0.0050102996
-0.0127797876 0.0050049405
-0.0128967211 0.0046294267
-0.0130136547 0.0042539129
-0.0131305882 0.0038783990
-0.0132475217 0.0035028852
-0.0133644552 0.0031273714
-0.0134813887 0.0027518576
-0.0135983222 0.0023763437
-0.0137152557 0.0020008299
-0.0132138086 0.0018043772
-0.0127123614 0.0016079245
-0.0122109142 0.0014114717
-0.0117094670 0.0012150190
-0.0112080198 0.0010185663
-0.0107065727 0.0008221136
-0.0102051255 0.0006256608
-0.0097036783 0.0004292081
-0.0091748565 0.0004263839
-0.0086460348 0.0004235597
-0.0081172130 0.0004207355
-0.0075883912 0.0004179113
-0.0070595694 0.0004150871
-0.0065307477 0.0004122629
-0.0060019259 0.0004094387
-0.0054731041 0.0004066145
-0.0054057839 0.0005978063
-0.0053384636 0.0007889982
-0.0052711433 0.0009801900
-0.0052038230 0.0011713818
-0.0051365028 0.0013625735
-0.0050691825 0.0015537653
-0.0050018622 0.0017449571
-0.0049345419 0.0019361488
-0.0051070724 0.0020387306
-0.0052796028 0.0021413123
-0.0054521332 0.0022438941
-0.0056246636 0.0023464758
-0.0057971940 0.0024490575
-0.0059697244 0.0025516393
-0.0061422548 0.0026542210
-0.0063147852 0.0027568028
-0.0063556344 0.0028201469
-0.0063964835 0.0028834910
-0.0064373327 0.0029468352
-0.0064781818 0.0030101793
-0.0065190309 0.0030735235
-0.0065598801 0.0031368676
-0.0066007292 0.0032002118
-0.0066415783 0.0032635559
-0.0066155079 0.0032428518
-0.0065894374 0.0032221477
-0.0065633669 0.0032014436
-0.0065372965 0.0031807394
-0.0065112260 0.0031600353
-0.0064851555 0.0031393312
-0.0064590851 0.0031186271
-0.0064330146 0.0030979230
-0.0065984002 0.0031065398
-0.0067637858 0.0031151567
-0.0069291713 0.0031237736
-0.0070945569 0.0031323904
-0.0072599425 0.0031410073
-0.0074253280 0.0031496242
-0.0075907136 0.0031582411
-0.0077560992 0.0031668579
-0.0078251535 0.0031403690
-0.0078942078 0.0031138801
-0.0079632622 0.0030873912
-0.0080323165 0.0030609022
-0.0081013708 0.0030344133
-0.0081704251 0.0030079244
-0.0082394795 0.0029814355
-0.0083085338 0.0029549465
-0.0080979711 0.0028452168
-0.0078874085 0.0027354871
-0.0076768458 0.0026257574
-0.0074662831 0.0025160277
-0.0072557205 0.0024062980
-0.0070451578 0.0022965682
-0.0068345951 0.0021868387
-0.0066240324 0.0020771091
-0.0065037522 0.0020834757
-0.0063834720 0.0020898423
-0.0062631918 0.0020962088
-0.0061429116 0.0021025754
-0.0060226314 0.0021089420
-0.0059023512 0.0021153086
-0.0057820710 0.0021216752
-0.0056617907 0.0021280418
-0.0054005557 0.0019701803
-0.0051393207 0.0018123188
-0.0048780857 0.0016544574
-0.0046168507 0.0014965959
-0.0043556157 0.0013387344
-0.0040943807 0.0011808729
-0.0038331457 0.0010230115
-0.0035719107 0.0008651500
-0.0035852440 0.0008112599
-0.0035985772 0.0007573699
-0.0036119105 0.0007034798
-0.0036252438 0.0006495898
-0.0036385770 0.0005956997
-0.0036519103 0.0005418097
-0.0036652435 0.0004879196
-0.0036785768 0.0004340295
-0.0037696534 0.0004217069
-0.0038607300 0.0004093843
-0.0039518067 0.0003970618
-0.0040428833 0.0003847392
-0.0041339600 0.0003724166
-0.0042250366 0.0003600940
-0.0043161132 0.0003477714
-0.0044071899 0.0003354488
-0.0043871075 0.0003527040
-0.0043670251 0.0003699592
-0.0043469427 0.0003872144
-0.0043268603 0.0004044696
-0.0043067779 0.0004217248
-0.0042866955 0.0004389800
-0.0042666131 0.0004562352
-0.0042465307 0.0004734904
-0.0040992164 0.0005782121
-0.0039519022 0.0006829337
-0.0038045879 0.0007876554
-0.0036572736 0.0008923770
-0.0035099593 0.0009970987
-0.0033626450 0.0011018203
-0.0032153307 0.0012065420
-0.0030680164 0.0013112636
-0.0030775507 0.0013939716
-0.0030870850 0.0014766795
-0.0030966193 0.0015593874
-0.0031061536 0.0016420954
-0.0031156878 0.0017248033
-0.0031252221 0.0018075112
-0.0031347564 0.0018902191
-0.0031442907 0.0019729271
-0.0031287727 0.0020801550
-0.0031132548 0.0021873830
-0.0030977369 0.0022946108
-0.0030822189 0.0024018386
-0.0030667010 0.0025090664
-0.0030511831 0.0026162941
-0.0030356651 0.0027235219
-0.0030201472 0.0028307497
-0.0033335159 0.0027450203
-0.0036468847 0.0026592908
-0.0039602535 0.0025735614
-0.0042736222 0.0024878319
-0.0045869910 0.0024021024
-0.0049003597 0.0023163730
-0.0052137285 0.0022306434
-0.0055270972 0.0021449138
-0.0056810304 0.0020298074
-0.0058349636 0.0019147010
-0.0059888967 0.0017995945
-0.0061428299 0.0016844881
-0.0062967631 0.0015693817
-0.0064506963 0.0014542753
-0.0066046294 0.0013391689
-0.0067585626 0.0012240625
-0.0065733342 0.0010876336
-0.0063881057 0.0009512049
-0.0062028773 0.0008147761
-0.0060176489 0.0006783474
-0.0058324204 0.0005419186
-0.0056471920 0.0004054899
-0.0054619636 0.0002690611
-0.0052767351 0.0001326324
-0.0049532396 0.0001167373
-0.0046297441 0.0001008422
-0.0043062486 0.0000849471
-0.0039827531 0.0000690519
-0.0036592577 0.0000531568
-0.0033357622 0.0000372617
-0.0030122667 0.0000213666
-0.0026887712 0.0000054715
-0.0025634235 0.0000948150
-0.0024380757 0.0001841585
-0.0023127280 0.0002735021
-0.0021873803 0.0003628455
-0.0020620326 0.0004521890
-0.0019366849 0.0005415325
-0.0018113371 0.0006308760
-0.0016859894 0.0007202195
-0.0014834218 0.0008911519
-0.0012808542 0.0010620844
-0.0010782865 0.0012330168
-0.0008757189 0.0014039494
-0.0006731513 0.0015748819
-0.0004705836 0.0017458144
-0.0002680160 0.0019167470
-0.0000654484 0.0020876795
-0.0004828775 0.0021484827
-0.0009003065 0.0022092859
-0.0013177357 0.0022700889
-0.0017351647 0.0023308919
-0.0021525937 0.0023916950
-0.0025700228 0.0024524980
-0.0029874518 0.0025133011
-0.0034048808 0.0025741041
-0.0035376154 0.0025852454
-0.0036703499 0.0025963868
-0.0038030845 0.0026075281
-0.0039358191 0.0026186695
-0.0040685537 0.0026298108
-0.0042012882 0.0026409522
-0.0043340228 0.0026520935
-0.0044667574 0.0026632349
-0.0043039859 0.0027702413
-0.0041412144 0.0028772478
-0.0039784428 0.0029842543
-0.0038156713 0.0030912608
-0.0036528998 0.0031982672
-0.0034901283 0.0033052737
-0.0033273568 0.0034122802
-0.0031645853 0.0035192867
-0.0029286379 0.0034888162
-0.0026926905 0.0034583458
-0.0024567431 0.0034278753
-0.0022207955 0.0033974049
-0.0019848480 0.0033669344
-0.0017489004 0.0033364640
-0.0015129529 0.0033059935
-0.0012770054 0.0032755231
-0.0014714280 0.0030788011
-0.0016658506 0.0028820791
-0.0018602732 0.0026853571
-0.0020546958 0.0024886351
-0.0022491184 0.0022919132
-0.0024435412 0.0020951913
-0.0026379639 0.0018984695
-0.0028323867 0.0017017477
-0.0030539359 0.0016939347
-0.0032754852 0.0016861217
-0.0034970345 0.0016783086
-0.0037185837 0.0016704955
-0.0039401330 0.0016626825
-0.0041616822 0.0016548694
-0.0043832315 0.0016470563
-0.0046047808 0.0016392433
-0.0045930488 0.0017120756
-0.0045813169 0.0017849080
-0.0045695850 0.0018577403
-0.0045578531 0.0019305727
-0.0045461211 0.0020034050
-0.0045343892 0.0020762373
-0.0045226573 0.0021490697
-0.0045109253 0.0022219020
-0.0046984811 0.0021354245
-0.0048860369 0.0020489469
-0.0050735927 0.0019624693
-0.0052611485 0.0018759917
-0.0054487043 0.0017895141
-0.0056362600 0.0017030365
-0.0058238158 0.0016165590
-0.0060113716 0.0015300814
-0.0056103110 0.0014278608
-0.0052092504 0.0013256402
-0.0048081898 0.0012234196
-0.0044071289 0.0011211991
-0.0040060680 0.0010189784
-0.0036050071 0.0009167578
-0.0032039462 0.0008145371
-0.0028028853 0.0007123165
-0.0026319891 0.0006077401
-0.0024610928 0.0005031637
-0.0022901966 0.0003985873
-0.0021193003 0.0002940109
-0.0019484041 0.0001894346
-0.0017775078 0.0000848582
-0.0016066116 -0.0000197182
-0.0014357153 -0.0001242945
-0.0017426650 0.0000434213
-0.0020496146 0.0002111371
-0.0023565643 0.0003788529
-0.0026635139 0.0005465687
-0.0029704636 0.0007142845
-0.0032774132 0.0008820003
-0.0035843629 0.0010497161
-0.0038913125 0.0012174318
-0.0038980644 0.0013876343
-0.0039048163 0.0015578368
-0.0039115682 0.0017280392
-0.0039183201 0.0018982417
-0.0039250720 0.0020684442
-0.0039318239 0.0022386466
-0.0039385758 0.0024088492
-0.0039453277 0.0025790518
-0.0042805330 0.0027858286
-0.0046157384 0.0029926053
-0.0049509437 0.0031993820
-0.0052861488 0.0034061588
-0.0056213539 0.0036129355
-0.0059565589 0.0038197122
-0.0062917640 0.0040264890
-0.0066269691 0.0042332657
-0.0072255571 0.0042805340
-0.0078241452 0.0043278020
-0.0084227332 0.0043750701
-0.0090213213 0.0044223381
-0.0096199093 0.0044696062
-0.0102184979 0.0045168742
-0.0108170865 0.0045641422
-0.0114156751 0.0046114103
-0.0110299296 0.0045437350
-0.0106441841 0.0044760597
-0.0102584386 0.0044083844
-0.0098726931 0.0043407092
-0.0094869476 0.0042730339
-0.0091012027 0.0042053586
-0.0087154578 0.0041376833
-0.0083297128 0.0040700081
-0.0078689663 0.0038970650
-0.0074082198 0.0037241220
-0.0069474733 0.0035511789
-0.0064867268 0.0033782359
-0.0060259803 0.0032052929
-0.0055652338 0.0030323498
-0.0051044873 0.0028594068
-0.0046437408 0.0026864637
-0.0046691067 0.0023612076
-0.0046944727 0.0020359515
-0.0047198389 0.0017106954
-0.0047452052 0.0013854393
-0.0047705714 0.0010601832
-0.0047959377 0.0007349271
-0.0048213039 0.0004096709
-0.0048466702 0.0000844148
-0.0048773015 -0.0000158543
-0.0049079328 -0.0001161234
-0.0049385642 -0.0002163925
-0.0049691955 -0.0003166616
-0.0049998268 -0.0004169307
-0.0050304582 -0.0005171998
-0.0050610895 -0.0006174689
-0.0050917208 -0.0007177380
-0.0050455597 -0.0005648717
-0.0049993985 -0.0004120054
-0.0049532374 -0.0002591391
-0.0049070763 -0.0001062728
-0.0048609152 0.0000465935
-0.0048147540 0.0001994598
-0.0047685929 0.0003523262
-0.0047224318 0.0005051925
-0.0046090331 0.0006120177
-0.0044956345 0.0007188430
-0.0043822359 0.0008256682
-0.0042688373 0.0009324935
-0.0041554386 0.0010393188
-0.0040420400 0.0011461441
-0.0039286414 0.0012529694
-0.0038152428 0.0013597948
-0.0038786071 0.0012452769
-0.0039419713 0.0011307590
-0.0040053356 0.0010162411
-0.0040686999 0.0009017233
-0.0041320642 0.0007872054
-0.0041954285 0.0006726875
-0.0042587928 0.0005581697
-0.0043221570 0.0004436518
-0.0042497842 0.0004298497
-0.0041774113 0.0004160477
-0.0041050384 0.0004022457
-0.0040326655 0.0003884438
-0.0039602926 0.0003746418
-0.0038879198 0.0003608398
-0.0038155469 0.0003470378
-0.0037431740 0.0003332358
-0.0036724129 0.0003743883
-0.0036016519 0.0004155407
-0.0035308908 0.0004566932
-0.0034601297 0.0004978457
-0.0033893687 0.0005389982
-0.0033186076 0.0005801508
-0.0032478465 0.0006213033
-0.0031770854 0.0006624558
-0.0029112692 0.0006529123
-0.0026454529 0.0006433689
-0.0023796364 0.0006338254
-0.0021138200 0.0006242820
-0.0018480036 0.0006147385
-0.0015821872 0.0006051950
-0.0013163707 0.0005956516
-0.0010505543 0.0005861081
-0.0007912559 0.0004601085
-0.0005319575 0.0003341089
-0.0002726592 0.0002081094
-0.0000133608 0.0000821098
0.0002459376 -0.0000438899
0.0005052359 -0.0001698895
0.0007645343 -0.0002958891
0.0010238326 -0.0004218886
0.0012514260 -0.0004687955
0.0014790193 -0.0005157023
0.0017066127 -0.0005626092
0.0019342060 -0.0006095160
0.0021617994 -0.0006564228
0.0023893927 -0.0007033297
0.0026169861 -0.0007502366
0.0028445794 -0.0007971434
0.0025901695 -0.0007596842
0.0023357595 -0.0007222250
0.0020813495 -0.0006847658
0.0018269395 -0.0006473066
0.0015725295 -0.0006098474
0.0013181196 -0.0005723882
0.0010637096 -0.0005349290
0.0008092997 -0.0004974698
0.0004394165 -0.0004301945
0.0000695332 -0.0003629191
-0.0003003500 -0.0002956437
-0.0006702333 -0.0002283684
-0.0010401165 -0.0001610930
-0.0014099997 -0.0000938176
-0.0017798829 -0.0000265423
-0.0021497661 0.0000407331
-0.0025731586 0.0001387833
-0.0029965512 0.0002368336
-0.0034199437 0.0003348838
-0.0038433362 0.0004329340
-0.0042667287 0.0005309842
-0.0046901213 0.0006290344
-0.0051135135 0.0007270847
-0.0055369061 0.0008251349
-0.0058081238 0.0009517146
-0.0060793415 0.0010782942
-0.0063505591 0.0012048739
-0.0066217768 0.0013314536
-0.0068929945 0.0014580334
-0.0071642122 0.0015846131
-0.0074354299 0.0017111929
-0.0077066476 0.0018377726
-0.0075041498 0.0019664642
-0.0073016520 0.0020951558
-0.0070991542 0.0022238474
-0.0068966564 0.0023525392
-0.0066941586 0.0024812309
-0.0064916607 0.0026099226
-0.0062891629 0.0027386144
-0.0060866651 0.0028673061
-0.0056080852 0.0027505508
-0.0051295053 0.0026337955
-0.0046509253 0.0025170401
-0.0041723454 0.0024002848
-0.0036937655 0.0022835295
-0.0032151856 0.0021667741
-0.0027366057 0.0020500188
-0.0022580257 0.0019332635
-0.0020025854 0.0018888931
-0.0017471450 0.0018445226
-0.0014917046 0.0018001522
-0.0012362643 0.0017557818
-0.0009808238 0.0017114114
-0.0007253834 0.0016670410
-0.0004699430 0.0016226705
-0.0002145025 0.0015783001
-0.0002881384 0.0015376503
-0.0003617742 0.0014970005
-0.0004354101 0.0014563506
-0.0005090460 0.0014157008
-0.0005826818 0.0013750510
-0.0006563177 0.0013344012
-0.0007299535 0.0012937513
-0.0008035894 0.0012531015
-0.0012285071 0.0012115226
-0.0016534248 0.0011699436
-0.0020783425 0.0011283647
-0.0025032602 0.0010867857
-0.0029281779 0.0010452068
-0.0033530956 0.0010036278
-0.0037780133 0.0009620489
-0.0042029310 0.0009204699
-0.0040303020 0.0009621728
-0.0038576731 0.0010038758
-0.0036850442 0.0010455787
-0.0035124152 0.0010872816
-0.0033397863 0.0011289846
-0.0031671574 0.0011706876
-0.0029945285 0.0012123907
-0.0028218995 0.0012540937
-0.0027037047 0.0011740516
-0.0025855098 0.0010940095
-0.0024673149 0.0010139675
-0.0023491200 0.0009339254
-0.0022309252 0.0008538833
-0.0021127303 0.0007738413
-0.0019945354 0.0006937992
-0.0018763405 0.0006137571
-0.0015314777 0.0004001644
-0.0011866149 0.0001865717
-0.0008417520 -0.0000270210
-0.0004968892 -0.0002406137
-0.0001520264 -0.0004542064
0.0001928365 -0.0006677991
0.0005376993 -0.0008813919
0.0008825621 -0.0010949846
0.0010642487 -0.0011905569
0.0012459353 -0.0012861292
0.0014276218 -0.0013817015
0.0016093084 -0.0014772739
0.0017909951 -0.0015728462
0.0019726817 -0.0016684186
0.0021543684 -0.0017639909
0.0023360550 -0.0018595632
0.0027153753 -0.0017733051
0.0030946957 -0.0016870471
0.0034740160 -0.0016007890
0.0038533363 -0.0015145309
0.0042326566 -0.0014282728
0.0046119767 -0.0013420147
0.0049912970 -0.0012557566
0.0053706173 -0.0011694985
0.0050153740 -0.0009768545
0.0046601307 -0.0007842106
0.0043048874 -0.0005915666
0.0039496441 -0.0003989227
0.0035944008 -0.0002062787
0.0032391575 -0.0000136347
0.0028839142 0.0001790092
0.0025286709 0.0003716532
0.0021404813 0.0004761597
0.0017522917 0.0005806662
0.0013641021 0.0006851727
0.0009759127 0.0007896793
0.0005877232 0.0008941858
0.0001995337 0.0009986923
-0.0001886558 0.0011031989
-0.0005768453 0.0012077054
-0.0009321740 0.0012155976
-0.0012875026 0.0012234897
-0.0016428311 0.0012313819
-0.0019981597 0.0012392740
-0.0023534883 0.0012471662
-0.0027088169 0.0012550583
-0.0030641454 0.0012629505
-0.0034194740 0.0012708426
-0.0036166907 0.0011192895
-0.0038139075 0.0009677364
-0.0040111242 0.0008161833
-0.0042083409 0.0006646302
-0.0044055576 0.0005130771
-0.0046027744 0.0003615240
-0.0047999914 0.0002099708
-0.0049972081 0.0000584177
-0.0045551598 0.0001448951
-0.0041131115 0.0002313726
-0.0036710633 0.0003178500
-0.0032290150 0.0004043274
-0.0027869667 0.0004908048
-0.0023449183 0.0005772822
-0.0019028699 0.0006637596
-0.0014608215 0.0007502371
-0.0012215369 0.0007154485
-0.0009822522 0.0006806600
-0.0007429676 0.0006458714
-0.0005036829 0.0006110829
-0.0002643982 0.0005762943
-0.0000251136 0.0005415058
0.0002141711 0.0005067172
0.0004534558 0.0004719287
0.0008549439 0.0004279950
0.0012564322 0.0003840613
0.0016579204 0.0003401276
0.0020594086 0.0002961939
0.0024608969 0.0002522602
0.0028623853 0.0002083265
0.0032638736 0.0001643928
0.0036653619 0.0001204591
0.0039340492 0.0000226667
0.0042027364 -0.0000751258
0.0044714237 -0.0001729182
0.0047401109 -0.0002707107
0.0050087982 -0.0003685031
0.0052774854 -0.0004662956
0.0055461727 -0.0005640881
0.0058148599 -0.0006618805
0.0058788589 -0.0006868977
0.0059428579 -0.0007119150
0.0060068568 -0.0007369322
0.0060708558 -0.0007619494
0.0061348547 -0.0007869666
0.0061988537 -0.0008119838
0.0062628527 -0.0008370010
0.0063268516 -0.0008620182
0.0061366611 -0.0007651691
0.0059464706 -0.0006683200
0.0057562800 -0.0005714709
0.0055660895 -0.0004746218
0.0053758990 -0.0003777727
0.0051857084 -0.0002809236
0.0049955179 -0.0001840745
0.0048053274 -0.0000872255
0.0043251224 0.0000057956
0.0038449174 0.0000988166
0.0033647124 0.0001918376
0.0028845074 0.0002848586
0.0024043025 0.0003778796
0.0019240975 0.0004709007
0.0014438925 0.0005639217
0.0009636875 0.0006569427
0.0006304273 0.0006581738
0.0002971672 0.0006594049
-0.0000360930 0.0006606360
-0.0003693531 0.0006618670
-0.0007026133 0.0006630981
-0.0010358735 0.0006643292
-0.0013691336 0.0006655603
-0.0017023938 0.0006667914
-0.0016914594 0.0007122871
-0.0016805249 0.0007577828
-0.0016695905 0.0008032785
-0.0016586561 0.0008487742
-0.0016477216 0.0008942699
-0.0016367872 0.0009397656
-0.0016258528 0.0009852613
-0.0016149183 0.0010307570


==> data/gru_sample62.tex <==
-0.0573203197 -0.0008144872
-0.0509108116 -0.0011422796
-0.0445013034 -0.0014700721
-0.0380917953 -0.0017978645
-0.0316822850 -0.0021256569
-0.0252727746 -0.0024534493
-0.0188632643 -0.0027812416
-0.0124537540 -0.0031090341
-0.0107137672 -0.0028867598
-0.0089737799 -0.0026644855
-0.0072337925 -0.0024422112
-0.0054938052 -0.0022199368
-0.0037538179 -0.0019976625
-0.0020138305 -0.0017753882
-0.0002738432 -0.0015531139
0.0014661441 -0.0013308396
0.0013312994 -0.0014898757
0.0011964546 -0.0016489117
0.0010616100 -0.0018079477
0.0009267653 -0.0019669837
0.0007919206 -0.0021260198
0.0006570759 -0.0022850558
0.0005222312 -0.0024440918
0.0003873866 -0.0026031278
0.0005498084 -0.0033953275
0.0007122303 -0.0041875271
0.0008746522 -0.0049797267
0.0010370741 -0.0057719263
0.0011994960 -0.0065641259
0.0013619179 -0.0073563256
0.0015243398 -0.0081485252
0.0016867617 -0.0089407248
0.0024857350 -0.0101482913
0.0032847082 -0.0113558578
0.0040836814 -0.0125634243
0.0048826546 -0.0137709908
0.0056816278 -0.0149785573
0.0064806010 -0.0161861238
0.0072795742 -0.0173936904
0.0080785474 -0.0186012569
0.0121599585 -0.0196123024
0.0162413695 -0.0206233480
0.0203227795 -0.0216343935
0.0244041916 -0.0226454391
0.0284856038 -0.0236564846
0.0325670159 -0.0246675302
0.0366484281 -0.0256785757
0.0407298402 -0.0266896213
0.0441830799 -0.0285367778
0.0476363196 -0.0303839342
0.0510895594 -0.0322310907
0.0545427991 -0.0340782471
0.0579960388 -0.0359254036
0.0614492785 -0.0377725600
0.0649025182 -0.0396197165
0.0683557579 -0.0414668752
0.0672004763 -0.0454727544
0.0660451946 -0.0494786337
0.0648899129 -0.0534845129
0.0637346312 -0.0574903922
0.0625793496 -0.0614962714
0.0614240679 -0.0655021507
0.0602687862 -0.0695080299
0.0591135046 -0.0735139092
0.0615749651 -0.0787546815
0.0640364256 -0.0839954538
0.0664978862 -0.0892362261
0.0689593467 -0.0944769984
0.0714208073 -0.0997177707
0.0738822678 -0.1049585430
0.0763437283 -0.1101993154
0.0788051933 -0.1154400877
0.0777832938 -0.1219472624
0.0767613944 -0.1284544372
0.0757394949 -0.1349616120
0.0747175955 -0.1414687868
0.0736956960 -0.1479759616
0.0726737966 -0.1544831454
0.0716518971 -0.1609903292
0.0706299977 -0.1674975130
0.0665579016 -0.1748881868
0.0624858054 -0.1822788606
0.0584137093 -0.1896695344
0.0543416131 -0.1970602083
0.0502695170 -0.2044508821
0.0461974208 -0.2118415559
0.0421253247 -0.2192322297
0.0380532285 -0.2266229035
0.0337225581 -0.2359066311
0.0293918876 -0.2451903586
0.0250612172 -0.2544740862
0.0207305467 -0.2637578137
0.0163998774 -0.2730415412
0.0120692080 -0.2823252688
0.0077385387 -0.2916089963
0.0034078693 -0.3008927238
-0.0034458814 -0.3100255672
-0.0102996322 -0.3191584105
-0.0171533823 -0.3282912538
-0.0240071336 -0.3374240971
-0.0308608849 -0.3465569405
-0.0377146340 -0.3556897838
-0.0445683831 -0.3648226271
-0.0514221322 -0.3739554704
-0.0588331726 -0.3808615717
-0.0662442130 -0.3877676730
-0.0736552534 -0.3946737743
-0.0810662894 -0.4015798756
-0.0884773254 -0.4084859769
-0.0958883614 -0.4153920782
-0.1032993973 -0.4222981795
-0.1107104333 -0.4292042808
-0.1213878459 -0.4347413091
-0.1320652584 -0.4402783374
-0.1427426710 -0.4458153657
-0.1534200836 -0.4513523940
-0.1640974961 -0.4568894222
-0.1747749087 -0.4624264505
-0.1854523212 -0.4679634788
-0.1961297338 -0.4735005071
-0.2091177273 -0.4771875888
-0.2221057209 -0.4808746706
-0.2350937145 -0.4845617524
-0.2480817080 -0.4882488341
-0.2610697016 -0.4919359159
-0.2740576952 -0.4956229977
-0.2870456887 -0.4993100794
-0.3000336999 -0.5029971612
-0.3062319246 -0.5035986410
-0.3124301493 -0.5042001209
-0.3186283740 -0.5048016007
-0.3248265987 -0.5054030805
-0.3310248233 -0.5060045603
-0.3372230480 -0.5066060401
-0.3434212727 -0.5072075200
-0.3496194974 -0.5078089998
-0.3484186423 -0.5062575738
-0.3472177873 -0.5047061477
-0.3460169323 -0.5031547217
-0.3448160772 -0.5016032957
-0.3436152222 -0.5000518697
-0.3424143672 -0.4985004437
-0.3412135121 -0.4969490176
-0.3400126571 -0.4953975916
-0.3382666878 -0.4876381519
-0.3365207538 -0.4798787121
-0.3347748197 -0.4721192724
-0.3330288857 -0.4643598326
-0.3312829517 -0.4566003929
-0.3295370177 -0.4488409532
-0.3277910837 -0.4410815134
-0.3260451497 -0.4333220737
-0.3187412963 -0.4188164028
-0.3114374429 -0.4043107319
-0.3041335896 -0.3898050610
-0.2968297362 -0.3752993901
-0.2895258828 -0.3607937192
-0.2822220294 -0.3462880483
-0.2749181761 -0.3317823774
-0.2676143227 -0.3172767065
-0.2529781823 -0.2998483171
-0.2383420418 -0.2824199278
-0.2237059014 -0.2649915384
-0.2090697610 -0.2475631491
-0.1944336205 -0.2301347597
-0.1797974801 -0.2127063703
-0.1651613397 -0.1952779810
-0.1505251992 -0.1778495916
-0.1373840523 -0.1666283499
-0.1242429054 -0.1554071081
-0.1111017585 -0.1441858754
-0.0979606116 -0.1329646427
-0.0848194647 -0.1217434100
-0.0716783178 -0.1105221772
-0.0585371709 -0.0993009445
-0.0453960240 -0.0880797118
-0.0354758922 -0.0819281218
-0.0255557604 -0.0757765317
-0.0156356286 -0.0696249417
-0.0057154968 -0.0634733517
0.0042046349 -0.0573217617
0.0141247667 -0.0511701716
0.0240448985 -0.0450185816
0.0339650303 -0.0388669916
0.0366750317 -0.0352675001
0.0393850330 -0.0316680085
0.0420950366 -0.0280685170
0.0448050402 -0.0244690255
0.0475150438 -0.0208695340
0.0502250474 -0.0172700425
0.0529350510 -0.0136705510
0.0556450546 -0.0100710595
0.0553237054 -0.0087220413
0.0550023562 -0.0073730231
0.0546810071 -0.0060240049
0.0543596579 -0.0046749867
0.0540383087 -0.0033259685
0.0537169596 -0.0019769504
0.0533956104 -0.0006279323
0.0530742612 0.0007210857
0.0517190034 0.0012159660
0.0503637455 0.0017108462
0.0490084876 0.0022057264
0.0476532297 0.0027006066
0.0462979719 0.0031954868
0.0449427140 0.0036903669
0.0435874561 0.0041852471
0.0422321982 0.0046801276
0.0400089757 0.0052034722
0.0377857533 0.0057268169
0.0355625285 0.0062501615
0.0333393038 0.0067735062
0.0311160791 0.0072968508
0.0288928544 0.0078201955
0.0266696297 0.0083435401
0.0244464050 0.0088668847
0.0238973480 0.0090194149
0.0233482910 0.0091719451
0.0227992339 0.0093244752
0.0222501769 0.0094770054
0.0217011198 0.0096295361
0.0211520628 0.0097820669
0.0206030058 0.0099345976
0.0200539487 0.0100871283
0.0194246725 0.0101351018
0.0187953963 0.0101830752
0.0181661212 0.0102310487
0.0175368460 0.0102790221
0.0169075709 0.0103269955
0.0162782958 0.0103749690
0.0156490207 0.0104229424
0.0150197455 0.0104709159
0.0148437669 0.0103047721
0.0146677882 0.0101386282
0.0144918096 0.0099724844
0.0143158309 0.0098063406
0.0141398522 0.0096401968
0.0139638736 0.0094740529
0.0137878949 0.0093079097
0.0136119163 0.0091417664
0.0136944071 0.0088996008
0.0137768978 0.0086574352
0.0138593886 0.0084152696
0.0139418794 0.0081731040
0.0140243702 0.0079309385
0.0141068610 0.0076887729
0.0141893518 0.0074466073
0.0142718426 0.0072044417
0.0147269548 0.0069726396
0.0151820670 0.0067408374
0.0156371792 0.0065090353
0.0160922914 0.0062772332
0.0165474036 0.0060454311
0.0170025158 0.0058136290
0.0174576280 0.0055818269
0.0179127402 0.0053500247
0.0178790668 0.0054466579
0.0178453934 0.0055432910
0.0178117200 0.0056399241
0.0177780467 0.0057365573
0.0177443733 0.0058331904
0.0177106999 0.0059298235
0.0176770265 0.0060264567
0.0176433531 0.0061230898
0.0168868936 0.0058892775
0.0161304340 0.0056554651
0.0153739745 0.0054216528
0.0146175149 0.0051878405
0.0138610554 0.0049540281
0.0131045958 0.0047202158
0.0123481363 0.0044864035
0.0115916767 0.0042525911
0.0109469551 0.0041910677
0.0103022335 0.0041295444
0.0096575119 0.0040680210
0.0090127904 0.0040064976
0.0083680688 0.0039449742
0.0077233472 0.0038834508
0.0070786256 0.0038219274
0.0064339040 0.0037604040
0.0058969042 0.0037566734
0.0053599045 0.0037529428
0.0048229047 0.0037492122
0.0042859049 0.0037454816
0.0037489052 0.0037417510
0.0032119054 0.0037380204
0.0026749056 0.0037342898
0.0021379059 0.0037305592
0.0016411429 0.0036170645
0.0011443799 0.0035035698
0.0006476170 0.0033900750
0.0001508540 0.0032765803
-0.0003459089 0.0031630856
-0.0008426719 0.0030495909
-0.0013394349 0.0029360962
-0.0018361978 0.0028226015
-0.0020291390 0.0025886346
-0.0022220802 0.0023546678
-0.0024150214 0.0021207009
-0.0026079626 0.0018867341
-0.0028009038 0.0016527673
-0.0029938449 0.0014188004
-0.0031867861 0.0011848336
-0.0033797273 0.0009508667
-0.0033653733 0.0007408238
-0.0033510193 0.0005307808
-0.0033366653 0.0003207379
-0.0033223114 0.0001106949
-0.0033079574 -0.0000993480
-0.0032936034 -0.0003093910
-0.0032792494 -0.0005194339
-0.0032648954 -0.0007294769
-0.0030940066 -0.0008319757
-0.0029231178 -0.0009344745
-0.0027522290 -0.0010369732
-0.0025813402 -0.0011394720
-0.0024104514 -0.0012419708
-0.0022395626 -0.0013444695
-0.0020686738 -0.0014469682
-0.0018977850 -0.0015494669
-0.0016593268 -0.0014993757
-0.0014208685 -0.0014492845
-0.0011824103 -0.0013991933
-0.0009439520 -0.0013491020
-0.0007054937 -0.0012990108
-0.0004670355 -0.0012489196
-0.0002285772 -0.0011988284
0.0000098810 -0.0011487371
0.0016013835 -0.0009770045
0.0031928860 -0.0008052718
0.0047843884 -0.0006335391
0.0063758909 -0.0004618063
0.0079673934 -0.0002900736
0.0095588959 -0.0001183409
0.0111503983 0.0000533918
0.0127419008 0.0002251245
0.0139409456 0.0002173505
0.0151399904 0.0002095766
0.0163390353 0.0002018026
0.0175380801 0.0001940286
0.0187371249 0.0001862546
0.0199361697 0.0001784806
0.0211352145 0.0001707066
0.0223342593 0.0001629327
0.0211119952 0.0006591483
0.0198897310 0.0011553640
0.0186674668 0.0016515798
0.0174452026 0.0021477955
0.0162229384 0.0026440112
0.0150006742 0.0031402269
0.0137784100 0.0036364426
0.0125561459 0.0041326584
0.0116732977 0.0045073585
0.0107904496 0.0048820589
0.0099076014 0.0052567591
0.0090247532 0.0056314592
0.0081419051 0.0060061594
0.0072590569 0.0063808595
0.0063762088 0.0067555597
0.0054933606 0.0071302598
0.0128094087 0.0058888489
0.0201254568 0.0046474380
0.0274415049 0.0034060271
0.0347575529 0.0021646160
0.0420736010 0.0009232050
0.0493896491 -0.0003182061
0.0567056971 -0.0015596171
0.0640217452 -0.0028010280
0.0680830992 -0.0030043564
0.0721444533 -0.0032076847
0.0762058073 -0.0034110131
0.0802671614 -0.0036143414
0.0843285154 -0.0038176698
0.0883898694 -0.0040209981
0.0924512235 -0.0042243265
0.0965125775 -0.0044276548
0.0967395790 -0.0046587515
0.0969665804 -0.0048898482
0.0971935819 -0.0051209449
0.0974205833 -0.0053520417
0.0976475848 -0.0055831384
0.0978745862 -0.0058142351
0.0981015876 -0.0060453318
0.0983285891 -0.0062764285
0.1017947697 -0.0070709930
0.1052609502 -0.0078655575
0.1087271308 -0.0086601220
0.1121933114 -0.0094546865
0.1156594919 -0.0102492511
0.1191256725 -0.0110438156
0.1225918531 -0.0118383801
0.1260580337 -0.0126329446
0.1342993861 -0.0130592868
0.1425407386 -0.0134856289
0.1507820911 -0.0139119711
0.1590234436 -0.0143383133
0.1672647960 -0.0147646555
0.1755061485 -0.0151909976
0.1837475010 -0.0156173398
0.1919888535 -0.0160436820
0.2003949447 -0.0147735094
0.2088010359 -0.0135033369
0.2172071271 -0.0122331644
0.2256132183 -0.0109629918
0.2340193096 -0.0096928193
0.2424254008 -0.0084226468
0.2508314920 -0.0071524742
0.2592375832 -0.0058823017
0.2666443453 -0.0065843127
0.2740511075 -0.0072863237
0.2814578696 -0.0079883348
0.2888646317 -0.0086903458
0.2962713938 -0.0093923568
0.3036781382 -0.0100943678
0.3110848827 -0.0107963789
0.3184916271 -0.0114983899
0.3310028002 -0.0116339130
0.3435139733 -0.0117694361
0.3560251464 -0.0119049592
0.3685363195 -0.0120404823
0.3810474926 -0.0121760054
0.3935586656 -0.0123115285
0.4060698387 -0.0124470516
0.4185810118 -0.0125825747
0.4405592233 -0.0132964395
0.4625374348 -0.0140103043
0.4845156463 -0.0147241692
0.5064938578 -0.0154380340
0.5284720693 -0.0161518988
0.5504502808 -0.0168657637
0.5724284923 -0.0175796285
0.5944066685 -0.0182934933
0.6168805797 -0.0184737780
0.6393544910 -0.0186540627
0.6618284022 -0.0188343474
0.6843023135 -0.0190146321
0.7067762247 -0.0191949169
0.7292501359 -0.0193752016
0.7517240472 -0.0195554863
0.7741979584 -0.0197357710
0.7965882287 -0.0187911342
0.8189784990 -0.0178464975
0.8413687693 -0.0169018607
0.8637590396 -0.0159572240
0.8861493099 -0.0150125873
0.9085395802 -0.0140679505
0.9309298505 -0.0131233138
0.9533201208 -0.0121786770
0.9719510698 -0.0115204544
0.9905820189 -0.0108622317
1.0092129679 -0.0102040090
1.0278439170 -0.0095457858
1.0464748661 -0.0088875626
1.0651058151 -0.0082293393
1.0837367642 -0.0075711161
1.1023677133 -0.0069128929
1.1214881455 -0.0091027862
1.1406085777 -0.0112926800
1.1597290100 -0.0134825739
1.1788494422 -0.0156724677
1.1979699451 -0.0178623616
1.2170903773 -0.0200522543
1.2362108096 -0.0222421482
1.2553312418 -0.0244320420
1.2725273673 -0.0280037232
1.2897234927 -0.0315754043
1.3069196182 -0.0351470855
1.3241157436 -0.0387187644
1.3413118691 -0.0422904455
1.3585079945 -0.0458621267
1.3757041200 -0.0494338078
1.3929002454 -0.0530054889
1.3997012995 -0.0545010912
1.4065023535 -0.0559966935
1.4133034076 -0.0574922958
1.4201044616 -0.0589878981
1.4269055157 -0.0604835004
1.4337065697 -0.0619791027
1.4405076238 -0.0634747050
1.4473086778 -0.0649703073
1.4406048281 -0.0680358849
1.4339009784 -0.0711014624
1.4271971287 -0.0741670400
1.4204932790 -0.0772326131
1.4137894292 -0.0802981862
1.4070855795 -0.0833637592
1.4003817298 -0.0864293323
1.3936778801 -0.0894949054
1.3807446170 -0.0937040010
1.3678113538 -0.0979130967
1.3548780907 -0.1021221924
1.3419448275 -0.1063312880
1.3290115644 -0.1105403837
1.3160783013 -0.1147494793
1.3031450381 -0.1189585750
1.2902117750 -0.1231676707
1.2711780920 -0.1258862931
1.2521444089 -0.1286049154
1.2331107259 -0.1313235378
1.2140770429 -0.1340421602
1.1950433599 -0.1367607826
1.1760096768 -0.1394794050
1.1569759938 -0.1421980274
1.1379423108 -0.1449166498
1.1143163586 -0.1437941124
1.0906904065 -0.1426715750
1.0670644543 -0.1415490376
1.0434385021 -0.1404265002
1.0198125499 -0.1393039629
0.9961865977 -0.1381814255
0.9725606456 -0.1370588881
0.9489346934 -0.1359363507
0.9236891163 -0.1328638848
0.8984435393 -0.1297914189
0.8731979622 -0.1267189530
0.8479523851 -0.1236464871
0.8227068081 -0.1205740213
0.7974612310 -0.1175015554
0.7722156540 -0.1144290895
0.7469700769 -0.1113566236
0.7258950321 -0.1110860984
0.7048199874 -0.1108155732
0.6837449427 -0.1105450481
0.6626698979 -0.1102745229
0.6415948532 -0.1100039977
0.6205198084 -0.1097334725
0.5994447637 -0.1094629474
0.5783697189 -0.1091924222
0.5544369302 -0.1054425742
0.5305041415 -0.1016927263
0.5065713528 -0.0979428784
0.4826385642 -0.0941930304
0.4587057755 -0.0904431825
0.4347729868 -0.0866933346
0.4108401981 -0.0829434866
0.3869074094 -0.0791936387
0.3676192008 -0.0770598505
0.3483309922 -0.0749260578
0.3290427835 -0.0727922651
0.3097545749 -0.0706584724
0.2904663663 -0.0685246797
0.2711781577 -0.0663908870
0.2518899491 -0.0642570943
0.2326017404 -0.0621233016
0.2221899267 -0.0626310381
0.2117781130 -0.0631387747
0.2013662993 -0.0636465113
0.1909544856 -0.0641542478
0.1805426719 -0.0646619844
0.1701308582 -0.0651697209
0.1597190444 -0.0656774575
0.1493072307 -0.0661851940
0.1477752911 -0.0658870074
0.1462433514 -0.0655888207
0.1447114118 -0.0652906340
0.1431794721 -0.0649924473
0.1416475325 -0.0646942606
0.1401155928 -0.0643960740
0.1385836532 -0.0640978873
0.1370517135 -0.0637997006
0.1401710650 -0.0601660833
0.1432904165 -0.0565324660
0.1464097679 -0.0528988487
0.1495291194 -0.0492652314
0.1526484709 -0.0456316141
0.1557678224 -0.0419979968
0.1588871738 -0.0383643795
0.1620065253 -0.0347307645
0.1615429856 -0.0313074752
0.1610794460 -0.0278841882
0.1606159063 -0.0244609012
0.1601523667 -0.0210376142
0.1596888270 -0.0176143260
0.1592252874 -0.0141910379
0.1587617477 -0.0107677497
0.1582982081 -0.0073444616
0.1553103226 -0.0044938860
0.1523224372 -0.0016433104
0.1493345518 0.0012072652
0.1463466664 0.0040578407
0.1433587809 0.0069084163
0.1403708955 0.0097589919
0.1373830101 0.0126095669
0.1343951246 0.0154601431
0.1278697360 0.0186812242
0.1213443474 0.0219023052
0.1148189588 0.0251233863
0.1082935701 0.0283444673
0.1017681815 0.0315655484
0.0952427929 0.0347866295
0.0887174043 0.0380077105
0.0821920156 0.0412287916
0.0735874979 0.0433688365
0.0649829802 0.0455088815
0.0563784625 0.0476489265
0.0477739448 0.0497889714
0.0391694271 0.0519290164
0.0305649094 0.0540690613
0.0219603917 0.0562091063
0.0133558729 0.0583491512
0.0067656189 0.0587093417
0.0001753648 0.0590695322
-0.0064148892 0.0594297227
-0.0130051433 0.0597899132
-0.0195953985 0.0601501037
-0.0261856525 0.0605102942
-0.0327759066 0.0608704847
-0.0393661585 0.0612306752
-0.0400992706 0.0588486011
-0.0408323828 0.0564665270
-0.0415654949 0.0540844529
-0.0422986070 0.0517023788
-0.0430317192 0.0493203047
-0.0437648313 0.0469382306
-0.0444979435 0.0445561565
-0.0452310556 0.0421740824
-0.0421027414 0.0401906236
-0.0389744271 0.0382071648
-0.0358461128 0.0362237059
-0.0327177986 0.0342402471
-0.0295894843 0.0322567883
-0.0264611701 0.0302733294
-0.0233328558 0.0282898706
-0.0202045415 0.0263064118
-0.0182327331 0.0249047715
-0.0162609246 0.0235031313
-0.0142891161 0.0221014911
-0.0123173076 0.0206998508
-0.0103454991 0.0192982106
-0.0083736906 0.0178965703
-0.0064018822 0.0164949301
-0.0044300737 0.0150932898
-0.0029081730 0.0143690576
-0.0013862724 0.0136448253
0.0001356283 0.0129205931
0.0016575290 0.0121963608
0.0031794296 0.0114721286
0.0047013303 0.0107478963
0.0062232310 0.0100236641
0.0077451316 0.0092994318
0.0073984350 0.0093220274
0.0070517383 0.0093446231
0.0067050417 0.0093672187
0.0063583450 0.0093898144
0.0060116484 0.0094124100
0.0056649517 0.0094350057
0.0053182551 0.0094576013
0.0049715584 0.0094801969
0.0047009870 0.0094237721
0.0044304156 0.0093673473
0.0041598442 0.0093109225
0.0038892727 0.0092544977
0.0036187013 0.0091980728
0.0033481299 0.0091416480
0.0030775585 0.0090852232
0.0028069870 0.0090287984
0.0030591279 0.0088697577
0.0033112688 0.0087107170
0.0035634096 0.0085516763
0.0038155505 0.0083926357
0.0040676913 0.0082335950
0.0043198322 0.0080745543
0.0045719730 0.0079155136
0.0048241139 0.0077564729
0.0045911553 0.0078172746
0.0043581967 0.0078780762
0.0041252381 0.0079388778
0.0038922795 0.0079996795
0.0036593209 0.0080604811
0.0034263622 0.0081212827
0.0031934036 0.0081820843
0.0029604450 0.0082428860
0.0023486689 0.0083610067
0.0017368927 0.0084791275
0.0011251166 0.0085972482
0.0005133404 0.0087153690
-0.0000984358 0.0088334897
-0.0007102119 0.0089516105
-0.0013219881 0.0090697313
-0.0019337642 0.0091878520
-0.0021489739 0.0091596999
-0.0023641835 0.0091315479
-0.0025793931 0.0091033958
-0.0027946028 0.0090752437
-0.0030098124 0.0090470916
-0.0032250220 0.0090189396
-0.0034402317 0.0089907875
-0.0036554413 0.0089626354
-0.0042491180 0.0091458432
-0.0048427947 0.0093290511
-0.0054364715 0.0095122589
-0.0060301482 0.0096954668
-0.0066238249 0.0098786746
-0.0072175017 0.0100618825
-0.0078111784 0.0102450903
-0.0084048551 0.0104282981
-0.0089366533 0.0106419203
-0.0094684514 0.0108555425
-0.0100002496 0.0110691647
-0.0105320477 0.0112827869
-0.0110638458 0.0114964091
-0.0115956440 0.0117100313
-0.0121274421 0.0119236534
-0.0126592403 0.0121372756
-0.0127099772 0.0121181140
-0.0127607141 0.0120989524
-0.0128114510 0.0120797907
-0.0128621879 0.0120606291
-0.0129129248 0.0120414675
-0.0129636617 0.0120223058
-0.0130143986 0.0120031442
-0.0130651355 0.0119839825
-0.0127849501 0.0118969584
-0.0125047646 0.0118099343
-0.0122245791 0.0117229102
-0.0119443937 0.0116358861
-0.0116642082 0.0115488620
-0.0113840228 0.0114618378
-0.0111038373 0.0113748137
-0.0108236519 0.0112877896
-0.0106782306 0.0111592236
-0.0105328093 0.0110306576
-0.0103873880 0.0109020916
-0.0102419668 0.0107735256
-0.0100965455 0.0106449596
-0.0099511242 0.0105163936
-0.0098057029 0.0103878276
-0.0096602816 0.0102592616
-0.0095153217 0.0101487577
-0.0093703618 0.0100382538
-0.0092254019 0.0099277499
-0.0090804420 0.0098172460
-0.0089354821 0.0097067420
-0.0087905222 0.0095962381
-0.0086455623 0.0094857342
-0.0085006024 0.0093752303
-0.0083549913 0.0090903996
-0.0082093802 0.0088055689
-0.0080637690 0.0085207381
-0.0079181579 0.0082359074
-0.0077725468 0.0079510767
-0.0076269356 0.0076662460
-0.0074813245 0.0073814153
-0.0073357134 0.0070965846
-0.0071772574 0.0070487414
-0.0070188014 0.0070008982
-0.0068603455 0.0069530550
-0.0067018895 0.0069052118
-0.0065434336 0.0068573686
-0.0063849776 0.0068095254
-0.0062265216 0.0067616822
-0.0060680657 0.0067138391
-0.0059044042 0.0067417030
-0.0057407428 0.0067695669
-0.0055770813 0.0067974309
-0.0054134199 0.0068252948
-0.0052497584 0.0068531587
-0.0050860970 0.0068810227
-0.0049224355 0.0069088866
-0.0047587741 0.0069367505
-0.0046704067 0.0069430118
-0.0045820393 0.0069492731
-0.0044936720 0.0069555344
-0.0044053046 0.0069617957
-0.0043169372 0.0069680569
-0.0042285698 0.0069743182
-0.0041402025 0.0069805795
-0.0040518351 0.0069868408
-0.0038623032 0.0070896489
-0.0036727714 0.0071924571
-0.0034832395 0.0072952652
-0.0032937077 0.0073980733
-0.0031041758 0.0075008815
-0.0029146440 0.0076036896
-0.0027251122 0.0077064977
-0.0025355803 0.0078093059
-0.0029409060 0.0079792254
-0.0033462316 0.0081491450
-0.0037515573 0.0083190645
-0.0041568830 0.0084889840
-0.0045622086 0.0086589036
-0.0049675343 0.0088288231
-0.0053728599 0.0089987426
-0.0057781856 0.0091686622
-0.0067617857 0.0093662387
-0.0077453858 0.0095638152
-0.0087289858 0.0097613918
-0.0097125859 0.0099589683
-0.0106961860 0.0101565448
-0.0116797861 0.0103541214
-0.0126633861 0.0105516979
-0.0136469862 0.0107492744
-0.0162183359 0.0115944073
-0.0187896855 0.0124395403
-0.0213610352 0.0132846732
-0.0239323848 0.0141298061
-0.0265037345 0.0149749390
-0.0290750841 0.0158200719
-0.0316464338 0.0166652049
-0.0342177835 0.0175103378
-0.0388978063 0.0198113581
-0.0435778269 0.0221123784
-0.0482578475 0.0244133987
-0.0529378681 0.0267144190
-0.0576178888 0.0290154392
-0.0622979094 0.0313164595
-0.0669779300 0.0336174798
-0.0716579506 0.0359185001
-0.0779627795 0.0384142832
-0.0842676040 0.0409100663
-0.0905724285 0.0434058494
-0.0968772530 0.0459016325
-0.1031820775 0.0483974155
-0.1094869020 0.0508931986
-0.1157917265 0.0533889817
-0.1220965510 0.0558847648
-0.1229604669 0.0569537069
-0.1238243828 0.0580226490
-0.1246882987 0.0590915911
-0.1255522146 0.0601605331
-0.1264161305 0.0612294752
-0.1272800465 0.0622984173
-0.1281439624 0.0633673594
-0.1290078783 0.0644363015
-0.1277568139 0.0639685460
-0.1265057496 0.0635007905
-0.1252546853 0.0630330351
-0.1240036210 0.0625652796
-0.1227525566 0.0620975241
-0.1215014923 0.0616297686
-0.1202504280 0.0611620131
-0.1189993637 0.0606942576
-0.1175980335 0.0585590440
-0.1161967034 0.0564238303
-0.1147953732 0.0542886166
-0.1133940431 0.0521534030
-0.1119927129 0.0500181893
-0.1105913828 0.0478829756
-0.1091900526 0.0457477620
-0.1077887224 0.0436125483
-0.1036609378 0.0397782453
-0.0995331531 0.0359439422
-0.0954053685 0.0321096392
-0.0912775838 0.0282753361
-0.0871497992 0.0244410331
-0.0830220145 0.0206067301
-0.0788942298 0.0167724270
-0.0747664452 0.0129381240
-0.0698529152 0.0103143365
-0.0649393851 0.0076905491
-0.0600258551 0.0050667616
-0.0551123251 0.0024429744
-0.0501987951 -0.0001808127
-0.0452852651 -0.0028045999
-0.0403717350 -0.0054283871
-0.0354582050 -0.0080521745
-0.0324710746 -0.0083011332
-0.0294839442 -0.0085500918
-0.0264968137 -0.0087990504
-0.0235096833 -0.0090480090
-0.0205225528 -0.0092969676
-0.0175354224 -0.0095459262
-0.0145482920 -0.0097948842
-0.0115611615 -0.0100438423
-0.0101689222 -0.0092100839
-0.0087766829 -0.0083763255
-0.0073844436 -0.0075425670
-0.0059922042 -0.0067088086
-0.0045999649 -0.0058750502
-0.0032077256 -0.0050412918
-0.0018154864 -0.0042075331
-0.0004232472 -0.0033737744
-0.0010137790 -0.0027836353
-0.0016043107 -0.0021934961
-0.0021948425 -0.0016033570
-0.0027853742 -0.0010132179
-0.0033759060 -0.0004230788
-0.0039664377 0.0001670602
-0.0045569695 0.0007571993
-0.0051475009 0.0013473385
-0.0060776968 0.0018122176
-0.0070078927 0.0022770968
-0.0079380885 0.0027419759
-0.0088682844 0.0032068551
-0.0097984797 0.0036717342
-0.0107286750 0.0041366134
-0.0116588703 0.0046014925
-0.0125890656 0.0050663720
-0.0152322478 0.0068635848
-0.0178754301 0.0086607976
-0.0205186123 0.0104580099
-0.0231617945 0.0122552227
-0.0258049768 0.0140524355
-0.0284481590 0.0158496484
-0.0310913412 0.0176468612
-0.0337345235 0.0194440740
-0.0370998616 0.0227404122
-0.0404651997 0.0260367505
-0.0438305379 0.0293330887
-0.0471958760 0.0326294269
-0.0505612141 0.0359257651
-0.0539265523 0.0392221011
-0.0572918904 0.0425184393
-0.0606572286 0.0458147775
-0.0660258299 0.0518209913
-0.0713944313 0.0578272050
-0.0767630283 0.0638334188
-0.0821316252 0.0698396325
-0.0875002222 0.0758458418
-0.0928688192 0.0818520510
-0.0982374161 0.0878582603
-0.1036060131 0.0938644695
-0.1171312178 0.1036156638
-0.1306564225 0.1133668582
-0.1441816272 0.1231180525
-0.1577068231 0.1328692468
-0.1712320190 0.1426204411
-0.1847572148 0.1523716354
-0.1982824107 0.1621228297
-0.2118076066 0.1718740241
-0.2314065724 0.1847482076
-0.2510055382 0.1976223911
-0.2706045040 0.2104965746
-0.2902034698 0.2233707581
-0.3098024179 0.2362449416
-0.3294013838 0.2491191251
-0.3490003496 0.2619933086
-0.3685993154 0.2748674921
-0.3914969414 0.2893730908
-0.4143945675 0.3038786895
-0.4372921936 0.3183842883
-0.4601898197 0.3328898870
-0.4830874457 0.3473954857
-0.5059850718 0.3619010844
-0.5288826979 0.3764066831
-0.5517803239 0.3909122819
-0.5758329226 0.4063830199
-0.5998855213 0.4218537579
-0.6239381553 0.4373244959
-0.6479907187 0.4527952339
-0.6720432820 0.4682659719
-0.6960958454 0.4837367099
-0.7201484088 0.4992074479
-0.7442009721 0.5146781859
-0.7649476697 0.5275985080
-0.7856943672 0.5405188301
-0.8064410648 0.5534391522
-0.8271877623 0.5663594743
-0.8479344598 0.5792797964
-0.8686811574 0.5922001185
-0.8894278549 0.6051204406
-0.9101745524 0.6180407627
-0.9183765216 0.6168493512
-0.9265784908 0.6156579397
-0.9347804600 0.6144665283
-0.9429824292 0.6132751168
-0.9511843983 0.6120837054
-0.9593863675 0.6108922939
-0.9675883367 0.6097008824
-0.9757903059 0.6085094710
-0.9693046008 0.5986850720
-0.9628188957 0.5888606730
-0.9563331906 0.5790362741
-0.9498474855 0.5692118751
-0.9433617804 0.5593874762
-0.9368760753 0.5495630772
-0.9303903702 0.5397386782
-0.9239046651 0.5299142793
-0.9157914938 0.5176958701
-0.9076783225 0.5054774609
-0.8995651511 0.4932590517
-0.8914519798 0.4810406425
-0.8833388085 0.4688222334
-0.8752256372 0.4566038242
-0.8671124659 0.4443854150
-0.8589992945 0.4321670058
-0.8491230937 0.4195484160
-0.8392468928 0.4069298263
-0.8293706920 0.3943112365
-0.8194944911 0.3816926467
-0.8096182902 0.3690740570
-0.7997420894 0.3564554672
-0.7898658885 0.3438368775
-0.7799896877 0.3312182877
-0.7666010618 0.3195091533
-0.7532124359 0.3078000189
-0.7398238100 0.2960908665
-0.7264351841 0.2843817141
-0.7130465582 0.2726725617
-0.6996579323 0.2609634093
-0.6862693064 0.2492542568
-0.6728806805 0.2375451044
-0.6534653856 0.2258480956
-0.6340500908 0.2141510869
-0.6146347960 0.2024540781
-0.5952195012 0.1907570693
-0.5758042064 0.1790600605
-0.5563889116 0.1673630517
-0.5369736167 0.1556660429
-0.5175583219 0.1439690341
-0.4965378487 0.1348854691
-0.4755173754 0.1258019040
-0.4544969021 0.1167183389
-0.4334764288 0.1076347739
-0.4124559556 0.0985512088
-0.3914354823 0.0894676437
-0.3704150090 0.0803840787
-0.3493945357 0.0713005091
-0.3349602215 0.0664943138
-0.3205259072 0.0616881140
-0.3060915929 0.0568819142
-0.2916572786 0.0520757144
-0.2772229644 0.0472695146
-0.2627886501 0.0424633148
-0.2483543358 0.0376571172
-0.2339200215 0.0328509197
-0.2278978738 0.0311286437
-0.2218757260 0.0294063677
-0.2158535782 0.0276840918
-0.2098314304 0.0259618158
-0.2038092826 0.0242395399
-0.1977871348 0.0225172639
-0.1917649871 0.0207949880
-0.1857428393 0.0190727120


==> data/interpolated_data_sample_0_copy.tex <==
-0.0156602859 0.0029363632
-0.0145630836 0.0049524307
-0.0163588524 0.0030213594
-0.0174086094 0.0009107590
-0.0148069859 0.0008232594
-0.0126025677 0.0013860464
-0.0045340061 -0.0043551922
0.0212156773 -0.0189433098
0.0793929100 -0.0541504622
0.1987695694 -0.0986760855
0.3605892658 -0.1126396656
0.4451696873 -0.0927981138
0.4260101318 -0.0456384420
0.4041140079 -0.0068489313
0.4492764473 -0.0093681812
0.4948675632 -0.0240179300
0.5014607906 -0.0351053476
0.4708454609 -0.0403814316
0.4372471571 -0.0457067490
0.3866078854 -0.0421488285
0.3163704872 -0.0350291729
0.2382090092 -0.0300235748
0.1194462776 -0.0037435293
-0.0105616450 0.0258829594
-0.0405423641 0.0291070938
-0.0036502481 0.0088167191
-0.0056462884 0.0003504753
-0.0094343424 0.0074989796
0.0042116642 0.0025409460
-0.0041767359 0.0028419495
-0.0069888830 0.0083645582
0.0191609263 -0.0055223703
0.0453673601 -0.0139385462
0.0732489824 -0.0120003223
0.1047576070 -0.0072760582
0.1206273437 0.0126279593
0.1074476242 0.0431402922
0.0765731335 0.0465490818
0.0373477936 0.0243358612
0.0154087543 0.0120269060
0.0118119717 0.0113716125
0.0099725127 0.0195691586
0.0330178738 0.0314457417
0.1458519697 0.0249450207
0.3688678443 -0.0171146393
0.5771000385 -0.0519816875
0.6711282730 -0.0618969202
0.5865981579 -0.0422399044
0.2928413153 -0.0000822544
-0.1113004088 0.0581116676
-0.3566481471 0.1090236902
-0.3120940924 0.0559831858
-0.1739443541 -0.0653283596
-0.0548454672 -0.1600018740
0.0459987074 -0.1973054409
0.1351308525 -0.2156496048
0.1756991148 -0.2098776698
0.1736912429 -0.1565806866
0.1412188411 -0.0931944847
0.0627565384 -0.0400592685
-0.0180843472 0.0075258017
-0.0886839628 0.0547588468
-0.2096934021 0.1175619960
-0.3559187949 0.1896890998
-0.3981538713 0.1875975728
-0.3696793318 0.0935105085
-0.3499842584 0.0038975477
-0.3533948362 -0.0329167843
-0.3351592124 -0.0472149849
-0.2564865947 -0.0683767796
-0.1694749594 -0.0655798912
-0.0834707618 -0.0400851965
-0.0073689222 -0.0215698481
0.0152086020 -0.0035313964
0.0123479962 -0.0003244281
0.0204948187 -0.0089533329
0.0166320205 -0.0088743567
0.0110071898 -0.0005049706
0.0169406533 0.0012724996
0.0135948658 0.0016995668
0.0011677146 0.0052851439
-0.0052593946 0.0101886988
-0.0152998567 0.0187759399
-0.0301897526 0.0278040171
-0.0406373143 0.0361731052
-0.0531657934 0.0464407206
-0.0551303029 0.0451607704
-0.0379285812 0.0303109884
-0.0163505077 0.0149725676
-0.0053703189 0.0060950518
-0.0101740360 0.0072501898
-0.0148913860 0.0092942715
-0.0066822767 0.0037264824
-0.0028961301 0.0015953779
-0.0090609193 0.0049350262
-0.0091799498 0.0045316219
-0.0089932084 0.0047230721
-0.0133370161 0.0077458620
-0.0174069405 0.0099385977
-0.0215480328 0.0126204491
-0.0233193636 0.0134936571
-0.0213940144 0.0119938850
-0.0212739706 0.0114248991
-0.0243434906 0.0129648447
-0.0415388346 0.0228137970
-0.0678077936 0.0374208689
-0.0797133446 0.0416040421
-0.0841901302 0.0389331579
-0.1118147373 0.0435255766
-0.1670386791 0.0509687662
-0.2402540445 0.0526607037
-0.3407146931 0.0626282692
-0.4207458496 0.0772293806
-0.4453942776 0.0618461370
-0.4243600368 0.0375645161
-0.3698947430 0.0323835611
-0.2890303135 0.0397413969
-0.2015905380 0.0478830338
-0.1198480129 0.0438387394
-0.0626442432 0.0332008600
-0.0494074821 0.0309112072
-0.0648646355 0.0379235744
-0.0913560390 0.0514149666
-0.1133317947 0.0599182844
-0.1123733521 0.0517581701
-0.0951924324 0.0402438641
-0.0714974403 0.0329610109
-0.0448017120 0.0215091705


==> data/interpolated_data_sample_0_keypoints.tex <==
-0.0156602859 0.0029363632
-0.0145630836 0.0049524307
-0.0163588524 0.0030213594
-0.0174086094 0.0009107590
-0.0148069859 0.0008232594
-0.0126025677 0.0013860464
-0.0045340061 -0.0043551922
0.0212156773 -0.0189433098
0.0793929100 -0.0541504622
0.1987695694 -0.0986760855
0.3605892658 -0.1126396656
0.4451696873 -0.0927981138
0.4260101318 -0.0456384420
0.4041140079 -0.0068489313
0.4492764473 -0.0093681812
0.4948675632 -0.0240179300
0.5014607906 -0.0351053476
0.4708454609 -0.0403814316
0.4372471571 -0.0457067490
0.3866078854 -0.0421488285
0.3163704872 -0.0350291729
0.2382090092 -0.0300235748
0.1194462776 -0.0037435293
-0.0105616450 0.0258829594
-0.0405423641 0.0291070938
-0.0036502481 0.0088167191
-0.0056462884 0.0003504753
-0.0094343424 0.0074989796
0.0042116642 0.0025409460
-0.0041767359 0.0028419495
-0.0069888830 0.0083645582
0.0191609263 -0.0055223703
0.0453673601 -0.0139385462
0.0732489824 -0.0120003223
0.1047576070 -0.0072760582
0.1206273437 0.0126279593
0.1074476242 0.0431402922
0.0765731335 0.0465490818
0.0373477936 0.0243358612
0.0154087543 0.0120269060
0.0118119717 0.0113716125
0.0099725127 0.0195691586
0.0330178738 0.0314457417
0.1458519697 0.0249450207
0.3688678443 -0.0171146393
0.5771000385 -0.0519816875
0.6711282730 -0.0618969202
0.5865981579 -0.0422399044
0.2928413153 -0.0000822544
-0.1113004088 0.0581116676
-0.3566481471 0.1090236902
-0.3120940924 0.0559831858
-0.1739443541 -0.0653283596
-0.0548454672 -0.1600018740
0.0459987074 -0.1973054409
0.1351308525 -0.2156496048
0.1756991148 -0.2098776698
0.1736912429 -0.1565806866
0.1412188411 -0.0931944847
0.0627565384 -0.0400592685
-0.0180843472 0.0075258017
-0.0886839628 0.0547588468
-0.2096934021 0.1175619960
-0.3559187949 0.1896890998
-0.3981538713 0.1875975728
-0.3696793318 0.0935105085
-0.3499842584 0.0038975477
-0.3533948362 -0.0329167843
-0.3351592124 -0.0472149849
-0.2564865947 -0.0683767796
-0.1694749594 -0.0655798912
-0.0834707618 -0.0400851965
-0.0073689222 -0.0215698481
0.0152086020 -0.0035313964
0.0123479962 -0.0003244281
0.0204948187 -0.0089533329
0.0166320205 -0.0088743567
0.0110071898 -0.0005049706
0.0169406533 0.0012724996
0.0135948658 0.0016995668
0.0011677146 0.0052851439
-0.0052593946 0.0101886988
-0.0152998567 0.0187759399
-0.0301897526 0.0278040171
-0.0406373143 0.0361731052
-0.0531657934 0.0464407206
-0.0551303029 0.0451607704
-0.0379285812 0.0303109884
-0.0163505077 0.0149725676
-0.0053703189 0.0060950518
-0.0101740360 0.0072501898
-0.0148913860 0.0092942715
-0.0066822767 0.0037264824
-0.0028961301 0.0015953779
-0.0090609193 0.0049350262
-0.0091799498 0.0045316219
-0.0089932084 0.0047230721
-0.0133370161 0.0077458620
-0.0174069405 0.0099385977
-0.0215480328 0.0126204491
-0.0233193636 0.0134936571
-0.0213940144 0.0119938850
-0.0212739706 0.0114248991
-0.0243434906 0.0129648447
-0.0415388346 0.0228137970
-0.0678077936 0.0374208689
-0.0797133446 0.0416040421
-0.0841901302 0.0389331579
-0.1118147373 0.0435255766
-0.1670386791 0.0509687662
-0.2402540445 0.0526607037
-0.3407146931 0.0626282692
-0.4207458496 0.0772293806
-0.4453942776 0.0618461370
-0.4243600368 0.0375645161
-0.3698947430 0.0323835611
-0.2890303135 0.0397413969
-0.2015905380 0.0478830338
-0.1198480129 0.0438387394
-0.0626442432 0.0332008600
-0.0494074821 0.0309112072
-0.0648646355 0.0379235744
-0.0913560390 0.0514149666
-0.1133317947 0.0599182844
-0.1123733521 0.0517581701
-0.0951924324 0.0402438641
-0.0714974403 0.0329610109
-0.0448017120 0.0215091705


==> data/lif_sample100.tex <==
-0.1079607164 -0.0848400849
-0.1387761923 -0.1005631044
-0.1695916682 -0.1162861239
-0.2004071441 -0.1320091434
-0.2312226199 -0.1477321630
-0.2620380958 -0.1634551825
-0.2928535717 -0.1791782020
-0.3236690476 -0.1949012216
-0.3331623342 -0.1984825067
-0.3426556208 -0.2020637917
-0.3521489074 -0.2056450768
-0.3616421940 -0.2092263619
-0.3711354805 -0.2128076470
-0.3806287671 -0.2163889321
-0.3901220537 -0.2199702172
-0.3996153403 -0.2235515023
-0.4034644749 -0.2197878281
-0.4073136095 -0.2160241539
-0.4111627440 -0.2122604797
-0.4150118786 -0.2084968055
-0.4188610132 -0.2047331314
-0.4227101478 -0.2009694572
-0.4265592824 -0.1972057830
-0.4304084169 -0.1934421088
-0.4152562405 -0.1994986632
-0.4001040641 -0.2055552175
-0.3849518876 -0.2116117719
-0.3697997112 -0.2176683263
-0.3546475348 -0.2237248806
-0.3394953584 -0.2297814350
-0.3243431819 -0.2358379893
-0.3091910055 -0.2418945437
-0.3097478818 -0.2301774609
-0.3103047581 -0.2184603781
-0.3108616344 -0.2067432954
-0.3114185107 -0.1950262126
-0.3119753870 -0.1833091298
-0.3125322633 -0.1715920470
-0.3130891396 -0.1598749643
-0.3136460159 -0.1481578815
-0.2940586576 -0.1435691382
-0.2744712993 -0.1389803950
-0.2548839409 -0.1343916517
-0.2352965826 -0.1298029085
-0.2157092243 -0.1252141652
-0.1961218660 -0.1206254219
-0.1765345076 -0.1160366787
-0.1569471493 -0.1114479354
-0.1519408599 -0.1064052764
-0.1469345705 -0.1013626175
-0.1419282811 -0.0963199585
-0.1369219917 -0.0912772995
-0.1319157024 -0.0862346406
-0.1269094130 -0.0811919816
-0.1219031236 -0.0761493226
-0.1168968342 -0.0711066636
-0.1016435088 -0.0652190257
-0.0863901834 -0.0593313877
-0.0711368581 -0.0534437498
-0.0558835327 -0.0475561118
-0.0406302073 -0.0416684739
-0.0253768819 -0.0357808359
-0.0101235566 -0.0298931980
0.0051297688 -0.0240055600
0.0043538670 -0.0208701630
0.0035779651 -0.0177347659
0.0028020633 -0.0145993689
0.0020261615 -0.0114639718
0.0012502596 -0.0083285748
0.0004743578 -0.0051931778
-0.0003015440 -0.0020577807
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0043432831 0.0009425678
-0.0076091203 0.0008075193
-0.0108749575 0.0006724709
-0.0141407947 0.0005374224
-0.0174066319 0.0004023739
-0.0206724691 0.0002673254
-0.0239383063 0.0001322769
-0.0272041435 -0.0000027716
-0.0285006782 0.0015762758
-0.0297972130 0.0031553231
-0.0310937478 0.0047343704
-0.0323902825 0.0063134178
-0.0336868173 0.0078924651
-0.0349833521 0.0094715124
-0.0362798868 0.0110505598
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0375764216 0.0126296071
-0.0465802277 0.0204312327
-0.0555840339 0.0282328582
-0.0645878401 0.0360344838
-0.0735916463 0.0438361094
-0.0825954524 0.0516377349
-0.0915992586 0.0594393605
-0.1006030648 0.0672409860
-0.1096068709 0.0750426116
-0.1154746645 0.0720835294
-0.1213424580 0.0691244471
-0.1272102515 0.0661653648
-0.1330780450 0.0632062826
-0.1389458385 0.0602472003
-0.1448136320 0.0572881181
-0.1506814255 0.0543290358
-0.1565492190 0.0513699536
-0.1548880331 0.0542273802
-0.1532268471 0.0570848069
-0.1515656611 0.0599422336
-0.1499044752 0.0627996603
-0.1482432892 0.0656570870
-0.1465821033 0.0685145137
-0.1449209173 0.0713719403
-0.1432597313 0.0742293670
-0.1421470008 0.0828905517
-0.1410342703 0.0915517364
-0.1399215398 0.1002129211
-0.1388088094 0.1088741058
-0.1376960789 0.1175352905
-0.1365833484 0.1261964751
-0.1354706179 0.1348576598
-0.1343578874 0.1435188445
-0.1360144297 0.1469799575
-0.1376709720 0.1504410704
-0.1393275143 0.1539021834
-0.1409840566 0.1573632963
-0.1426405989 0.1608244093
-0.1442971413 0.1642855222
-0.1459536836 0.1677466352
-0.1476102259 0.1712077481
-0.1463119590 0.1696971129
-0.1450136921 0.1681864777
-0.1437154252 0.1666758424
-0.1424171583 0.1651652072
-0.1411188914 0.1636545720
-0.1398206246 0.1621439368
-0.1385223577 0.1606333015
-0.1372240908 0.1591226663
-0.1215745050 0.1598637731
-0.1059249192 0.1606048799
-0.0902753334 0.1613459867
-0.0746257476 0.1620870935
-0.0589761618 0.1628282003
-0.0433265760 0.1635693072
-0.0276769902 0.1643104140
-0.0120274044 0.1650515208
-0.0148692461 0.1703658135
-0.0177110879 0.1756801062
-0.0205529296 0.1809943990
-0.0233947714 0.1863086917
-0.0262366131 0.1916229844
-0.0290784549 0.1969372771
-0.0319202966 0.2022515699
-0.0347621383 0.2075658626
-0.0230949613 0.2067349597
-0.0114277843 0.2059040567
0.0002393928 0.2050731538
0.0119065698 0.2042422508
0.0235737468 0.2034113479
0.0352409239 0.2025804449
0.0469081009 0.2017495420
0.0585752779 0.2009186391
0.0511926859 0.2107916577
0.0438100940 0.2206646763
0.0364275020 0.2305376949
0.0290449100 0.2404107135
0.0216623180 0.2502837321
0.0142797260 0.2601567507
0.0068971341 0.2700297693
-0.0004854579 0.2799027880
0.0016857702 0.2854416342
0.0038569983 0.2909804804
0.0060282264 0.2965193266
0.0081994545 0.3020581728
0.0103706826 0.3075970190
0.0125419108 0.3131358653
0.0147131389 0.3186747115
0.0168843670 0.3242135577
0.0149682295 0.3184352604
0.0130520920 0.3126569631
0.0111359545 0.3068786658
0.0092198170 0.3011003685
0.0073036794 0.2953220711
0.0053875419 0.2895437738
0.0034714044 0.2837654765
0.0015552669 0.2779871792
-0.0079525817 0.2835403050
-0.0174604303 0.2890934308
-0.0269682790 0.2946465566
-0.0364761276 0.3001996825
-0.0459839762 0.3057528083
-0.0554918248 0.3113059341
-0.0649996735 0.3168590599
-0.0745075221 0.3224121857
-0.0764071415 0.3136278516
-0.0783067608 0.3048435175
-0.0802063802 0.2960591835
-0.0821059996 0.2872748494
-0.0840056190 0.2784905153
-0.0859052384 0.2697061812
-0.0878048578 0.2609218471
-0.0897044771 0.2521375130
-0.0936384116 0.2532746548
-0.0975723461 0.2544117965
-0.1015062806 0.2555489383
-0.1054402151 0.2566860801
-0.1093741496 0.2578232219
-0.1133080842 0.2589603636
-0.1172420187 0.2600975054
-0.1211759532 0.2612346472
-0.1295936828 0.2643184695
-0.1380114124 0.2674022919
-0.1464291420 0.2704861142
-0.1548468716 0.2735699366
-0.1632646012 0.2766537589
-0.1716823308 0.2797375813
-0.1801000604 0.2828214036
-0.1885177900 0.2859052260
-0.1899908335 0.2811392441
-0.1914638770 0.2763732622
-0.1929369205 0.2716072803
-0.1944099641 0.2668412984
-0.1958830076 0.2620753165
-0.1973560511 0.2573093345
-0.1988290946 0.2525433526
-0.2003021381 0.2477773707
-0.2051524650 0.2557626586
-0.2100027919 0.2637479465
-0.2148531188 0.2717332344
-0.2197034457 0.2797185223
-0.2245537726 0.2877038102
-0.2294040995 0.2956890981
-0.2342544264 0.3036743860
-0.2391047533 0.3116596738
-0.2258282759 0.3072529013
-0.2125517986 0.3028461287
-0.1992753213 0.2984393562
-0.1859988440 0.2940325836
-0.1727223666 0.2896258110
-0.1594458893 0.2852190385
-0.1461694120 0.2808122659
-0.1328929347 0.2764054933
-0.1333279314 0.2657248035
-0.1337629281 0.2550441136
-0.1341979247 0.2443634238
-0.1346329214 0.2336827339
-0.1350679181 0.2230020440
-0.1355029148 0.2123213542
-0.1359379115 0.2016406643
-0.1363729082 0.1909599744
-0.1292586466 0.1881344006
-0.1221443849 0.1853088267
-0.1150301233 0.1824832528
-0.1079158616 0.1796576789
-0.1008016000 0.1768321050
-0.0936873383 0.1740065311
-0.0865730767 0.1711809572
-0.0794588150 0.1683553834
-0.0796559821 0.1616148823
-0.0798531491 0.1548743812
-0.0800503162 0.1481338802
-0.0802474832 0.1413933791
-0.0804446503 0.1346528781
-0.0806418173 0.1279123770
-0.0808389844 0.1211718760
-0.0810361514 0.1144313749
-0.0722192920 0.1072436773
-0.0634024326 0.1000559797
-0.0545855732 0.0928682821
-0.0457687138 0.0856805845
-0.0369518544 0.0784928869
-0.0281349950 0.0713051892
-0.0193181356 0.0641174916
-0.0105012762 0.0569297940
-0.0106198320 0.0515273191
-0.0107383878 0.0461248442
-0.0108569436 0.0407223693
-0.0109754994 0.0353198944
-0.0110940553 0.0299174195
-0.0112126111 0.0245149446
-0.0113311669 0.0191124697
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0315671029 -0.0187272262
0.0378659349 -0.0204788547
0.0441647669 -0.0222304833
0.0504635989 -0.0239821118
0.0567624309 -0.0257337403
0.0630612629 -0.0274853688
0.0693600950 -0.0292369973
0.0756589270 -0.0309886259
0.0903632221 -0.0297414397
0.1050675173 -0.0284942536
0.1197718125 -0.0272470675
0.1344761077 -0.0259998813
0.1491804028 -0.0247526952
0.1638846980 -0.0235055091
0.1785889932 -0.0222583229
0.1932932883 -0.0210111368
0.1900000764 -0.0187544851
0.1867068644 -0.0164978333
0.1834136525 -0.0142411816
0.1801204405 -0.0119845298
0.1768272286 -0.0097278781
0.1735340166 -0.0074712264
0.1702408047 -0.0052145746
0.1669475927 -0.0029579229
0.1592303328 0.0015284357
0.1515130729 0.0060147942
0.1437958130 0.0105011528
0.1360785531 0.0149875113
0.1283612932 0.0194738699
0.1206440333 0.0239602285
0.1129267734 0.0284465870
0.1052095135 0.0329329456
0.0967280134 0.0337400933
0.0882465134 0.0345472410
0.0797650133 0.0353543887
0.0712835132 0.0361615363
0.0628020131 0.0369686840
0.0543205130 0.0377758317
0.0458390129 0.0385829794
0.0373575129 0.0393901271
0.0234867550 0.0413798427
0.0096159972 0.0433695583
-0.0042547606 0.0453592739
-0.0181255184 0.0473489895
-0.0319962763 0.0493387051
-0.0458670341 0.0513284207
-0.0597377919 0.0533181363
-0.0736085497 0.0553078519
-0.0773617780 0.0602500440
-0.0811150063 0.0651922360
-0.0848682346 0.0701344281
-0.0886214629 0.0750766201
-0.0923746912 0.0800188122
-0.0961279195 0.0849610042
-0.0998811478 0.0899031963
-0.1036343761 0.0948453883
-0.0946305705 0.0870437630
-0.0856267649 0.0792421377
-0.0766229593 0.0714405125
-0.0676191537 0.0636388872
-0.0586153480 0.0558372619
-0.0496115424 0.0480356366
-0.0406077368 0.0402340113
-0.0316039312 0.0324323860
-0.0290846551 0.0300920871
-0.0265653791 0.0277517882
-0.0240461030 0.0254114893
-0.0215268269 0.0230711904
-0.0190075509 0.0207308915
-0.0164882748 0.0183905926
-0.0139689988 0.0160502937
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0252682709 -0.0169755977
0.0184174667 -0.0161028044
0.0115666626 -0.0152300111
0.0047158584 -0.0143572178
-0.0021349458 -0.0134844245
-0.0089857499 -0.0126116312
-0.0158365541 -0.0117388379
-0.0226873582 -0.0108660446
-0.0295381624 -0.0099932513
-0.0228092528 -0.0097103620
-0.0160803431 -0.0094274726
-0.0093514334 -0.0091445833
-0.0026225238 -0.0088616939
0.0041063859 -0.0085788045
0.0108352955 -0.0082959152
0.0175642052 -0.0080130258
0.0242931148 -0.0077301365
0.0314604032 -0.0081621003
0.0386276916 -0.0085940641
0.0457949799 -0.0090260279
0.0529622683 -0.0094579917
0.0601295567 -0.0098899555
0.0672968450 -0.0103219193
0.0744641334 -0.0107538831
0.0816314218 -0.0111858469
0.0934910055 -0.0203269014
0.1053505892 -0.0294679559
0.1172101729 -0.0386090104
0.1290697566 -0.0477500649
0.1409293403 -0.0568911194
0.1527889240 -0.0660321739
0.1646485077 -0.0751732283
0.1765080914 -0.0843142828
0.1872941966 -0.0941310695
0.1980803017 -0.1039478561
0.2088664069 -0.1137646427
0.2196525120 -0.1235814294
0.2304386172 -0.1333982160
0.2412247224 -0.1432150027
0.2520108275 -0.1530317893
0.2627969327 -0.1628485759
0.2810548177 -0.1737540538
0.2993127027 -0.1846595318
0.3175705878 -0.1955650097
0.3358284728 -0.2064704876
0.3540863578 -0.2173759655
0.3723442429 -0.2282814435
0.3906021279 -0.2391869214
0.4088600129 -0.2500923993
0.4247546263 -0.2554507353
0.4406492398 -0.2608090712
0.4565438532 -0.2661674072
0.4724384666 -0.2715257431
0.4883330800 -0.2768840791
0.5042276934 -0.2822424151
0.5201223068 -0.2876007510
0.5360169202 -0.2929590870
0.5671637534 -0.3076411203
0.5983105865 -0.3223231536
0.6294574196 -0.3370051868
0.6606042528 -0.3516872201
0.6917510859 -0.3663692534
0.7228979190 -0.3810512867
0.7540447522 -0.3957333200
0.7851915853 -0.4104153533
0.7736104320 -0.4061325477
0.7620292787 -0.4018497422
0.7504481254 -0.3975669367
0.7388669722 -0.3932841311
0.7272858189 -0.3890013256
0.7157046656 -0.3847185200
0.7041235123 -0.3804357145
0.6925423590 -0.3761529090
0.7087561361 -0.3900185399
0.7249699132 -0.4038841709
0.7411836903 -0.4177498019
0.7573974673 -0.4316154329
0.7736112444 -0.4454810639
0.7898250215 -0.4593466948
0.8060387985 -0.4732123258
0.8222525756 -0.4870779568
0.7793475101 -0.4697475375
0.7364424445 -0.4524171182
0.6935373789 -0.4350866990
0.6506323134 -0.4177562797
0.6077272478 -0.4004258604
0.5648221823 -0.3830954412
0.5219171167 -0.3657650219
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4790120512 -0.3484346026
0.4583269806 -0.3353882204
0.4376419099 -0.3223418382
0.4169568393 -0.3092954559
0.3962717687 -0.2962490737
0.3755866981 -0.2832026915
0.3549016274 -0.2701563093
0.3342165568 -0.2571099270
0.3135314862 -0.2440635448
0.2902082423 -0.2434807225
0.2668849985 -0.2428979002
0.2435617546 -0.2423150779
0.2202385108 -0.2417322556
0.1969152669 -0.2411494334
0.1735920231 -0.2405666111
0.1502687793 -0.2399837888
0.1269455354 -0.2394009665
0.1174008176 -0.2186833793
0.1078560998 -0.1979657921
0.0983113821 -0.1772482049
0.0887666643 -0.1565306177
0.0792219465 -0.1358130304
0.0696772287 -0.1150954432
0.0601325110 -0.0943778560
0.0505877932 -0.0736602688
0.0445321321 -0.0681812693
0.0384764711 -0.0627022698
0.0324208100 -0.0572232703
0.0263651489 -0.0517442708
0.0203094879 -0.0462652712
0.0142538268 -0.0407862717
0.0081981657 -0.0353072722
0.0021425047 -0.0298282727
0.0017400109 -0.0259650366
0.0013375170 -0.0221018004
0.0009350232 -0.0182385643
0.0005325294 -0.0143753282
0.0001300356 -0.0105120921
-0.0002724582 -0.0066488559
-0.0006749520 -0.0027856198
-0.0010774458 0.0010776163
-0.0017054512 0.0040047434
-0.0023334565 0.0069318705
-0.0029614618 0.0098589975
-0.0035894672 0.0127861246
-0.0042174725 0.0157132517
-0.0048454778 0.0186403788
-0.0054734832 0.0215675058
-0.0061014885 0.0244946329
-0.0076248024 0.0312102896
-0.0091481163 0.0379259462
-0.0106714303 0.0446416029
-0.0121947442 0.0513572596
-0.0137180581 0.0580729163
-0.0152413721 0.0647885729
-0.0167646860 0.0715042296
-0.0182879999 0.0782198863
-0.0215178234 0.0864634474
-0.0247476470 0.0947070086
-0.0279774705 0.1029505698
-0.0312072940 0.1111941309
-0.0344371175 0.1194376921
-0.0376669411 0.1276812533
-0.0408967646 0.1359248144
-0.0441265881 0.1441683756
-0.0468430997 0.1464958812
-0.0495596112 0.1488233867
-0.0522761228 0.1511508923
-0.0549926343 0.1534783978
-0.0577091459 0.1558059034
-0.0604256574 0.1581334089
-0.0631421690 0.1604609145
-0.0658586805 0.1627884200
-0.0746729590 0.1663098643
-0.0834872374 0.1698313086
-0.0923015159 0.1733527529
-0.1011157944 0.1768741972
-0.1099300728 0.1803956415
-0.1187443513 0.1839170858
-0.1275586298 0.1874385301
-0.1363729082 0.1909599744
-0.1294558136 0.1813938995
-0.1225387190 0.1718278246
-0.1156216244 0.1622617496
-0.1087045298 0.1526956747
-0.1017874352 0.1431295998
-0.0948703406 0.1335635248
-0.0879532460 0.1239974499
-0.0810361514 0.1144313749
-0.0722192920 0.1072436773
-0.0634024326 0.1000559797
-0.0545855732 0.0928682821
-0.0457687138 0.0856805845
-0.0369518544 0.0784928869
-0.0281349950 0.0713051892
-0.0193181356 0.0641174916
-0.0105012762 0.0569297940
-0.0106198320 0.0515273191
-0.0107383878 0.0461248442
-0.0108569436 0.0407223693
-0.0109754994 0.0353198944
-0.0110940553 0.0299174195
-0.0112126111 0.0245149446
-0.0113311669 0.0191124697
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163


==> data/lif_sample53.tex <==
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0134190253 0.0119958990
-0.0153883279 0.0102818032
-0.0173576305 0.0085677074
-0.0193269331 0.0068536116
-0.0212962357 0.0051395158
-0.0232655383 0.0034254200
-0.0252348409 0.0017113242
-0.0272041435 -0.0000027716
-0.0252348409 0.0017113242
-0.0232655383 0.0034254200
-0.0212962357 0.0051395158
-0.0193269331 0.0068536116
-0.0173576305 0.0085677074
-0.0153883279 0.0102818032
-0.0134190253 0.0119958990
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0134190253 0.0119958990
-0.0153883279 0.0102818032
-0.0173576305 0.0085677074
-0.0193269331 0.0068536116
-0.0212962357 0.0051395158
-0.0232655383 0.0034254200
-0.0252348409 0.0017113242
-0.0272041435 -0.0000027716
-0.0239383063 0.0001322769
-0.0206724691 0.0002673254
-0.0174066319 0.0004023739
-0.0141407947 0.0005374224
-0.0108749575 0.0006724709
-0.0076091203 0.0008075193
-0.0043432831 0.0009425678
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0101531881 0.0121309474
-0.0088566535 0.0105519001
-0.0075601189 0.0089728528
-0.0062635843 0.0073938055
-0.0049670497 0.0058147582
-0.0036705151 0.0042357109
-0.0023739805 0.0026566636
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163


==> data/lif_sample62.tex <==
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0219750563 -0.0147189459
0.0186818417 -0.0124622942
0.0153886271 -0.0102056424
0.0120954125 -0.0079489907
0.0088021979 -0.0056923389
0.0055089833 -0.0034356872
0.0022157687 -0.0011790354
-0.0010774458 0.0010776163
-0.0027031940 -0.0023561191
-0.0043289422 -0.0057898545
-0.0059546903 -0.0092235899
-0.0075804385 -0.0126573253
-0.0092061866 -0.0160910607
-0.0108319348 -0.0195247961
-0.0124576829 -0.0229585315
-0.0140834311 -0.0263922669
-0.0166027073 -0.0240519679
-0.0191219835 -0.0217116689
-0.0216412597 -0.0193713700
-0.0241605359 -0.0170310710
-0.0266798121 -0.0146907720
-0.0291990883 -0.0123504730
-0.0317183645 -0.0100101740
-0.0342376407 -0.0076698750
-0.0342083000 -0.0132806190
-0.0341789592 -0.0188913631
-0.0341496185 -0.0245021071
-0.0341202778 -0.0301128511
-0.0340909371 -0.0357235951
-0.0340615963 -0.0413343391
-0.0340322556 -0.0469450831
-0.0340029149 -0.0525558271
-0.0302287379 -0.0605063092
-0.0264545608 -0.0684567913
-0.0226803838 -0.0764072733
-0.0189062068 -0.0843577554
-0.0151320297 -0.0923082375
-0.0113578527 -0.1002587196
-0.0075836757 -0.1082092017
-0.0038094986 -0.1161596837
-0.0050310065 -0.1205504941
-0.0062525143 -0.1249413045
-0.0074740221 -0.1293321148
-0.0086955299 -0.1337229252
-0.0099170377 -0.1381137355
-0.0111385455 -0.1425045459
-0.0123600533 -0.1468953563
-0.0135815611 -0.1512861666
-0.0177345673 -0.1679878427
-0.0218875735 -0.1846895187
-0.0260405796 -0.2013911947
-0.0301935858 -0.2180928708
-0.0343465920 -0.2347945468
-0.0384995981 -0.2514962229
-0.0426526043 -0.2681978989
-0.0468056105 -0.2848995750
-0.0603819870 -0.2930394010
-0.0739583635 -0.3011792270
-0.0875347400 -0.3093190530
-0.1011111165 -0.3174588790
-0.1146874930 -0.3255987051
-0.1282638695 -0.3337385311
-0.1418402460 -0.3418783571
-0.1554166225 -0.3500181831
-0.1409929824 -0.3598373583
-0.1265693424 -0.3696565335
-0.1121457023 -0.3794757087
-0.0977220623 -0.3892948840
-0.0832984222 -0.3991140592
-0.0688747822 -0.4089332344
-0.0544511421 -0.4187524096
-0.0400275021 -0.4285715848
-0.0558157072 -0.4331352277
-0.0716039123 -0.4376988706
-0.0873921174 -0.4422625135
-0.1031803225 -0.4468261564
-0.1189685276 -0.4513897992
-0.1347567327 -0.4559534421
-0.1505449378 -0.4605170850
-0.1663331429 -0.4650807279
-0.1567041031 -0.4716295393
-0.1470750634 -0.4781783506
-0.1374460236 -0.4847271620
-0.1278169839 -0.4912759734
-0.1181879441 -0.4978247848
-0.1085589043 -0.5043735962
-0.0989298646 -0.5109224076
-0.0893008248 -0.5174712190
-0.0984770317 -0.5222601326
-0.1076532386 -0.5270490462
-0.1168294455 -0.5318379598
-0.1260056524 -0.5366268734
-0.1351818593 -0.5414157871
-0.1443580662 -0.5462047007
-0.1535342730 -0.5509936143
-0.1627104799 -0.5557825279
-0.1752541442 -0.5583581739
-0.1877978085 -0.5609338199
-0.2003414729 -0.5635094659
-0.2128851372 -0.5660851118
-0.2254288015 -0.5686607578
-0.2379724658 -0.5712364038
-0.2505161301 -0.5738120498
-0.2630597944 -0.5763876957
-0.2576101195 -0.5609817268
-0.2521604446 -0.5455757578
-0.2467107697 -0.5301697889
-0.2412610948 -0.5147638200
-0.2358114199 -0.4993578510
-0.2303617450 -0.4839518821
-0.2249120701 -0.4685459131
-0.2194623952 -0.4531399442
-0.2164547806 -0.4465132908
-0.2134471660 -0.4398866375
-0.2104395514 -0.4332599842
-0.2074319367 -0.4266333308
-0.2044243221 -0.4200066775
-0.2014167075 -0.4133800241
-0.1984090929 -0.4067533708
-0.1954014783 -0.4001267174
-0.1959208875 -0.3884120074
-0.1964402967 -0.3766972975
-0.1969597059 -0.3649825875
-0.1974791151 -0.3532678775
-0.1979985243 -0.3415531675
-0.1985179334 -0.3298384575
-0.1990373426 -0.3181237475
-0.1995567518 -0.3064090376
-0.1905043076 -0.2922368430
-0.1814518634 -0.2780646484
-0.1723994192 -0.2638924538
-0.1633469750 -0.2497202592
-0.1542945307 -0.2355480646
-0.1452420865 -0.2213758700
-0.1361896423 -0.2072036754
-0.1271371981 -0.1930314807
-0.1128507565 -0.1843834445
-0.0985643149 -0.1757354083
-0.0842778733 -0.1670873721
-0.0699914317 -0.1584393358
-0.0557049901 -0.1497912996
-0.0414185485 -0.1411432634
-0.0271321068 -0.1324952272
-0.0128456652 -0.1238471909
-0.0109721440 -0.1120948262
-0.0090986228 -0.1003424614
-0.0072251015 -0.0885900966
-0.0053515803 -0.0768377318
-0.0034780590 -0.0650853670
-0.0016045378 -0.0533330023
0.0002689834 -0.0415806375
0.0021425047 -0.0298282727
0.0017400109 -0.0259650366
0.0013375170 -0.0221018004
0.0009350232 -0.0182385643
0.0005325294 -0.0143753282
0.0001300356 -0.0105120921
-0.0002724582 -0.0066488559
-0.0006749520 -0.0027856198
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0384179071 -0.0196000192
0.0515675432 -0.0222244408
0.0647171794 -0.0248488623
0.0778668156 -0.0274732838
0.0910164518 -0.0300977054
0.1041660879 -0.0327221269
0.1173157241 -0.0353465484
0.1304653603 -0.0379709700
0.1279659900 -0.0368285670
0.1254666197 -0.0356861639
0.1229672494 -0.0345437609
0.1204678792 -0.0334013579
0.1179685089 -0.0322589549
0.1154691386 -0.0311165519
0.1129697683 -0.0299741488
0.1104703981 -0.0288317458
0.1278989059 -0.0332803228
0.1453274138 -0.0377288997
0.1627559217 -0.0421774766
0.1801844296 -0.0466260535
0.1976129374 -0.0510746304
0.2150414453 -0.0555232074
0.2324699532 -0.0599717843
0.2498984611 -0.0644203612
0.2514213717 -0.0493742089
0.2529442823 -0.0343280566
0.2544671930 -0.0192819043
0.2559901036 -0.0042357520
0.2575130142 0.0108104003
0.2590359249 0.0258565526
0.2605588355 0.0409027049
0.2620817461 0.0559488572
0.2832734528 0.0449870340
0.3044651596 0.0340252107
0.3256568663 0.0230633875
0.3468485730 0.0121015642
0.3680402798 0.0011397410
0.3892319865 -0.0098220822
0.4104236932 -0.0207839055
0.4316154000 -0.0317457287
0.4318420968 -0.0273595351
0.4320687936 -0.0229733414
0.4322954904 -0.0185871477
0.4325221872 -0.0142009541
0.4327488840 -0.0098147604
0.4329755807 -0.0054285668
0.4332022775 -0.0010423731
0.4334289743 0.0033438206
0.4641158000 -0.0037431539
0.4948026256 -0.0108301283
0.5254894512 -0.0179171028
0.5561762768 -0.0250040772
0.5868631024 -0.0320910517
0.6175499280 -0.0391780261
0.6482367536 -0.0462650006
0.6789235793 -0.0533519750
0.7055635370 -0.0573036793
0.7322034947 -0.0612553836
0.7588434525 -0.0652070879
0.7854834102 -0.0691587921
0.8121233680 -0.0731104964
0.8387633257 -0.0770622007
0.8654032834 -0.0810139050
0.8920432412 -0.0849656093
0.8851420511 -0.0756914412
0.8782408611 -0.0664172730
0.8713396710 -0.0571431049
0.8644384809 -0.0478689367
0.8575372909 -0.0385947686
0.8506361008 -0.0293206004
0.8437349108 -0.0200464323
0.8368337207 -0.0107722641
0.8654465079 0.0007332529
0.8940592952 0.0122387699
0.9226720824 0.0237442870
0.9512848696 0.0352498040
0.9798976569 0.0467553211
1.0085104441 0.0582608381
1.0371232313 0.0697663551
1.0657360185 0.0812718722
1.0905743758 0.0764389114
1.1154127331 0.0716059506
1.1402510904 0.0667729898
1.1650894477 0.0619400290
1.1899278050 0.0571070682
1.2147661623 0.0522741074
1.2396045196 0.0474411466
1.2644428769 0.0426081858
1.2780021579 0.0443858693
1.2915614388 0.0461635529
1.3051207198 0.0479412364
1.3186800008 0.0497189200
1.3322392817 0.0514966035
1.3457985627 0.0532742871
1.3593578437 0.0550519706
1.3729171247 0.0568296541
1.4048829405 0.0504745819
1.4368487564 0.0441195097
1.4688145723 0.0377644374
1.5007803882 0.0314093652
1.5327462041 0.0250542929
1.5647120199 0.0186992207
1.5966778358 0.0123441484
1.6286436517 0.0059890762
1.6125730409 0.0044163534
1.5965024300 0.0028436306
1.5804318192 0.0012709079
1.5643612084 -0.0003018149
1.5482905975 -0.0018745377
1.5322199867 -0.0034472604
1.5161493758 -0.0050199832
1.5000787650 -0.0065927060
1.5153224855 -0.0147418597
1.5305662061 -0.0228910134
1.5458099266 -0.0310401672
1.5610536471 -0.0391893209
1.5762973676 -0.0473384746
1.5915410881 -0.0554876283
1.6067848087 -0.0636367821
1.6220285292 -0.0717859358
1.6000450195 -0.0770714804
1.5780615098 -0.0823570251
1.5560780001 -0.0876425697
1.5340944904 -0.0929281143
1.5121109807 -0.0982136590
1.4901274710 -0.1034992036
1.4681439613 -0.1087847483
1.4461604516 -0.1140702929
1.4182550007 -0.1081717101
1.3903495499 -0.1022731273
1.3624440991 -0.0963745445
1.3345386482 -0.0904759617
1.3066331974 -0.0845773789
1.2787277466 -0.0786787962
1.2508222957 -0.0727802134
1.2229168449 -0.0668816306
1.1973981279 -0.0658334995
1.1718794109 -0.0647853683
1.1463606939 -0.0637372372
1.1208419768 -0.0626891061
1.0953232598 -0.0616409750
1.0698045428 -0.0605928439
1.0442858258 -0.0595447128
1.0187671088 -0.0584965816
1.0150431707 -0.0519728748
1.0113192326 -0.0454491679
1.0075952946 -0.0389254611
1.0038713565 -0.0324017542
1.0001474184 -0.0258780474
0.9964234803 -0.0193543405
0.9926995423 -0.0128306337
0.9889756042 -0.0063069268
0.9813383262 -0.0146830331
0.9737010481 -0.0230591393
0.9660637701 -0.0314352455
0.9584264921 -0.0398113517
0.9507892140 -0.0481874580
0.9431519360 -0.0565635642
0.9355146580 -0.0649396704
0.9278773800 -0.0733157766
0.8929513794 -0.0680299642
0.8580253789 -0.0627441517
0.8230993783 -0.0574583392
0.7881733778 -0.0521725267
0.7532473772 -0.0468867143
0.7183213767 -0.0416009018
0.6833953761 -0.0363150893
0.6484693756 -0.0310292768
0.6201181341 -0.0370998198
0.5917668926 -0.0431703628
0.5634156511 -0.0492409058
0.5350644096 -0.0553114488
0.5067131680 -0.0613819918
0.4783619265 -0.0674525348
0.4500106850 -0.0735230778
0.4216594435 -0.0795936208
0.4049838244 -0.0773081589
0.3883082053 -0.0750226971
0.3716325862 -0.0727372353
0.3549569671 -0.0704517735
0.3382813481 -0.0681663116
0.3216057290 -0.0658808498
0.3049301099 -0.0635953880
0.2882544908 -0.0613099262
0.2685308495 -0.0583925566
0.2488072082 -0.0554751871
0.2290835668 -0.0525578176
0.2093599255 -0.0496404481
0.1896362842 -0.0467230785
0.1699126429 -0.0438057090
0.1501890016 -0.0408883395
0.1304653603 -0.0379709700
0.1387213468 -0.0397142266
0.1469773334 -0.0414574833
0.1552333199 -0.0432007399
0.1634893065 -0.0449439966
0.1717452930 -0.0466872532
0.1800012796 -0.0484305099
0.1882572661 -0.0501737666
0.1965132527 -0.0519170232
0.1863968192 -0.0428898246
0.1762803857 -0.0338626260
0.1661639523 -0.0248354274
0.1560475188 -0.0158082288
0.1459310854 -0.0067810302
0.1358146519 0.0022461684
0.1256982185 0.0112733671
0.1155817850 0.0203005657
0.1071002855 0.0211077134
0.0986187859 0.0219148610
0.0901372864 0.0227220087
0.0816557869 0.0235291564
0.0731742873 0.0243363041
0.0646927878 0.0251434518
0.0562112883 0.0259505995
0.0477297888 0.0267577472
0.0410008791 0.0264748579
0.0342719694 0.0261919686
0.0275430598 0.0259090793
0.0208141501 0.0256261900
0.0140852405 0.0253433008
0.0073563308 0.0250604115
0.0006274212 0.0247775222
-0.0061014885 0.0244946329
-0.0067700178 0.0231465531
-0.0074385470 0.0217984734
-0.0081070763 0.0204503936
-0.0087756056 0.0191023138
-0.0094441349 0.0177542341
-0.0101126641 0.0164061543
-0.0107811934 0.0150580745
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0147155601 0.0135749463
-0.0179813974 0.0134398978
-0.0212472348 0.0133048494
-0.0245130721 0.0131698009
-0.0277789095 0.0130347525
-0.0310447469 0.0128997040
-0.0343105842 0.0127646556
-0.0375764216 0.0126296071
-0.0330140496 0.0111856082
-0.0284516776 0.0097416094
-0.0238893057 0.0082976106
-0.0193269337 0.0068536117
-0.0147645617 0.0054096129
-0.0102021898 0.0039656140
-0.0056398178 0.0025216152
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0147155601 0.0135749463
-0.0179813974 0.0134398978
-0.0212472348 0.0133048494
-0.0245130721 0.0131698009
-0.0277789095 0.0130347525
-0.0310447469 0.0128997040
-0.0343105842 0.0127646556
-0.0375764216 0.0126296071
-0.0504870697 0.0239473066
-0.0633977178 0.0352650061
-0.0763083659 0.0465827056
-0.0892190140 0.0579004051
-0.1021296621 0.0692181047
-0.1150403102 0.0805358042
-0.1279509583 0.0918535037
-0.1408616064 0.1031712032
-0.1411613720 0.0995534737
-0.1414611376 0.0959357442
-0.1417609032 0.0923180146
-0.1420606688 0.0887002851
-0.1423604345 0.0850825556
-0.1426602001 0.0814648261
-0.1429599657 0.0778470965
-0.1432597313 0.0742293670
-0.1459059324 0.0731528645
-0.1485521335 0.0720763619
-0.1511983346 0.0709998594
-0.1538445357 0.0699233568
-0.1564907368 0.0688468543
-0.1591369379 0.0677703518
-0.1617831390 0.0666938492
-0.1644293401 0.0656173467
-0.1565325617 0.0638344163
-0.1486357833 0.0620514859
-0.1407390049 0.0602685554
-0.1328422265 0.0584856250
-0.1249454480 0.0567026946
-0.1170486696 0.0549197642
-0.1091518912 0.0531368338
-0.1012551128 0.0513539034
-0.0982142387 0.0453362827
-0.0951733646 0.0393186621
-0.0921324906 0.0333010414
-0.0890916165 0.0272834208
-0.0860507424 0.0212658001
-0.0830098684 0.0152481795
-0.0799689943 0.0092305588
-0.0769281202 0.0032129382
-0.0704866949 0.0037299722
-0.0640452695 0.0042470063
-0.0576038441 0.0047640403
-0.0511624187 0.0052810744
-0.0447209934 0.0057981085
-0.0382795680 0.0063151425
-0.0318381426 0.0068321766
-0.0253967172 0.0073492106
-0.0223568083 0.0065652614
-0.0193168994 0.0057813121
-0.0162769905 0.0049973628
-0.0132370815 0.0042134135
-0.0101971726 0.0034294642
-0.0071572637 0.0026455149
-0.0041173548 0.0018615656
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0056398178 0.0025216152
-0.0102021898 0.0039656140
-0.0147645617 0.0054096129
-0.0193269337 0.0068536117
-0.0238893057 0.0082976106
-0.0284516776 0.0097416094
-0.0330140496 0.0111856082
-0.0375764216 0.0126296071
-0.0422887386 0.0191428368
-0.0470010556 0.0256560665
-0.0517133726 0.0321692961
-0.0564256897 0.0386825258
-0.0611380067 0.0451957555
-0.0658503237 0.0517089852
-0.0705626407 0.0582222148
-0.0752749577 0.0647354445
-0.0927804970 0.0773528659
-0.1102860364 0.0899702874
-0.1277915757 0.1025877088
-0.1452971150 0.1152051302
-0.1628026543 0.1278225516
-0.1803081936 0.1404399730
-0.1978137329 0.1530573944
-0.2153192722 0.1656748158
-0.2252334789 0.1702264279
-0.2351476855 0.1747780399
-0.2450618921 0.1793296519
-0.2549760987 0.1838812639
-0.2648903054 0.1884328759
-0.2748045120 0.1929844880
-0.2847187186 0.1975361000
-0.2946329252 0.2020877120
-0.3083703891 0.2198840102
-0.3221078530 0.2376803084
-0.3358453169 0.2554766065
-0.3495827808 0.2732729047
-0.3633202448 0.2910692029
-0.3770577087 0.3088655011
-0.3907951726 0.3266617993
-0.4045326365 0.3444580974
-0.4381292123 0.3723481920
-0.4717257881 0.4002382866
-0.5053223639 0.4281283811
-0.5389189397 0.4560184757
-0.5725155156 0.4839085703
-0.6061120914 0.5117986648
-0.6397086672 0.5396887594
-0.6733052430 0.5675788540
-0.7028557678 0.5708074504
-0.7324062925 0.5740360468
-0.7619568173 0.5772646432
-0.7915073420 0.5804932396
-0.8210578668 0.5837218360
-0.8506083915 0.5869504324
-0.8801589162 0.5901790288
-0.9097094410 0.5934076252
-0.9217879894 0.5955760940
-0.9338665379 0.5977445628
-0.9459450863 0.5999130317
-0.9580236348 0.6020815005
-0.9701021832 0.6042499693
-0.9821807316 0.6064184381
-0.9942592801 0.6085869069
-1.0063378285 0.6107553758
-0.9807453429 0.6020550118
-0.9551528572 0.5933546479
-0.9295603716 0.5846542840
-0.9039678860 0.5759539201
-0.8783754003 0.5672535561
-0.8527829147 0.5585531922
-0.8271904291 0.5498528283
-0.8015979434 0.5411524644
-0.7863563598 0.5261469331
-0.7711147763 0.5111414019
-0.7558731927 0.4961358707
-0.7406316091 0.4811303394
-0.7253900255 0.4661248082
-0.7101484419 0.4511192770
-0.6949068583 0.4361137457
-0.6796652748 0.4211082145
-0.6677607413 0.4116763860
-0.6558562079 0.4022445576
-0.6439516745 0.3928127291
-0.6320471411 0.3833809007
-0.6201426076 0.3739490722
-0.6082380742 0.3645172438
-0.5963335408 0.3550854153
-0.5844290074 0.3456535869
-0.5942770262 0.3385888830
-0.6041250450 0.3315241792
-0.6139730639 0.3244594753
-0.6238210827 0.3173947715
-0.6336691016 0.3103300676
-0.6435171204 0.3032653638
-0.6533651393 0.2962006600
-0.6632131581 0.2891359561
-0.6253335824 0.2678461368
-0.5874540067 0.2465563174
-0.5495744310 0.2252664981
-0.5116948553 0.2039766787
-0.4738152796 0.1826868594
-0.4359357039 0.1613970401
-0.3980561282 0.1401072207
-0.3601765525 0.1188174014
-0.3630228302 0.1209762369
-0.3658691080 0.1231350725
-0.3687153857 0.1252939081
-0.3715616635 0.1274527436
-0.3744079412 0.1296115792
-0.3772542190 0.1317704148
-0.3801004967 0.1339292503
-0.3829467744 0.1360880859
-0.3865051923 0.1362714471
-0.3900636101 0.1364548083
-0.3936220280 0.1366381695
-0.3971804458 0.1368215307
-0.4007388637 0.1370048920
-0.4042972815 0.1371882532
-0.4078556994 0.1373716144
-0.4114141172 0.1375549756
-0.3961902738 0.1296709198
-0.3809664303 0.1217868640
-0.3657425869 0.1139028082
-0.3505187435 0.1060187525
-0.3352949000 0.0981346967
-0.3200710566 0.0902506409
-0.3048472132 0.0823665851
-0.2896233697 0.0744825293
-0.2662001190 0.0690569119
-0.2427768683 0.0636312946
-0.2193536176 0.0582056772
-0.1959303669 0.0527800598
-0.1725071162 0.0473544425
-0.1490838654 0.0419288251
-0.1256606147 0.0365032077
-0.1022373640 0.0310775904


==> data/original_data_sample_0_copy.tex <==
-0.0155124664 0.0020627975
-0.0158786774 0.0022678375
-0.0160255432 0.0024728775
-0.0159950256 0.0027017593
-0.0158386230 0.0029735565
-0.0156078339 0.0032958984
-0.0153427124 0.0036621094
-0.0150814056 0.0040540695
-0.0148468018 0.0044403076
-0.0146522522 0.0047845840
-0.0145053864 0.0050525665
-0.0144119263 0.0052165985
-0.0143814087 0.0052604675
-0.0144214630 0.0051794052
-0.0145416260 0.0049858093
-0.0147438049 0.0046997070
-0.0150260925 0.0043468475
-0.0153751373 0.0039548874
-0.0157718658 0.0035495758
-0.0161895752 0.0031528473
-0.0166034698 0.0027770996
-0.0169887543 0.0024318695
-0.0173244476 0.0021200180
-0.0175914764 0.0018377304
-0.0177745819 0.0015821457
-0.0178680420 0.0013494492
-0.0178585052 0.0011348724
-0.0177421570 0.0009393692
-0.0175266266 0.0007629395
-0.0172214508 0.0006113052
-0.0168476105 0.0004920959
-0.0164299011 0.0004138947
-0.0159950256 0.0003862381
-0.0155715942 0.0004119873
-0.0151824951 0.0004940033
-0.0148410797 0.0006322861
-0.0145473480 0.0008192062
-0.0143013000 0.0010414124
-0.0140972137 0.0012826920
-0.0139198303 0.0015182495
-0.0137462616 0.0017204285
-0.0135536194 0.0018587112
-0.0133171082 0.0019025803
-0.0130157471 0.0018301010
-0.0126361847 0.0016212463
-0.0121574402 0.0012664795
-0.0115623474 0.0007658005
-0.0108318329 0.0001230240
-0.0099411011 -0.0006513596
-0.0088672638 -0.0015430450
-0.0075893402 -0.0025320053
-0.0060844421 -0.0035972595
-0.0043258667 -0.0047292709
-0.0022869110 -0.0059299469
0.0000648499 -0.0072202682
0.0027580261 -0.0086383820
0.0058250427 -0.0102310181
0.0093059540 -0.0120515823
0.0132255554 -0.0141544342
0.0176010132 -0.0165891647
0.0224437714 -0.0193910599
0.0277633667 -0.0225934982
0.0335903168 -0.0262269974
0.0399703979 -0.0303087234
0.0469512939 -0.0348386765
0.0545921326 -0.0397939682
0.0629558563 -0.0451278687
0.0720996857 -0.0507678986
0.0820865631 -0.0566225052
0.0930213928 -0.0626087189
0.1050605774 -0.0686731339
0.1183757782 -0.0747709274
0.1330928802 -0.0808305740
0.1492729187 -0.0867538452
0.1669139862 -0.0924234390
0.1859436035 -0.0977115631
0.2062206268 -0.1024904251
0.2275123596 -0.1066322327
0.2494850159 -0.1100177765
0.2717151642 -0.1125488281
0.2937602997 -0.1141786575
0.3152103424 -0.1149330139
0.3357162476 -0.1149053574
0.3550510406 -0.1142473221
0.3730792999 -0.1131343842
0.3896560669 -0.1116991043
0.4045886993 -0.1099977493
0.4176521301 -0.1080217361
0.4286060333 -0.1057090759
0.4372673035 -0.1029758453
0.4436340332 -0.0997648239
0.4479522705 -0.0960693359
0.4505882263 -0.0919113159
0.4517879486 -0.0872907639
0.4515914917 -0.0821666718
0.4499301910 -0.0764970779
0.4467525482 -0.0702733994
0.4420967102 -0.0635375977
0.4361686707 -0.0563955307
0.4294223785 -0.0490217209
0.4224681854 -0.0416517258
0.4158763885 -0.0345306396
0.4100513458 -0.0278682709
0.4052448273 -0.0218286514
0.4016418457 -0.0165357590
0.3993892670 -0.0120744705
0.3986015320 -0.0084867477
0.3993568420 -0.0057764053
0.4016551971 -0.0039100647
0.4053955078 -0.0028305054
0.4104022980 -0.0024614334
0.4164695740 -0.0027160645
0.4233608246 -0.0035018921
0.4307861328 -0.0047216415
0.4384403229 -0.0062789917
0.4460754395 -0.0080804825
0.4535255432 -0.0100383759
0.4606857300 -0.0120744705
0.4674854279 -0.0141220093
0.4738521576 -0.0161275864
0.4797344208 -0.0180597305
0.4851131439 -0.0199060440
0.4899806976 -0.0216646194
0.4943428040 -0.0233469009
0.4981994629 -0.0249700546
0.5014953613 -0.0265445709
0.5041198730 -0.0280790329
0.5059547424 -0.0295724869
0.5069255829 -0.0310192108
0.5070037842 -0.0324068069
0.5061864853 -0.0337133408
0.5045013428 -0.0349121094
0.5020189285 -0.0359783173
0.4988584518 -0.0368938446
0.4951543808 -0.0376520157
0.4910373688 -0.0382671356
0.4866237640 -0.0387639999
0.4820299149 -0.0391817093
0.4773979187 -0.0395698547
0.4728384018 -0.0399789810
0.4683799744 -0.0404491425
0.4640197754 -0.0410060883
0.4597826004 -0.0416679382
0.4556913376 -0.0424337387
0.4517345428 -0.0432844162
0.4478740692 -0.0441837311
0.4440345764 -0.0450716019
0.4401025772 -0.0458707809
0.4359378815 -0.0465040207
0.4313850403 -0.0469026566
0.4263029099 -0.0470170975
0.4206056595 -0.0468196869
0.4142665863 -0.0463018417
0.4073076248 -0.0454788208
0.3997840881 -0.0443887711
0.3917665482 -0.0430898666
0.3833255768 -0.0416536331
0.3745412827 -0.0401630402
0.3655147552 -0.0387144089
0.3563566208 -0.0374002457
0.3471832275 -0.0362949371
0.3381032944 -0.0354585648
0.3292016983 -0.0349149704
0.3205089569 -0.0346479416
0.3119668961 -0.0346059799
0.3034381866 -0.0346946716
0.2947597504 -0.0348024368
0.2858018875 -0.0348138809
0.2764759064 -0.0346212387
0.2667169571 -0.0341358185
0.2564725876 -0.0332851410
0.2456841469 -0.0320186615
0.2342596054 -0.0303010941
0.2220702171 -0.0281076431
0.2090005875 -0.0254306793
0.1949920654 -0.0222883224
0.1800332069 -0.0187206268
0.1641340256 -0.0147867203
0.1473274231 -0.0105619431
0.1297092438 -0.0061349869
0.1114726067 -0.0016078949
0.0928807259 0.0029172897
0.0742220879 0.0073461533
0.0557909012 0.0116004944
0.0378990173 0.0156173706
0.0208797455 0.0193405151
0.0050721169 0.0227222443
-0.0091938972 0.0257205963
-0.0216150284 0.0282926559
-0.0319352150 0.0303916931
-0.0399718285 0.0319747925
-0.0456280708 0.0330038071
-0.0489034653 0.0334482193
-0.0498967171 0.0332937241
-0.0487985611 0.0325441360
-0.0458836555 0.0312223434
-0.0414943695 0.0293760300
-0.0360207558 0.0270757675
-0.0298748016 0.0244112015
-0.0234665871 0.0214853287
-0.0171918869 0.0184125900
-0.0114107132 0.0153121948
-0.0064163208 0.0122890472
-0.0024132729 0.0094366074
0.0004854202 0.0068321228
0.0022459030 0.0045404434
0.0029101372 0.0026159286
0.0025887489 0.0010948181
0.0014472008 -0.0000009537
-0.0003089905 -0.0006666183
-0.0024552345 -0.0009117126
-0.0047707558 -0.0007572174
-0.0070519447 -0.0002336502
-0.0091209412 0.0006151199
-0.0108332634 0.0017290115
-0.0120763779 0.0030298233
-0.0127706528 0.0044231415
-0.0128741264 0.0058012009
-0.0123810768 0.0070466995
-0.0113205910 0.0080490112
-0.0097560883 0.0087146759
-0.0077800751 0.0089740753
-0.0055093765 0.0087947845
-0.0030827522 0.0081882477
-0.0006523132 0.0072011948
0.0016250610 0.0059137344
0.0035953522 0.0044355392
0.0051264763 0.0028982162
0.0061125755 0.0014438629
0.0064778328 0.0002136230
0.0061812401 -0.0006685257
0.0052270889 -0.0011100769
0.0036730766 -0.0010643005
0.0016283989 -0.0005359650
-0.0007510185 0.0004234314
-0.0032777786 0.0017175674
-0.0057544708 0.0032291412
-0.0079927444 0.0048265457
-0.0098247528 0.0063772202
-0.0111145973 0.0077619553
-0.0117640495 0.0088748932
-0.0117168427 0.0096292496
-0.0109581947 0.0099592209
-0.0095090866 0.0098257065
-0.0074210167 0.0092115402
-0.0047683716 0.0081243515
-0.0016388893 0.0065984726
0.0018653870 0.0046930313
0.0056376457 0.0024919510
0.0095739365 0.0000963211
0.0135731697 -0.0023832321
0.0175437927 -0.0048303604
0.0214076042 -0.0071325302
0.0251021385 -0.0091924667
0.0285882950 -0.0109310150
0.0318608284 -0.0122976303
0.0349540710 -0.0132846832
0.0379271507 -0.0139198303
0.0408401489 -0.0142545700
0.0437469482 -0.0143527985
0.0466933250 -0.0142765045
0.0497226715 -0.0140848160
0.0528750420 -0.0138206482
0.0561795235 -0.0135145187
0.0596489906 -0.0131855011
0.0632848740 -0.0128431320
0.0670814514 -0.0124979019
0.0710177422 -0.0121564865
0.0750570297 -0.0118236542
0.0791583061 -0.0114994049
0.0832953453 -0.0111732483
0.0874481201 -0.0108232498
0.0915846825 -0.0104227066
0.0956668854 -0.0099325180
0.0996580124 -0.0093030930
0.1035146713 -0.0084829330
0.1071748734 -0.0074167252
0.1105651855 -0.0060520172
0.1136193275 -0.0043430328
0.1162772179 -0.0022554398
0.1184787750 0.0002336502
0.1201744080 0.0031270981
0.1213293076 0.0064067841
0.1219286919 0.0100383759
0.1219782829 0.0139646530
0.1214990616 0.0181131363
0.1205258369 0.0224008560
0.1191043854 0.0267391205
0.1172819138 0.0310344696
0.1150913239 0.0351943970
0.1125521660 0.0391244888
0.1096849442 0.0427293777
0.1065258980 0.0459146500
0.1031250954 0.0485801697
0.0995321274 0.0506172180
0.0957875252 0.0519275665
0.0919141769 0.0524396896
0.0879087448 0.0521202087
0.0837450027 0.0509834290
0.0793890953 0.0490989685
0.0748157501 0.0465965271
0.0700149536 0.0436429977
0.0649981499 0.0404186249
0.0597991943 0.0370922089
0.0544757843 0.0337991714
0.0491161346 0.0306386948
0.0438375473 0.0276784897
0.0387716293 0.0249538422
0.0340442657 0.0224809647
0.0297613144 0.0202655792
0.0259947777 0.0182991028
0.0227808952 0.0165710449
0.0201230049 0.0150775909
0.0179944038 0.0138120651
0.0163435936 0.0127611160
0.0151023865 0.0119113922
0.0141973495 0.0112476349
0.0135593414 0.0107555389
0.0131235123 0.0104207993
0.0128264427 0.0102291107
0.0126118660 0.0101718903
0.0124340057 0.0102443695
0.0122556686 0.0104475021
0.0120501518 0.0107851028
0.0117988586 0.0112590790
0.0114917755 0.0118751526
0.0111303329 0.0126390457
0.0107231140 0.0135507584
0.0102887154 0.0146074295
0.0098624229 0.0158033371
0.0094957352 0.0171298981
0.0092601776 0.0185756683
0.0092473030 0.0201234818
0.0095653534 0.0217504501
0.0103421211 0.0234298706
0.0117182732 0.0251331329
0.0138416290 0.0268259048
0.0168609619 0.0284690857
0.0209240913 0.0300216675
0.0261778831 0.0314340591
0.0327672958 0.0326471329
0.0408463478 0.0335931778
0.0505805016 0.0341987610
0.0621442795 0.0343761444
0.0757069588 0.0340261459
0.0914001465 0.0330381393
0.1092944145 0.0312986374
0.1293992996 0.0287218094
0.1516866684 0.0252733231
0.1760964394 0.0209827423
0.2025098801 0.0159387589
0.2307219505 0.0102806091
0.2604353428 0.0041847229
0.2912645340 -0.0021572113
0.3227472305 -0.0085525513
0.3543908596 -0.0148286819
0.3857288361 -0.0208444595
0.4163496494 -0.0264968872
0.4459044933 -0.0317230225
0.4741218090 -0.0364990234
0.5008270741 -0.0408334732
0.5259364843 -0.0447492599
0.5494257212 -0.0482797623
0.5712939501 -0.0514507294
0.5915153027 -0.0542774200
0.6099990010 -0.0567607880
0.6266072989 -0.0588817596
0.6411957145 -0.0606203079
0.6536226869 -0.0619544983
0.6637503505 -0.0628604889
0.6714615226 -0.0633230209
0.6766710877 -0.0633306503
0.6792879105 -0.0628709793
0.6791219711 -0.0619230270
0.6758668423 -0.0604581833
0.6692440510 -0.0584545135
0.6591198444 -0.0559110641
0.6454656124 -0.0528469086
0.6282947063 -0.0492992401
0.6076073647 -0.0453176498
0.5833437443 -0.0409488678
0.5554649830 -0.0362472534
0.5240778923 -0.0312719345
0.4894108772 -0.0260763168
0.4516968727 -0.0206995010
0.4111175537 -0.0151596069
0.3678460121 -0.0094594955
0.3221020699 -0.0035915375
0.2741279602 0.0024557114
0.2241411209 0.0086984634
0.1723961830 0.0151720047
0.1193027496 0.0219259262
0.0654430389 0.0290193558
0.0115146637 0.0365238190
-0.0417156219 0.0444974899
-0.0934362411 0.0529527664
-0.1428122520 0.0618267059
-0.1890234947 0.0709657669
-0.2313175201 0.0801248550
-0.2690558434 0.0889825821
-0.3017225266 0.0971641541
-0.3289008141 0.1042613983
-0.3502626419 0.1098575592
-0.3656525612 0.1135787964
-0.3752012253 0.1151618958
-0.3793115616 0.1144695282
-0.3785572052 0.1114721298
-0.3735766411 0.1062240601
-0.3649928570 0.0988397598
-0.3533840179 0.0894813538
-0.3393096924 0.0783519745
-0.3233563900 0.0657005310
-0.3061304092 0.0518093109
-0.2881734371 0.0369529724
-0.2698824406 0.0213842392
-0.2515234947 0.0053453445
-0.2333045006 -0.0109319687
-0.2154033184 -0.0272302628
-0.1979441643 -0.0433502197
-0.1809830666 -0.0591106415
-0.1645252705 -0.0743541718
-0.1485471725 -0.0889520645
-0.1330046654 -0.1028146744
-0.1178426743 -0.1158828735
-0.1030201912 -0.1280946732
-0.0885375738 -0.1393747330
-0.0744286776 -0.1496448517
-0.0607124567 -0.1588268280
-0.0473554134 -0.1668519974
-0.0342974663 -0.1736936569
-0.0214945078 -0.1794071198
-0.0089174509 -0.1841211319
0.0034688711 -0.1879987717
0.0157119036 -0.1912221909
0.0278638601 -0.1939811707
0.0399748087 -0.1964483261
0.0520837307 -0.1987590790
0.0642060041 -0.2010192871
0.0763206482 -0.2033147812
0.0883598328 -0.2056999207
0.1002061367 -0.2081737518
0.1116991043 -0.2106885910
0.1226544380 -0.2131681442
0.1328835487 -0.2155141830
0.1422028542 -0.2175874710
0.1504511833 -0.2192153931
0.1575281620 -0.2202491760
0.1634213924 -0.2206001282
0.1681869030 -0.2202167511
0.1719112396 -0.2190380096
0.1746971607 -0.2169976234
0.1766686440 -0.2140588760
0.1779541969 -0.2102141380
0.1786580086 -0.2054586411
0.1788630486 -0.1997904778
0.1786537170 -0.1932468414
0.1781227589 -0.1859292984
0.1773493290 -0.1779942513
0.1763796806 -0.1696295738
0.1752142906 -0.1610236168
0.1737966537 -0.1523375511
0.1720209122 -0.1436910629
0.1697583199 -0.1351742744
0.1668879986 -0.1268658638
0.1633005142 -0.1188197136
0.1588826180 -0.1110477448
0.1535348892 -0.1035313606
0.1472048759 -0.0962448120
0.1398944855 -0.0891675949
0.1316528320 -0.0822768211
0.1225614548 -0.0755419731
0.1127190590 -0.0689258575
0.1022357941 -0.0623884201
0.0912475586 -0.0559005737
0.0799160004 -0.0494527817
0.0684051514 -0.0430502892
0.0568747520 -0.0367078781
0.0454759598 -0.0304465294
0.0343370438 -0.0242862701
0.0235600471 -0.0182414055
0.0132260323 -0.0123205185
0.0033841133 -0.0065217018
-0.0059533119 -0.0008244514
-0.0148072243 0.0048017502
-0.0232276917 0.0103864670
-0.0312943459 0.0159583092
-0.0391254425 0.0215458870
-0.0468769073 0.0271806717
-0.0547385216 0.0328984261
-0.0629186630 0.0387363434
-0.0716261864 0.0447306633
-0.0810627937 0.0509171486
-0.0914134979 0.0573344231
-0.1028399467 0.0640249252
-0.1154723167 0.0710315704
-0.1293997765 0.0783972740
-0.1446614265 0.0861563683
-0.1612381935 0.0943322182
-0.1790480614 0.1029357910
-0.1979482174 0.1119599342
-0.2177379131 0.1213793755
-0.2381689548 0.1311469078
-0.2589602470 0.1411895752
-0.2797842026 0.1513957977
-0.3002352715 0.1615920067
-0.3198242188 0.1715302467
-0.3380341530 0.1809043884
-0.3544075489 0.1893897057
-0.3686003685 0.1966724396
-0.3803792000 0.2024569511
-0.3896079063 0.2064714432
-0.3962616920 0.2084956169
-0.4004710913 0.2084040642
-0.4025421143 0.2061929703
-0.4028632641 0.2019443512
-0.4017776251 0.1957693100
-0.3995677233 0.1878070831
-0.3964959979 0.1782360077
-0.3928053379 0.1672725677
-0.3887077570 0.1551542282
-0.3843877316 0.1421279907
-0.3799876869 0.1284503937
-0.3755862713 0.1143712997
-0.3712353408 0.1001281738
-0.3670259714 0.0859565735
-0.3630940318 0.0720958710
-0.3595730960 0.0587739944
-0.3565444350 0.0461797714
-0.3540192246 0.0344514847
-0.3519731760 0.0236825943
-0.3503868580 0.0139350891
-0.3492503166 0.0052375793
-0.3485543728 -0.0024232864
-0.3482867479 -0.0090951920
-0.3484333754 -0.0148468018
-0.3489701748 -0.0197610855
-0.3498516083 -0.0239295959
-0.3510053158 -0.0274410248
-0.3523218632 -0.0303783417
-0.3536336422 -0.0328226089
-0.3547234535 -0.0348529816
-0.3553824425 -0.0365533829
-0.3554494381 -0.0380153656
-0.3547909260 -0.0393409729
-0.3532552719 -0.0406417847
-0.3506605625 -0.0420217514
-0.3468341827 -0.0435762405
-0.3416652679 -0.0453863144
-0.3351283073 -0.0475111008
-0.3272809982 -0.0499763489
-0.3182487488 -0.0527696609
-0.3082003593 -0.0558366776
-0.2973303795 -0.0590753555
-0.2858567238 -0.0623531342
-0.2740249634 -0.0655164719
-0.2620878220 -0.0684003830
-0.2502541542 -0.0708427429
-0.2386522293 -0.0727014542
-0.2273430824 -0.0738649368
-0.2163434029 -0.0742597580
-0.2056336403 -0.0738601685
-0.1951694489 -0.0726814270
-0.1848864555 -0.0707778931
-0.1746997833 -0.0682373047
-0.1645016670 -0.0651702881
-0.1541876793 -0.0617065430
-0.1436967850 -0.0579967499
-0.1330242157 -0.0542087555
-0.1221971512 -0.0505008698
-0.1112399101 -0.0469913483
-0.1001749039 -0.0437502861
-0.0890297890 -0.0408034325
-0.0778450966 -0.0381360054
-0.0666885376 -0.0357050896
-0.0556654930 -0.0334568024
-0.0449252129 -0.0313377380
-0.0346465111 -0.0292935371
-0.0250053406 -0.0272636414
-0.0161466599 -0.0251832008
-0.0081954002 -0.0229992867
-0.0012698174 -0.0206875801
0.0045323372 -0.0182538033
0.0091600418 -0.0157265663
0.0126199722 -0.0131511688
0.0149703026 -0.0105886459
0.0163164139 -0.0081110001
0.0168004036 -0.0057883263
0.0165891647 -0.0036873817
0.0158677101 -0.0018692017
0.0148353577 -0.0003843307
0.0136880875 0.0007286072
0.0126013756 0.0014491081
0.0117211342 0.0017766953
0.0111541748 0.0017290115
0.0109658241 0.0013403893
0.0111789703 0.0006585121
0.0117788315 -0.0002608299
0.0127196312 -0.0013613701
0.0139322281 -0.0025882721
0.0153331757 -0.0038895607
0.0168261528 -0.0052165985
0.0183081627 -0.0065217018
0.0196790695 -0.0077614784
0.0208439827 -0.0088930130
0.0217161179 -0.0098714828
0.0222272873 -0.0106558800
0.0223336220 -0.0112085342
0.0220241547 -0.0114979744
0.0213198662 -0.0115056038
0.0202703476 -0.0112233162
0.0189514160 -0.0106587410
0.0174589157 -0.0098400116
0.0158982277 -0.0088081360
0.0143737793 -0.0076179504
0.0129818916 -0.0063314438
0.0118017197 -0.0050096512
0.0108957291 -0.0037131310
0.0103063583 -0.0024952888
0.0100522041 -0.0013990402
0.0101289749 -0.0004587173
0.0105109215 0.0003056526
0.0111551285 0.0008878708
0.0120067596 0.0012936592
0.0130014420 0.0015392303
0.0140714645 0.0016460419
0.0151486397 0.0016398430
0.0161676407 0.0015478134
0.0170674324 0.0013980865
0.0177936554 0.0012197495
0.0182957649 0.0010414124
0.0185275078 0.0008907318
0.0184531212 0.0007963181
0.0180478096 0.0007805824
0.0173044205 0.0008592606
0.0162358284 0.0010418892
0.0148768425 0.0013260841
0.0132822990 0.0016980171
0.0115232468 0.0021381378
0.0096759796 0.0026235580
0.0078125000 0.0031290054
0.0059971809 0.0036339760
0.0042839050 0.0041265488
0.0027170181 0.0046005249
0.0013256073 0.0050578117
0.0001230240 0.0055074692
-0.0008945465 0.0059628487
-0.0017471313 0.0064396858
-0.0024633408 0.0069522858
-0.0030803680 0.0075139999
-0.0036392212 0.0081362724
-0.0041813850 0.0088267326
-0.0047469139 0.0095901489
-0.0053749084 0.0104274750
-0.0061020851 0.0113377571
-0.0069627762 0.0123171806
-0.0079874992 0.0133600235
-0.0091996193 0.0144629478
-0.0106120110 0.0156226158
-0.0122232437 0.0168352127
-0.0140171051 0.0180907249
-0.0159621239 0.0193753242
-0.0180158615 0.0206708908
-0.0201268196 0.0219526291
-0.0222420692 0.0231971741
-0.0243086815 0.0243825912
-0.0262770653 0.0254898071
-0.0281100273 0.0265111923
-0.0297865868 0.0274548531
-0.0313053131 0.0283432007
-0.0326800346 0.0292053223
-0.0339374542 0.0300717354
-0.0351128578 0.0309734344
-0.0362443924 0.0319352150
-0.0373678207 0.0329728127
-0.0385174751 0.0340967178
-0.0397315025 0.0353126526
-0.0410418510 0.0366210938
-0.0424699783 0.0380125046
-0.0440254211 0.0394687653
-0.0457000732 0.0409650803
-0.0474677086 0.0424623489
-0.0492825508 0.0439119339
-0.0510854721 0.0452613831
-0.0528135300 0.0464620590
-0.0543990135 0.0474720001
-0.0557727814 0.0482473373
-0.0568704605 0.0487518311
-0.0576348305 0.0489568710
-0.0580234528 0.0488424301
-0.0580062866 0.0483989716
-0.0575618744 0.0476198196
-0.0566902161 0.0465154648
-0.0554170609 0.0451173782
-0.0537896156 0.0434741974
-0.0518636703 0.0416431427
-0.0496902466 0.0396747589
-0.0473194122 0.0376157761
-0.0447959900 0.0355091095
-0.0421590805 0.0333919525
-0.0394434929 0.0312881470
-0.0366721153 0.0292110443
-0.0338611603 0.0271673203
-0.0310196877 0.0251502991
-0.0281577110 0.0231542587
-0.0252971649 0.0211811066
-0.0224742889 0.0192451477
-0.0197324753 0.0173664093
-0.0171141624 0.0155639648
-0.0146622658 0.0138587952
-0.0124177933 0.0122671127
-0.0104169846 0.0108060837
-0.0086889267 0.0094919205
-0.0072536469 0.0083341599
-0.0061202049 0.0073404312
-0.0052919388 0.0065183640
-0.0047674179 0.0058746338
-0.0045385361 0.0054121017
-0.0045933723 0.0051317215
-0.0049152374 0.0050344467
-0.0054821968 0.0051145554
-0.0062661171 0.0053586960
-0.0072312355 0.0057497025
-0.0083355904 0.0062599182
-0.0095314980 0.0068578720
-0.0107669830 0.0075063705
-0.0119862556 0.0081634521
-0.0131316185 0.0087842941
-0.0141429901 0.0093212128
-0.0149593353 0.0097322464
-0.0155277252 0.0099802017
-0.0158104897 0.0100393295
-0.0157876015 0.0099029541
-0.0154566765 0.0095758438
-0.0148305893 0.0090723038
-0.0139384270 0.0084161758
-0.0128202438 0.0076351166
-0.0115242004 0.0067634583
-0.0101065636 0.0058364868
-0.0086259842 0.0048904419
-0.0071463585 0.0039653778
-0.0057334900 0.0031003952
-0.0044517517 0.0023336411
-0.0033602715 0.0016994476
-0.0025095940 0.0012226105
-0.0019392967 0.0009241104
-0.0016708374 0.0008115768
-0.0017075539 0.0008783340
-0.0020341873 0.0011091232
-0.0026187897 0.0014801025
-0.0034160614 0.0019588470
-0.0043687820 0.0025081635
-0.0054135323 0.0030927658
-0.0064849854 0.0036754608
-0.0075168610 0.0042200089
-0.0084462166 0.0046949387
-0.0092229843 0.0050754547
-0.0098147392 0.0053443909
-0.0102043152 0.0054922104
-0.0103945732 0.0055246353
-0.0104026794 0.0054531097
-0.0102577209 0.0052967072
-0.0099987984 0.0050821304
-0.0096678734 0.0048351288
-0.0093069077 0.0045824051
-0.0089530945 0.0043487549
-0.0086393356 0.0041542053
-0.0083904266 0.0040140152
-0.0082254410 0.0039396286
-0.0081577301 0.0039396286
-0.0081930161 0.0040187836
-0.0083351135 0.0041780472
-0.0085835457 0.0044136047
-0.0089330673 0.0047187805
-0.0093736649 0.0050840378
-0.0098934174 0.0054950714
-0.0104761124 0.0059366226
-0.0111036301 0.0063886642
-0.0117588043 0.0068340302
-0.0124235153 0.0072593689
-0.0130815506 0.0076551437
-0.0137176514 0.0080146790
-0.0143213272 0.0083341599
-0.0148849487 0.0086154938
-0.0154047012 0.0088653564
-0.0158834457 0.0090932846
-0.0163278580 0.0093097687
-0.0167503357 0.0095243454
-0.0171642303 0.0097513199
-0.0175857544 0.0100030899
-0.0180301666 0.0102844238
-0.0185041428 0.0105981827
-0.0190095901 0.0109443665
-0.0195484161 0.0113172531
-0.0201168060 0.0117073059
-0.0207061768 0.0121059418
-0.0213069916 0.0125017166
-0.0219011307 0.0128784180
-0.0224647522 0.0132207870
-0.0229663849 0.0135087967
-0.0233736038 0.0137233734
-0.0236587524 0.0138521194
-0.0238056183 0.0138902664
-0.0238103867 0.0138425827
-0.0236816406 0.0137176514
-0.0234384537 0.0135297775
-0.0231075287 0.0132980347
-0.0227241516 0.0130405426
-0.0223283768 0.0127782822
-0.0219573975 0.0125284195
-0.0216445923 0.0123033524
-0.0214128494 0.0121154785
-0.0212678909 0.0119695663
-0.0212020874 0.0118618011
-0.0211944580 0.0117826462
-0.0212202072 0.0117216110
-0.0212526321 0.0116682053
-0.0212707520 0.0116119385
-0.0212707520 0.0115489960
-0.0212564468 0.0114822388
-0.0212364197 0.0114173889
-0.0212249756 0.0113611221
-0.0212354660 0.0113220215
-0.0212888718 0.0113115311
-0.0214080811 0.0113439560
-0.0216207504 0.0114364624
-0.0219640732 0.0116100311
-0.0224771500 0.0118894577
-0.0232028961 0.0122976303
-0.0241785049 0.0128555298
-0.0254344940 0.0135803223
-0.0269956589 0.0144824982
-0.0288743973 0.0155668259
-0.0310726166 0.0168333054
-0.0335807800 0.0182743073
-0.0363750458 0.0198745728
-0.0394258499 0.0216169357
-0.0426959991 0.0234813690
-0.0461387634 0.0254421234
-0.0497007370 0.0274677277
-0.0533208847 0.0295200348
-0.0569314957 0.0315580368
-0.0604619980 0.0335359573
-0.0638542175 0.0354137421
-0.0670623779 0.0371570587
-0.0700292587 0.0387248993
-0.0726613998 0.0400581360
-0.0748634338 0.0410985947
-0.0765981674 0.0418205261
-0.0778989792 0.0422391891
-0.0788345337 0.0423936844
-0.0794801712 0.0423278809
-0.0799074173 0.0420856476
-0.0801792145 0.0417079926
-0.0803499222 0.0412340164
-0.0804691315 0.0407009125
-0.0805873871 0.0401430130
-0.0807638168 0.0396013260
-0.0810766220 0.0391225815
-0.0816144943 0.0387487411
-0.0824670792 0.0385198593
-0.0837249756 0.0384654999
-0.0854701996 0.0386037827
-0.0877637863 0.0389394760
-0.0906400681 0.0394639969
-0.0941085815 0.0401535034
-0.0981578827 0.0409774780
-0.1027584076 0.0419054031
-0.1078758240 0.0429067612
-0.1134719849 0.0439558029
-0.1195068359 0.0450286865
-0.1259336472 0.0461063385
-0.1327047348 0.0471706390
-0.1397829056 0.0482034683
-0.1471433640 0.0491933823
-0.1547718048 0.0501260757
-0.1626358032 0.0509710312
-0.1706657410 0.0516881943
-0.1788015366 0.0522356033
-0.1870450974 0.0525875092
-0.1954631805 0.0527448654
-0.2041549683 0.0527315140
-0.2132377625 0.0525941849
-0.2228460312 0.0524053574
-0.2330904007 0.0522527695
-0.2440299988 0.0522260666
-0.2556800842 0.0524158478
-0.2680196762 0.0529050827
-0.2809734344 0.0537548065
-0.2943983078 0.0549983978
-0.3080787659 0.0566349030
-0.3217658997 0.0586271286
-0.3352489471 0.0609216690
-0.3483572006 0.0634498596
-0.3609390259 0.0661191940
-0.3728694916 0.0688247681
-0.3840599060 0.0714502335
-0.3944311142 0.0738658905
-0.4038848877 0.0759410858
-0.4123497009 0.0775537491
-0.4198265076 0.0786066055
-0.4263582230 0.0790328979
-0.4319772720 0.0787878036
-0.4366827011 0.0778446198
-0.4404563904 0.0762023926
-0.4433135986 0.0739049911
-0.4453163147 0.0710353851
-0.4465494156 0.0677089691
-0.4470939636 0.0640621185
-0.4470024109 0.0602350235
-0.4462747574 0.0563602448
-0.4448623657 0.0525512695
-0.4427413940 0.0489110947
-0.4399509430 0.0455312729
-0.4365634918 0.0424852371
-0.4326248169 0.0398187637
-0.4281406403 0.0375499725
-0.4231224060 0.0356769562
-0.4176063538 0.0341815948
-0.4116344452 0.0330410004
-0.4052371979 0.0322313309
-0.3984279633 0.0317220688
-0.3912029266 0.0314836502
-0.3835430145 0.0314903259
-0.3754119873 0.0317125320
-0.3667812347 0.0321283340
-0.3576564789 0.0327177048
-0.3480720520 0.0334634781
-0.3380622864 0.0343503952
-0.3276634216 0.0353622437
-0.3169364929 0.0364866257
-0.3059616089 0.0377063751
-0.2948226929 0.0389995575
-0.2835845947 0.0403385162
-0.2723064423 0.0416936874
-0.2610588074 0.0430297852
-0.2499084473 0.0443143845
-0.2389068604 0.0455141068
-0.2280750275 0.0465927124
-0.2173976898 0.0475168228
-0.2068157196 0.0482454300
-0.1962547302 0.0487375259
-0.1856746674 0.0489635468
-0.1750812531 0.0489110947
-0.1645183563 0.0485830307
-0.1540374756 0.0479898453
-0.1436977386 0.0471525192
-0.1335582733 0.0460968018
-0.1236801147 0.0448532104
-0.1141414642 0.0434598923
-0.1050148010 0.0419578552
-0.0963687897 0.0403909683
-0.0882854462 0.0388088226
-0.0808506012 0.0372638702
-0.0741271973 0.0358028412
-0.0681476593 0.0344610214
-0.0629291534 0.0332679749
-0.0584907532 0.0322504044
-0.0548362732 0.0314226151
-0.0519542694 0.0307893753
-0.0498180389 0.0303487778
-0.0483894348 0.0300951004
-0.0476264954 0.0300197601
-0.0474739075 0.0301132202
-0.0478706360 0.0303640366
-0.0487461090 0.0307607651
-0.0500240326 0.0312919617
-0.0516300201 0.0319423676
-0.0534992218 0.0327024460
-0.0555915833 0.0335721970
-0.0578861237 0.0345611572
-0.0603675842 0.0356750488
-0.0630264282 0.0369167328
-0.0658550262 0.0382909775
-0.0688514709 0.0397939682
-0.0720138550 0.0414209366
-0.0753250122 0.0431575775
-0.0787754059 0.0449829102
-0.0823478699 0.0468730927
-0.0859985352 0.0487928391
-0.0896759033 0.0506954193
-0.0933170319 0.0525312424
-0.0968742371 0.0542669296
-0.1003055573 0.0558710098
-0.1035537720 0.0573062897
-0.1065597534 0.0585374832
-0.1092720032 0.0595321655
-0.1116466522 0.0602617264
-0.1136379242 0.0606927872
-0.1152000427 0.0607948303
-0.1163024902 0.0605497360
-0.1169338226 0.0599546432
-0.1171016693 0.0590229034
-0.1168270111 0.0577859879
-0.1161499023 0.0562915802
-0.1151199341 0.0546016693
-0.1137828827 0.0527820587
-0.1121883392 0.0508985519
-0.1103706360 0.0490179062
-0.1083583832 0.0471973419
-0.1061897278 0.0454902649
-0.1039009094 0.0439367294
-0.1015205383 0.0425615311
-0.0990715027 0.0413713455
-0.0965747833 0.0403556824
-0.0940456390 0.0394945145
-0.0914783478 0.0387516022
-0.0888442993 0.0380735397
-0.0861034393 0.0374059677
-0.0832214355 0.0366954803
-0.0801753998 0.0358943939
-0.0769519806 0.0349721909
-0.0735588074 0.0339050293
-0.0700168610 0.0326900482
-0.0663700104 0.0313377380
-0.0626792908 0.0298709869
-0.0590057373 0.0283222198
-0.0554161072 0.0267276764
-0.0519676208 0.0251245499
-0.0487022400 0.0235462189
-0.0456447601 0.0220203400
-0.0428180695 0.0205726624
-0.0402317047 0.0192260742
-0.0378799438 0.0179891586
-0.0357532501 0.0168666840


==> data/sgru_sample100.tex <==
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0104810525 -0.0073327905
-0.0189628197 -0.0160847728
-0.0274445869 -0.0248367539
-0.0359263541 -0.0335887373
-0.0444081213 -0.0423407207
-0.0528898885 -0.0510927041
-0.0613716557 -0.0598446875
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0698534229 -0.0685966709
-0.0747523961 -0.0711551074
-0.0796513693 -0.0737135438
-0.0845503425 -0.0762719848
-0.0894493158 -0.0788304213
-0.0943482890 -0.0813888578
-0.0992472622 -0.0839472943
-0.1041462354 -0.0865057307
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1090452086 -0.0890641672
-0.1116691341 -0.0859199853
-0.1142930596 -0.0827758034
-0.1169169850 -0.0796316215
-0.1195409105 -0.0764874396
-0.1221648360 -0.0733432577
-0.1247887615 -0.0701990758
-0.1274126869 -0.0670548939
-0.1300366124 -0.0639107120
-0.1203342720 -0.0615955542
-0.1106319317 -0.0592803964
-0.1009295913 -0.0569652386
-0.0912272509 -0.0546500808
-0.0815249105 -0.0523349230
-0.0718225701 -0.0500197652
-0.0621202298 -0.0477046074
-0.0524178894 -0.0453894497
-0.0461155639 -0.0395383695
-0.0398132384 -0.0336872893
-0.0335109129 -0.0278362091
-0.0272085874 -0.0219851289
-0.0209062618 -0.0161340488
-0.0146039363 -0.0102829686
-0.0083016108 -0.0044318884
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0033845266 0.0032142258
-0.0047697679 0.0050092598
-0.0061550092 0.0068042938
-0.0075402504 0.0085993278
-0.0089254917 0.0103943618
-0.0103107330 0.0121893958
-0.0116959743 0.0139844298
-0.0130812156 0.0157794638
-0.0171717163 0.0162536836
-0.0212622171 0.0167279034
-0.0253527179 0.0172021231
-0.0294432186 0.0176763429
-0.0335337194 0.0181505627
-0.0376242202 0.0186247824
-0.0417147188 0.0190990022
-0.0458052217 0.0195732219
-0.0547425239 0.0248452668
-0.0636798260 0.0301173117
-0.0726171282 0.0353893566
-0.0815544303 0.0406614015
-0.0904917281 0.0459334441
-0.0994290258 0.0512054867
-0.1083663235 0.0564775293
-0.1173036213 0.0617495720
-0.1283104054 0.0683981759
-0.1393171894 0.0750467798
-0.1503239735 0.0816953837
-0.1613307576 0.0883439876
-0.1723375417 0.0949925915
-0.1833443258 0.1016411954
-0.1943511099 0.1082897994
-0.2053578939 0.1149384033
-0.2273473906 0.1232428089
-0.2493368873 0.1315472146
-0.2713263840 0.1398516202
-0.2933158806 0.1481560259
-0.3153053773 0.1564604315
-0.3372948916 0.1647648372
-0.3592844060 0.1730692428
-0.3812739203 0.1813736485
-0.3786422330 0.1820049190
-0.3760105456 0.1826361895
-0.3733788583 0.1832674600
-0.3707471709 0.1838987305
-0.3681154836 0.1845300011
-0.3654837963 0.1851612716
-0.3628521089 0.1857925421
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3602204216 0.1864238126
-0.3428682111 0.1844000299
-0.3255160006 0.1823762472
-0.3081637902 0.1803524644
-0.2908115621 0.1783286817
-0.2734593339 0.1763048989
-0.2561071058 0.1742811162
-0.2387548777 0.1722573335
-0.2214026496 0.1702335507
-0.2092827840 0.1636440140
-0.1971629007 0.1570544772
-0.1850430175 0.1504649314
-0.1729231343 0.1438753856
-0.1608032510 0.1372858398
-0.1486833678 0.1306962940
-0.1365634934 0.1241067482
-0.1244436189 0.1175172024
-0.1117308228 0.1188641445
-0.0990180267 0.1202110865
-0.0863052305 0.1215580285
-0.0735924344 0.1229049705
-0.0608796382 0.1242519125
-0.0481668421 0.1255988545
-0.0354540459 0.1269457965
-0.0227412498 0.1282927385
-0.0236352197 0.1339221252
-0.0245291897 0.1395515118
-0.0254231597 0.1451808985
-0.0263171296 0.1508102852
-0.0272110996 0.1564396809
-0.0281050695 0.1620690766
-0.0289990395 0.1676984723
-0.0298930095 0.1733278679
-0.0247904330 0.1785968160
-0.0196878565 0.1838657641
-0.0145852800 0.1891347122
-0.0094827036 0.1944036602
-0.0043801271 0.1996726083
0.0007224494 0.2049415564
0.0058250259 0.2102105045
0.0109276023 0.2154794525
0.0065045997 0.2242520648
0.0020815970 0.2330246770
-0.0023414056 0.2417972892
-0.0067644083 0.2505699015
-0.0111874109 0.2593425137
-0.0156104136 0.2681151259
-0.0200334163 0.2768877382
-0.0244564189 0.2856603504
-0.0284122659 0.2884219898
-0.0323681129 0.2911836291
-0.0363239599 0.2939452685
-0.0402798068 0.2967069079
-0.0442356560 0.2994685472
-0.0481915052 0.3022301866
-0.0521473544 0.3049918260
-0.0561032036 0.3077534653
-0.0552715979 0.3068281673
-0.0544399922 0.3059028692
-0.0536083864 0.3049775712
-0.0527767807 0.3040522731
-0.0519451750 0.3031269751
-0.0511135693 0.3022016951
-0.0502819636 0.3012764151
-0.0494503579 0.3003511351
-0.0601575110 0.3003357615
-0.0708646641 0.3003203880
-0.0815718173 0.3003050145
-0.0922789704 0.3002896410
-0.1029861235 0.3002742675
-0.1136932766 0.3002588940
-0.1244004298 0.3002435204
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1351075829 0.3002281469
-0.1342136174 0.2945987512
-0.1333196518 0.2889693555
-0.1324256863 0.2833399599
-0.1315317207 0.2777105642
-0.1306377552 0.2720811685
-0.1297437896 0.2664517728
-0.1288498241 0.2608223771
-0.1279558586 0.2551929814
-0.1288498241 0.2608223771
-0.1297437896 0.2664517728
-0.1306377552 0.2720811685
-0.1315317207 0.2777105642
-0.1324256863 0.2833399599
-0.1333196518 0.2889693555
-0.1342136174 0.2945987512
-0.1351075829 0.3002281469
-0.1272474802 0.2896694460
-0.1193873775 0.2791107451
-0.1115272747 0.2685520442
-0.1036671720 0.2579933433
-0.0958070693 0.2474346423
-0.0879469666 0.2368759414
-0.0800868638 0.2263172405
-0.0722267655 0.2157585396
-0.0722267699 0.2157585396
-0.0722267744 0.2157585396
-0.0722267788 0.2157585396
-0.0722267832 0.2157585396
-0.0722267876 0.2157585396
-0.0722267920 0.2157585396
-0.0722267964 0.2157585396
-0.0722268008 0.2157585396
-0.0652095007 0.2039000367
-0.0581922006 0.1920415338
-0.0511749004 0.1801830309
-0.0441576003 0.1683245281
-0.0371403001 0.1564660252
-0.0301230000 0.1446075223
-0.0231056998 0.1327490194
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0160883997 0.1208905165
-0.0174025325 0.1150003665
-0.0187166653 0.1091102165
-0.0200307981 0.1032200664
-0.0213449309 0.0973299164
-0.0226590636 0.0914397664
-0.0239731964 0.0855496164
-0.0252873292 0.0796594664
-0.0266014620 0.0737693163
-0.0295054328 0.0681913236
-0.0324094035 0.0626133308
-0.0353133743 0.0570353381
-0.0382173450 0.0514573453
-0.0411213158 0.0458793526
-0.0440252865 0.0403013598
-0.0469292573 0.0347233671
-0.0498332280 0.0291453743
-0.0444076224 0.0265493566
-0.0389820168 0.0239533390
-0.0335564112 0.0213573213
-0.0281308056 0.0187613024
-0.0227051999 0.0161652836
-0.0172795943 0.0135692648
-0.0118539887 0.0109732460
-0.0064283837 0.0083772272
-0.0064283842 0.0083772266
-0.0064283848 0.0083772261
-0.0064283853 0.0083772255
-0.0064283859 0.0083772249
-0.0064283864 0.0083772244
-0.0064283870 0.0083772238
-0.0064283875 0.0083772232
-0.0064283881 0.0083772227
-0.0050431468 0.0065821887
-0.0036579055 0.0047871547
-0.0022726642 0.0029921206
-0.0008874230 0.0011970868
0.0004978183 -0.0005979471
0.0018830596 -0.0023929810
0.0032683009 -0.0041880148
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0046535422 -0.0059830488
0.0087283956 -0.0074853973
0.0128032496 -0.0089877459
0.0168781030 -0.0104900938
0.0209529564 -0.0119924423
0.0250278098 -0.0134947908
0.0291026632 -0.0149971393
0.0331775166 -0.0164994878
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0456426815 -0.0239975259
0.0540329929 -0.0299932155
0.0624233043 -0.0359889050
0.0708136157 -0.0419845946
0.0792039271 -0.0479802842
0.0875942385 -0.0539759738
0.0959845499 -0.0599716633
0.1043748613 -0.0659673529
0.1017509359 -0.0628231710
0.0991270104 -0.0596789891
0.0965030849 -0.0565348072
0.0938791594 -0.0533906253
0.0912552340 -0.0502464434
0.0886313085 -0.0471022615
0.0860073830 -0.0439580796
0.0833834575 -0.0408138977
0.0927053694 -0.0390034767
0.1020272812 -0.0371930556
0.1113491931 -0.0353826345
0.1206711049 -0.0335722135
0.1299930168 -0.0317617924
0.1393149286 -0.0299513714
0.1486368493 -0.0281409503
0.1579587700 -0.0263305292
0.1414852309 -0.0234944086
0.1250116918 -0.0206582880
0.1085381528 -0.0178221674
0.0920646137 -0.0149860467
0.0755910747 -0.0121499261
0.0591175312 -0.0093138055
0.0426439877 -0.0064776849
0.0261704442 -0.0036415642
0.0140492431 0.0010966434
0.0019280419 0.0058348510
-0.0101931593 0.0105730587
-0.0223143604 0.0153112663
-0.0344355616 0.0200494739
-0.0465567628 0.0247876815
-0.0586779617 0.0295258892
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0707991607 0.0342640968
-0.0668433159 0.0315024574
-0.0628874712 0.0287408181
-0.0589316264 0.0259791787
-0.0549757816 0.0232175393
-0.0510199368 0.0204559000
-0.0470640921 0.0176942606
-0.0431082473 0.0149326213
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0391524025 0.0121709819
-0.0336766583 0.0099017281
-0.0282009140 0.0076324743
-0.0227251697 0.0053632206
-0.0172494266 0.0030939668
-0.0117736834 0.0008247130
-0.0062979403 -0.0014445407
-0.0008221971 -0.0037137945
0.0046535460 -0.0059830483
0.0046535455 -0.0059830483
0.0046535449 -0.0059830483
0.0046535444 -0.0059830483
0.0046535438 -0.0059830483
0.0046535433 -0.0059830483
0.0046535427 -0.0059830483
0.0046535422 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0046535416 -0.0059830483
0.0087283950 -0.0074853968
0.0128032485 -0.0089877453
0.0168781019 -0.0104900938
0.0209529564 -0.0119924423
0.0250278098 -0.0134947908
0.0291026632 -0.0149971393
0.0331775166 -0.0164994878
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0372523701 -0.0180018363
0.0448473684 -0.0195368197
0.0524423668 -0.0210718031
0.0600373652 -0.0226067865
0.0676323636 -0.0241417699
0.0752273620 -0.0256767533
0.0828223603 -0.0272117367
0.0904173587 -0.0287467201
0.0980123571 -0.0302817035
0.1144858962 -0.0331178241
0.1309594352 -0.0359539447
0.1474329743 -0.0387900654
0.1639065133 -0.0416261860
0.1803800524 -0.0444623066
0.1968535915 -0.0472984272
0.2133271305 -0.0501345479
0.2298006696 -0.0529706685
0.2530785476 -0.0652062466
0.2763564256 -0.0774418246
0.2996343036 -0.0896774027
0.3229121992 -0.1019129808
0.3461900949 -0.1141485589
0.3694679906 -0.1263841370
0.3927458862 -0.1386197150
0.4160237819 -0.1508552931
0.4164658285 -0.1594401482
0.4169078751 -0.1680249942
0.4173499217 -0.1766098402
0.4177919683 -0.1851946862
0.4182340149 -0.1937795323
0.4186760616 -0.2023643783
0.4191181082 -0.2109492243
0.4195601548 -0.2195340703
0.4476937815 -0.2347433322
0.4758274082 -0.2499525941
0.5039610349 -0.2651618560
0.5320946616 -0.2803711180
0.5602282883 -0.2955803799
0.5883619151 -0.3107896237
0.6164955771 -0.3259988676
0.6446291685 -0.3412081115
0.6861513858 -0.3495806875
0.7276736031 -0.3579532635
0.7691958204 -0.3663258395
0.8107180377 -0.3746984155
0.8522402550 -0.3830709915
0.8937624723 -0.3914435675
0.9352846896 -0.3998161435
0.9768069068 -0.4081887195
0.9778358882 -0.4144393893
0.9788648696 -0.4206900592
0.9798938510 -0.4269407290
0.9809228324 -0.4331913988
0.9819518137 -0.4394420686
0.9829807951 -0.4456927384
0.9840097765 -0.4519434082
0.9850387579 -0.4581940780
0.9891060812 -0.4547103525
0.9931734046 -0.4512266270
0.9972407279 -0.4477429015
1.0013080513 -0.4442591760
1.0053753746 -0.4407754505
1.0094426980 -0.4372917250
1.0135100213 -0.4338079995
1.0175773447 -0.4303242740
1.0068701739 -0.4303396836
0.9961630031 -0.4303550932
0.9854558323 -0.4303705028
0.9747486615 -0.4303859124
0.9640414907 -0.4304013220
0.9533343199 -0.4304167316
0.9426271492 -0.4304321412
0.9319199784 -0.4304475508
0.8922055781 -0.4194715095
0.8524911778 -0.4084954681
0.8127767775 -0.3975194267
0.7730623772 -0.3865433853
0.7333479769 -0.3755673440
0.6936335766 -0.3645913026
0.6539191763 -0.3536152612
0.6142047760 -0.3426392199
0.5814933972 -0.3302691686
0.5487820184 -0.3178991174
0.5160706397 -0.3055290661
0.4833592609 -0.2931590329
0.4506478821 -0.2807889997
0.4179365033 -0.2684189665
0.3852251245 -0.2560489333
0.3525137457 -0.2436789001
0.3148983869 -0.2176881657
0.2772830280 -0.1916974312
0.2396676692 -0.1657066967
0.2020523104 -0.1397159623
0.1644369516 -0.1137252278
0.1268216016 -0.0877344933
0.0892062517 -0.0617437589
0.0515909017 -0.0357530267
0.0515909061 -0.0357530289
0.0515909105 -0.0357530312
0.0515909149 -0.0357530334
0.0515909193 -0.0357530357
0.0515909238 -0.0357530379
0.0515909282 -0.0357530402
0.0515909326 -0.0357530425
0.0515909370 -0.0357530447
0.0489670115 -0.0326088628
0.0463430861 -0.0294646809
0.0437191606 -0.0263204990
0.0410952351 -0.0231763171
0.0384713096 -0.0200321352
0.0358473841 -0.0168879544
0.0332234587 -0.0137437737
0.0305995332 -0.0105995929
0.0265246820 -0.0090972449
0.0224498308 -0.0075948970
0.0183749785 -0.0060925491
0.0143001261 -0.0045902011
0.0102252738 -0.0030878532
0.0061504215 -0.0015855051
0.0020755692 -0.0000831570
-0.0019992831 0.0014191911
-0.0033845247 0.0032142252
-0.0047697662 0.0050092592
-0.0061550080 0.0068042932
-0.0075402493 0.0085993272
-0.0089254906 0.0103943618
-0.0103107319 0.0121893958
-0.0116959732 0.0139844298
-0.0130812144 0.0157794638
-0.0211275633 0.0190153230
-0.0291739133 0.0222511821
-0.0372202632 0.0254870412
-0.0452666154 0.0287229004
-0.0533129676 0.0319587595
-0.0613593197 0.0351946186
-0.0694056719 0.0384304777
-0.0774520241 0.0416663369
-0.0873433336 0.0509662364
-0.0972346432 0.0602661359
-0.1071259528 0.0695660354
-0.1170172623 0.0788659349
-0.1269085719 0.0881658389
-0.1367998814 0.0974657429
-0.1466911910 0.1067656469
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1565824917 0.1160655509
-0.1454434292 0.1091121291
-0.1343043667 0.1021587074
-0.1231653042 0.0952052856
-0.1120262417 0.0882518638
-0.1008871792 0.0812984420
-0.0897481167 0.0743450157
-0.0786090541 0.0673915894
-0.0674699916 0.0604381632
-0.0606713924 0.0548558263
-0.0538727932 0.0492734895
-0.0470741940 0.0436911526
-0.0402755948 0.0381088158
-0.0334769978 0.0325264789
-0.0266784007 0.0269441421
-0.0198798037 0.0213618052
-0.0130812067 0.0157794684
-0.0130812078 0.0157794684
-0.0130812089 0.0157794684
-0.0130812100 0.0157794684
-0.0130812111 0.0157794684
-0.0130812122 0.0157794684
-0.0130812133 0.0157794684
-0.0130812144 0.0157794684
-0.0130812156 0.0157794684
-0.0116959743 0.0139844343
-0.0103107330 0.0121894003
-0.0089254917 0.0103943663
-0.0075402504 0.0085993318
-0.0061550092 0.0068042972
-0.0047697679 0.0050092626
-0.0033845266 0.0032142280
-0.0019992853 0.0014191935
-0.0019992853 0.0014191932
-0.0019992853 0.0014191929
-0.0019992853 0.0014191926
-0.0019992853 0.0014191923
-0.0019992853 0.0014191921
-0.0019992853 0.0014191918
-0.0019992853 0.0014191915
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912
-0.0019992853 0.0014191912


==> data/sgru_sample53.tex <==
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0034026376 -0.0018734519
-0.0048059899 -0.0051660956
-0.0062093422 -0.0084587393
-0.0076126945 -0.0117513830
-0.0090160468 -0.0150440267
-0.0104193991 -0.0183366704
-0.0118227514 -0.0216293141
-0.0132261037 -0.0249219578
-0.0118227514 -0.0216293141
-0.0104193991 -0.0183366704
-0.0090160468 -0.0150440267
-0.0076126945 -0.0117513830
-0.0062093422 -0.0084587393
-0.0048059899 -0.0051660956
-0.0034026376 -0.0018734519
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0060897861 0.0018934115
-0.0101802869 0.0023676313
-0.0142707876 0.0028418511
-0.0183612884 0.0033160708
-0.0224517892 0.0037902906
-0.0265422899 0.0042645103
-0.0306327907 0.0047387301
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0347232915 0.0052129499
-0.0306327907 0.0047387301
-0.0265422899 0.0042645103
-0.0224517892 0.0037902906
-0.0183612884 0.0033160708
-0.0142707876 0.0028418511
-0.0101802869 0.0023676313
-0.0060897861 0.0018934115
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918


==> data/sgru_sample62.tex <==
-0.0709508129 -0.0055474912
-0.0660518397 -0.0029890536
-0.0611528665 -0.0004306160
-0.0562538933 0.0021278216
-0.0513549201 0.0046862592
-0.0464559468 0.0072446968
-0.0415569736 0.0098031344
-0.0366580004 0.0123615720
-0.0311822540 0.0100923182
-0.0257065075 0.0078230645
-0.0202307610 0.0055538107
-0.0147550145 0.0032845569
-0.0092792681 0.0010153031
-0.0038035216 -0.0012539506
0.0016722249 -0.0035232044
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0071479713 -0.0057924582
0.0112228225 -0.0072948067
0.0152976737 -0.0087971552
0.0193725250 -0.0102995037
0.0234473762 -0.0118018522
0.0275222274 -0.0133042007
0.0315970786 -0.0148065492
0.0356719298 -0.0163088977
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0397467810 -0.0178112462
0.0423707065 -0.0209554281
0.0449946319 -0.0240996100
0.0476185574 -0.0272437919
0.0502424829 -0.0303879738
0.0528664084 -0.0335321557
0.0554903339 -0.0366763376
0.0581142593 -0.0398205195
0.0607381848 -0.0429647014
0.0602305420 -0.0452174088
0.0597228993 -0.0474701162
0.0592152565 -0.0497228236
0.0587076137 -0.0519755310
0.0581999710 -0.0542282384
0.0576923282 -0.0564809458
0.0571846855 -0.0587336532
0.0566770427 -0.0609863606
0.0503747172 -0.0668374453
0.0440723917 -0.0726885299
0.0377700662 -0.0785396146
0.0314677406 -0.0843906993
0.0251654151 -0.0902417840
0.0188630896 -0.0960928687
0.0125607641 -0.1019439534
0.0062584386 -0.1077950381
0.0014384406 -0.1148920452
-0.0033815574 -0.1219890524
-0.0082015554 -0.1290860596
-0.0130215534 -0.1361830668
-0.0178415514 -0.1432800739
-0.0226615494 -0.1503770811
-0.0274815463 -0.1574740883
-0.0323015454 -0.1645710955
-0.0247805518 -0.1746432390
-0.0172595583 -0.1847153826
-0.0097385648 -0.1947875261
-0.0022175712 -0.2048596697
0.0053034223 -0.2149318132
0.0128244159 -0.2250039568
0.0203454094 -0.2350761003
0.0278664030 -0.2451482438
0.0185295678 -0.2506926882
0.0091927338 -0.2562371326
-0.0001441002 -0.2617815770
-0.0094809342 -0.2673260214
-0.0188177682 -0.2728704657
-0.0281546033 -0.2784149101
-0.0374914384 -0.2839593545
-0.0468282735 -0.2895037989
-0.0452946738 -0.2948198238
-0.0437610740 -0.3001358488
-0.0422274743 -0.3054518738
-0.0406938745 -0.3107678987
-0.0391602748 -0.3160839237
-0.0376266750 -0.3213999486
-0.0360930753 -0.3267159736
-0.0345594755 -0.3320319985
-0.0300349483 -0.3390169162
-0.0255104210 -0.3460018338
-0.0209858938 -0.3529867514
-0.0164613666 -0.3599716691
-0.0119368393 -0.3669565867
-0.0074123116 -0.3739415044
-0.0028877838 -0.3809264220
0.0016367440 -0.3879113396
-0.0104509499 -0.3901746750
-0.0225386444 -0.3924380103
-0.0346263388 -0.3947013456
-0.0467140311 -0.3969646809
-0.0588017277 -0.3992280163
-0.0708894244 -0.4014913516
-0.0829771211 -0.4037546869
-0.0950648177 -0.4060180223
-0.1089674752 -0.4088508634
-0.1228701326 -0.4116837045
-0.1367727900 -0.4145165456
-0.1506754386 -0.4173493867
-0.1645780960 -0.4201822279
-0.1784807534 -0.4230150690
-0.1923834108 -0.4258479101
-0.2062860682 -0.4286807512
-0.2258088282 -0.4330139538
-0.2453315882 -0.4373471563
-0.2648543482 -0.4416803588
-0.2843771082 -0.4460135613
-0.3038998682 -0.4503467639
-0.3234226106 -0.4546799664
-0.3429453529 -0.4590131689
-0.3624680953 -0.4633463714
-0.3444396930 -0.4618421486
-0.3264112907 -0.4603379258
-0.3083828885 -0.4588337030
-0.2903544862 -0.4573294801
-0.2723260839 -0.4558252573
-0.2542976817 -0.4543210345
-0.2362692794 -0.4528168116
-0.2182408772 -0.4513125888
-0.2268202372 -0.4510982979
-0.2353995973 -0.4508840069
-0.2439789574 -0.4506697160
-0.2525583174 -0.4504554250
-0.2611376775 -0.4502411341
-0.2697170376 -0.4500268431
-0.2782963977 -0.4498125522
-0.2868757577 -0.4495982613
-0.2774976231 -0.4397805386
-0.2681194885 -0.4299628159
-0.2587413539 -0.4201450932
-0.2493632194 -0.4103273706
-0.2399850848 -0.4005096479
-0.2306069502 -0.3906919252
-0.2212288156 -0.3808742026
-0.2118506810 -0.3710564799
-0.1811843197 -0.3479057320
-0.1505179584 -0.3247549841
-0.1198515970 -0.3016042362
-0.0891852357 -0.2784534883
-0.0585188744 -0.2553027404
-0.0278525131 -0.2321519925
0.0028138482 -0.2090012445
0.0334802095 -0.1858504966
0.0285329520 -0.1664787468
0.0235856945 -0.1471069970
0.0186384371 -0.1277352471
0.0136911796 -0.1083634973
0.0087439221 -0.0889917475
0.0037966646 -0.0696199977
-0.0011505929 -0.0502482478
-0.0060978504 -0.0308765002
-0.0052737262 -0.0268157153
-0.0044496020 -0.0227549303
-0.0036254778 -0.0186941453
-0.0028013535 -0.0146333603
-0.0019772293 -0.0105725753
-0.0011531051 -0.0065117903
-0.0003289809 -0.0024510051
0.0004951433 0.0016097802
0.0004951433 0.0016097805
0.0004951433 0.0016097807
0.0004951433 0.0016097810
0.0004951433 0.0016097813
0.0004951433 0.0016097816
0.0004951433 0.0016097819
0.0004951433 0.0016097822
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0004951433 0.0016097824
0.0045699945 0.0001074339
0.0086448457 -0.0013949146
0.0127196969 -0.0028972631
0.0167945481 -0.0043996116
0.0208693993 -0.0059019601
0.0249442505 -0.0074043086
0.0290191018 -0.0089066571
0.0330939530 -0.0104090062
0.0357178784 -0.0135531869
0.0383418039 -0.0166973677
0.0409657294 -0.0198415474
0.0435896549 -0.0229857293
0.0462135803 -0.0261299112
0.0488375058 -0.0292740931
0.0514614313 -0.0324182750
0.0540853568 -0.0355624569
0.0648228200 -0.0368047660
0.0755602833 -0.0380470752
0.0862977509 -0.0392893844
0.0970352098 -0.0405316935
0.1077726686 -0.0417740027
0.1185101275 -0.0430163119
0.1292475863 -0.0442586210
0.1399850451 -0.0455009302
0.1458350720 -0.0437475779
0.1516850989 -0.0419942256
0.1575351258 -0.0402408733
0.1633851527 -0.0384875210
0.1692351795 -0.0367341665
0.1750852064 -0.0349808119
0.1809352333 -0.0332274574
0.1867852602 -0.0314741029
0.1995917550 -0.0353117215
0.2123982498 -0.0391493401
0.2252047447 -0.0429869587
0.2380112395 -0.0468245774
0.2508177343 -0.0506621960
0.2636242292 -0.0544998146
0.2764307240 -0.0583374333
0.2892372189 -0.0621750519
0.2940943451 -0.0639130171
0.2989514714 -0.0656509824
0.3038085800 -0.0673889476
0.3086656885 -0.0691269129
0.3135227971 -0.0708648781
0.3183799057 -0.0726028433
0.3232370143 -0.0743408086
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3280941229 -0.0760787783
0.3414142607 -0.0722412815
0.3547343985 -0.0684037847
0.3680545363 -0.0645662878
0.3813746742 -0.0607287910
0.3946948120 -0.0568912942
0.4080149498 -0.0530537973
0.4213350876 -0.0492163005
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4346552254 -0.0453788037
0.4549169609 -0.0427174621
0.4751786964 -0.0400561205
0.4954404319 -0.0373947811
0.5157021674 -0.0347334418
0.5359639029 -0.0320721024
0.5562256384 -0.0294107631
0.5764873739 -0.0267494237
0.5967491094 -0.0240880844
0.6163396687 -0.0244923068
0.6359302280 -0.0248965293
0.6555207873 -0.0253007517
0.6751113467 -0.0257049742
0.6947019060 -0.0261091966
0.7142924653 -0.0265134191
0.7338830246 -0.0269176415
0.7534735840 -0.0273218639
0.7615660570 -0.0317748518
0.7696585300 -0.0362278396
0.7777510030 -0.0406808275
0.7858434760 -0.0451338153
0.7939359490 -0.0495868032
0.8020284220 -0.0540397910
0.8101208950 -0.0584927789
0.8182133680 -0.0629457667
0.8256218079 -0.0553694062
0.8330302478 -0.0477930458
0.8404386877 -0.0402166853
0.8478471275 -0.0326403248
0.8552555674 -0.0250639644
0.8626640073 -0.0174876039
0.8700724472 -0.0099112434
0.8774808870 -0.0023348830
0.9141030450 0.0004000540
0.9507252029 0.0031349910
0.9873473609 0.0058699281
1.0239695188 0.0086048651
1.0605916768 0.0113398015
1.0972138347 0.0140747380
1.1338359927 0.0168096744
1.1704581506 0.0195446109
1.1784555386 0.0132549028
1.1864529266 0.0069651947
1.1944503852 0.0006754866
1.2024478438 -0.0056142215
1.2104453024 -0.0119039295
1.2184427609 -0.0181936376
1.2264402195 -0.0244833457
1.2344376781 -0.0307730538
1.2305578405 -0.0333287882
1.2266780028 -0.0358845226
1.2227981652 -0.0384402592
1.2189183275 -0.0409959936
1.2150384899 -0.0435517280
1.2111586522 -0.0461074624
1.2072788145 -0.0486631967
1.2033989769 -0.0512189311
1.2299063736 -0.0640110413
1.2564137704 -0.0768031470
1.2829211671 -0.0895952573
1.3094285638 -0.1023873675
1.3359359606 -0.1151794777
1.3624433573 -0.1279715879
1.3889507541 -0.1407636981
1.4154581508 -0.1535558083
1.4066463233 -0.1644248125
1.3978344958 -0.1752938167
1.3890226683 -0.1861628208
1.3802108408 -0.1970318250
1.3713990133 -0.2079008291
1.3625871858 -0.2187698333
1.3537753583 -0.2296388375
1.3449635308 -0.2405078416
1.2838155035 -0.2149041697
1.2226674762 -0.1893004978
1.1615193782 -0.1636968260
1.1003712803 -0.1380931541
1.0392231823 -0.1124894822
0.9780750844 -0.0868858103
0.9169269864 -0.0612821384
0.8557788884 -0.0356784665
0.8508965604 -0.0308966126
0.8460142324 -0.0261147587
0.8411319044 -0.0213329048
0.8362495763 -0.0165510498
0.8313672483 -0.0117691947
0.8264849203 -0.0069873397
0.8216025922 -0.0022054847
0.8167202642 0.0025763703
0.7962357217 0.0086099845
0.7757511792 0.0146435987
0.7552666366 0.0206772123
0.7347820941 0.0267108259
0.7142975516 0.0327444396
0.6938130091 0.0387780554
0.6733284665 0.0448116691
0.6528439240 0.0508452827
0.6491266352 0.0437812871
0.6454093463 0.0367172937
0.6416920575 0.0296533004
0.6379747687 0.0225893070
0.6342574798 0.0155253136
0.6305401910 0.0084613203
0.6268229022 0.0013973269
0.6231056133 -0.0056666664
0.6050519563 -0.0080672515
0.5869982993 -0.0104678365
0.5689446423 -0.0128684215
0.5508909852 -0.0152690065
0.5328373282 -0.0176695915
0.5147836712 -0.0200701765
0.4967300142 -0.0224707616
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4786763571 -0.0248713466
0.4582046009 -0.0240623017
0.4377328447 -0.0232532569
0.4172610885 -0.0224442120
0.3967893323 -0.0216351672
0.3763175761 -0.0208261223
0.3558458199 -0.0200170775
0.3353740637 -0.0192080326
0.3149023075 -0.0183989889
0.3069049196 -0.0121092819
0.2989075316 -0.0058195744
0.2909101260 0.0004701331
0.2829127204 0.0067598406
0.2749153148 0.0130495481
0.2669179091 0.0193392562
0.2589205035 0.0256289643
0.2509230979 0.0319186724
0.2469850330 0.0291727088
0.2430469681 0.0264267452
0.2391089032 0.0236807816
0.2351708384 0.0209348180
0.2312327735 0.0181888532
0.2272947086 0.0154428885
0.2233566437 0.0126969237
0.2194185788 0.0099509590
0.2039672217 0.0162729028
0.1885158647 0.0225948465
0.1730645077 0.0289167903
0.1576131506 0.0352387340
0.1421618024 0.0415606800
0.1267104542 0.0478826238
0.1112591060 0.0542045675
0.0958077578 0.0605265113
0.0801295317 0.0589019257
0.0644513057 0.0572773402
0.0487730797 0.0556527546
0.0330948515 0.0540281690
0.0174166232 0.0524035835
0.0017383950 0.0507789979
-0.0139398333 0.0491544124
-0.0296180615 0.0475298268
-0.0275509549 0.0435610326
-0.0254838484 0.0395922383
-0.0234167418 0.0356234441
-0.0213496352 0.0316546498
-0.0192825286 0.0276858556
-0.0172154232 0.0237170614
-0.0151483177 0.0197482671
-0.0130812122 0.0157794717
-0.0130812122 0.0157794706
-0.0130812122 0.0157794695
-0.0130812122 0.0157794684
-0.0130812122 0.0157794672
-0.0130812122 0.0157794661
-0.0130812122 0.0157794650
-0.0130812122 0.0157794638
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0130812122 0.0157794627
-0.0116959710 0.0139844287
-0.0103107297 0.0121893947
-0.0089254890 0.0103943607
-0.0075402482 0.0085993267
-0.0061550075 0.0068042927
-0.0047697668 0.0050092587
-0.0033845260 0.0032142247
-0.0019992852 0.0014191908
-0.0019992852 0.0014191909
-0.0019992852 0.0014191911
-0.0019992852 0.0014191912
-0.0019992852 0.0014191913
-0.0019992852 0.0014191915
-0.0019992852 0.0014191916
-0.0019992852 0.0014191918
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0019992852 0.0014191919
-0.0033845266 0.0032142258
-0.0047697679 0.0050092598
-0.0061550092 0.0068042938
-0.0075402504 0.0085993278
-0.0089254917 0.0103943618
-0.0103107330 0.0121893958
-0.0116959743 0.0139844298
-0.0130812156 0.0157794638
-0.0171717163 0.0162536836
-0.0212622171 0.0167279034
-0.0253527179 0.0172021231
-0.0294432186 0.0176763429
-0.0335337194 0.0181505627
-0.0376242202 0.0186247824
-0.0417147188 0.0190990022
-0.0458052217 0.0195732219
-0.0575852739 0.0276659643
-0.0693653261 0.0357587067
-0.0811453739 0.0438514513
-0.0929254305 0.0519441914
-0.1047054871 0.0600369315
-0.1164855436 0.0681296716
-0.1282656002 0.0762224117
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1400456568 0.0843151518
-0.1360898077 0.0815535125
-0.1321339585 0.0787918731
-0.1281781093 0.0760302338
-0.1242222601 0.0732685944
-0.1202664109 0.0705069550
-0.1163105617 0.0677453157
-0.1123547125 0.0649836763
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1083988633 0.0622220369
-0.1070136221 0.0604270029
-0.1056283808 0.0586319689
-0.1042431395 0.0568369349
-0.1028578982 0.0550419009
-0.1014726569 0.0532468669
-0.1000874157 0.0514518329
-0.0987021744 0.0496567989
-0.0973169331 0.0478617649
-0.0854022315 0.0420564444
-0.0734875256 0.0362511238
-0.0615728196 0.0304458033
-0.0496581136 0.0246404828
-0.0377434076 0.0188351623
-0.0258287017 0.0130298407
-0.0139139957 0.0072245190
-0.0019992897 0.0014191974
-0.0019992892 0.0014191967
-0.0019992886 0.0014191960
-0.0019992881 0.0014191953
-0.0019992875 0.0014191946
-0.0019992870 0.0014191939
-0.0019992864 0.0014191932
-0.0019992859 0.0014191925
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0019992853 0.0014191918
-0.0074750274 0.0036884455
-0.0129507694 0.0059576993
-0.0184265115 0.0082269531
-0.0239022535 0.0104962069
-0.0293779956 0.0127654606
-0.0348537376 0.0150347144
-0.0403294775 0.0173039682
-0.0458052217 0.0195732219
-0.0538625147 0.0215379623
-0.0619198076 0.0235027027
-0.0699771006 0.0254674431
-0.0780343935 0.0274321836
-0.0860916865 0.0293969240
-0.0941489795 0.0313616644
-0.1022062724 0.0333264048
-0.1102635654 0.0352911452
-0.1223834398 0.0418806910
-0.1345033142 0.0484702367
-0.1466231886 0.0550597825
-0.1587430630 0.0616493283
-0.1708629463 0.0682388741
-0.1829828295 0.0748284199
-0.1951027127 0.0814179657
-0.2072225960 0.0880075115
-0.2275159794 0.0953806916
-0.2478093628 0.1027538627
-0.2681027462 0.1101270339
-0.2883961296 0.1175002050
-0.3086895131 0.1248733761
-0.3289828965 0.1322465472
-0.3492762799 0.1396197183
-0.3695696633 0.1469928894
-0.3887004447 0.1654616256
-0.4078312261 0.1839303617
-0.4269620075 0.2023990979
-0.4460927889 0.2208678341
-0.4652235703 0.2393365702
-0.4843543517 0.2578053064
-0.5034851331 0.2762740426
-0.5226159145 0.2947427787
-0.5570651387 0.3105515897
-0.5915143629 0.3263604007
-0.6259636224 0.3421692118
-0.6604128820 0.3579780228
-0.6948621415 0.3737868338
-0.7293114011 0.3895956448
-0.7637606606 0.4054044558
-0.7982099201 0.4212132669
-0.8276476462 0.4264899558
-0.8570853722 0.4317666448
-0.8865230983 0.4370433337
-0.9159608243 0.4423200227
-0.9453985503 0.4475967117
-0.9748362764 0.4528734006
-1.0042740024 0.4581500896
-1.0337117285 0.4634267786
-1.0867840251 0.4883699847
-1.1398563217 0.5133131908
-1.1929286890 0.5382563969
-1.2460009856 0.5631996031
-1.2990732822 0.5881428092
-1.3521455788 0.6130860153
-1.4052178755 0.6380292215
-1.4582901721 0.6629724276
-1.4524401099 0.6647258024
-1.4465900477 0.6664791773
-1.4407399855 0.6682325521
-1.4348899233 0.6699859270
-1.4290398611 0.6717393018
-1.4231897989 0.6734926767
-1.4173397367 0.6752460515
-1.4114896745 0.6769994264
-1.3931025133 0.6655584985
-1.3747153522 0.6541175707
-1.3563281910 0.6426766428
-1.3379410299 0.6312357149
-1.3195538687 0.6197947871
-1.3011667076 0.6083538592
-1.2827795464 0.5969129675
-1.2643923853 0.5854720757
-1.2436299344 0.5756715309
-1.2228674836 0.5658709862
-1.2021050327 0.5560704414
-1.1813425819 0.5462698967
-1.1605801310 0.5364693519
-1.1398176801 0.5266688072
-1.1190552293 0.5168682624
-1.0982927784 0.5070677177
-1.0444234910 0.4814371060
-0.9905542036 0.4558064944
-0.9366849162 0.4301758828
-0.8828156288 0.4045452711
-0.8289463413 0.3789146595
-0.7750770539 0.3532840478
-0.7212077665 0.3276534362
-0.6673384791 0.3020228426
-0.6614630562 0.2938830527
-0.6555876332 0.2857432808
-0.6497122103 0.2776035089
-0.6438367874 0.2694637370
-0.6379613645 0.2613239651
-0.6320859416 0.2531841933
-0.6262105186 0.2450444214
-0.6203350957 0.2369046495
-0.6265481907 0.2284560540
-0.6327612856 0.2200074584
-0.6389743806 0.2115588629
-0.6451874756 0.2031102674
-0.6514005705 0.1946616719
-0.6576136655 0.1862130764
-0.6638267605 0.1777644808
-0.6700398554 0.1693158853
-0.6550164165 0.1624218374
-0.6399929775 0.1555277895
-0.6249695386 0.1486337507
-0.6099460996 0.1417397118
-0.5949226606 0.1348456730
-0.5798992217 0.1279516341
-0.5648757827 0.1210575952
-0.5498523437 0.1141635564
-0.5283610723 0.1078917841
-0.5068698008 0.1016200117
-0.4853785293 0.0953482394
-0.4638872579 0.0890764671
-0.4423959864 0.0828046948
-0.4209047150 0.0765329225
-0.3994134435 0.0702611457
-0.3779221720 0.0639893688
-0.3538213244 0.0554239382
-0.3297204768 0.0468585076
-0.3056196291 0.0382930769
-0.2815187638 0.0297276463
-0.2574178985 0.0211622156
-0.2333170332 0.0125967850
-0.2092161679 0.0040313544
-0.1851153026 -0.0045340763
-0.1811594534 -0.0072957145
-0.1772036042 -0.0100573528
-0.1732477551 -0.0128189910
-0.1692919059 -0.0155806292
-0.1653360567 -0.0183422675
-0.1613802075 -0.0211039057
-0.1574243583 -0.0238655428
-0.1534685091 -0.0266271822


==> data/target_sample100.tex <==
-0.5420970917 -0.0844650269
-0.5507707596 -0.0886783600
-0.5646486282 -0.0939598083
-0.5832338333 -0.1002655029
-0.6040091515 -0.1072044373
-0.6226391792 -0.1140708923
-0.6346549988 -0.1201190948
-0.6378736496 -0.1249637604
-0.6330556870 -0.1287136078
-0.6224994659 -0.1317443848
-0.6087713242 -0.1345005035
-0.5944232941 -0.1374588013
-0.5820016861 -0.1411151886
-0.5739049911 -0.1459217072
-0.5718889236 -0.1521396637
-0.5762720108 -0.1596431732
-0.5852394104 -0.1677436829
-0.5948715210 -0.1752147675
-0.6006450653 -0.1807231903
-0.5998277664 -0.1835346222
-0.5924968719 -0.1837940216
-0.5804443359 -0.1821823120
-0.5658283234 -0.1795043945
-0.5507211685 -0.1765384674
-0.5371341705 -0.1740398407
-0.5270671844 -0.1727352142
-0.5222997665 -0.1732616425
-0.5238103867 -0.1759700775
-0.5310878754 -0.1807098389
-0.5417051315 -0.1866855621
-0.5515670776 -0.1925277710
-0.5564594269 -0.1968078613
-0.5542402267 -0.1987590790
-0.5454244614 -0.1984901428
-0.5318803787 -0.1965656281
-0.5156593323 -0.1936225891
-0.4987087250 -0.1902961731
-0.4828643799 -0.1872119904
-0.4697437286 -0.1849498749
-0.4604511261 -0.1839256287
-0.4550819397 -0.1841659546
-0.4522705078 -0.1851158142
-0.4492511749 -0.1856575012
-0.4429454803 -0.1845493317
-0.4316577911 -0.1811122894
-0.4157409668 -0.1755123138
-0.3967838287 -0.1684188843
-0.3765907288 -0.1605758667
-0.3568000793 -0.1526622772
-0.3388824463 -0.1452884674
-0.3241481781 -0.1390113831
-0.3136100769 -0.1342716217
-0.3076496124 -0.1312370300
-0.3056774139 -0.1296806335
-0.3059806824 -0.1288890839
-0.3059310913 -0.1277618408
-0.3028964996 -0.1252155304
-0.2955455780 -0.1207180023
-0.2841739655 -0.1144371033
-0.2698993683 -0.1068859100
-0.2539291382 -0.0985965729
-0.2373695374 -0.0900573730
-0.2212638855 -0.0817146301
-0.2065486908 -0.0739517212
-0.1938953400 -0.0670547485
-0.1834812164 -0.0611324310
-0.1748180389 -0.0560550690
-0.1667652130 -0.0514736176
-0.1578979492 -0.0469398499
-0.1471748352 -0.0421142578
-0.1343650818 -0.0369167328
-0.1198883057 -0.0314807892
-0.1043872833 -0.0260066986
-0.0884647369 -0.0206842422
-0.0726642609 -0.0156774521
-0.0574779510 -0.0111198425
-0.0433292389 -0.0071048737
-0.0305366516 -0.0036792755
-0.0192623138 -0.0008583069
-0.0095386505 0.0013751984
-0.0013122559 0.0030612946
0.0054836273 0.0042581558
0.0108585358 0.0050468445
0.0147838593 0.0055246353
0.0172672272 0.0058012009
0.0184001923 0.0059766769
0.0183410645 0.0061407089
0.0173072815 0.0063676834
0.0155353546 0.0067071915
0.0132503510 0.0071897507
0.0106544495 0.0078220367
0.0079154968 0.0085811615
0.0051975250 0.0094108582
0.0026512146 0.0102310181
0.0004119873 0.0109615326
-0.0014095306 0.0115413666
-0.0027427673 0.0119495392
-0.0035686493 0.0121994019
-0.0039005280 0.0123081207
-0.0037708282 0.0123023987
-0.0032501221 0.0122203827
-0.0024223328 0.0121059418
-0.0013751984 0.0120010376
-0.0001983643 0.0119132996
0.0010261536 0.0118064880
0.0022220612 0.0116138458
0.0033168793 0.0112743378
0.0042552948 0.0107688904
0.0050086975 0.0101356506
0.0055675507 0.0094375610
0.0059394836 0.0087299347
0.0061454773 0.0080604553
0.0062141418 0.0074653625
0.0061855316 0.0069732666
0.0060977936 0.0066032410
0.0059776306 0.0063591003
0.0058288574 0.0062217712
0.0056400299 0.0061492920
0.0053920746 0.0060977936
0.0050659180 0.0060291290
0.0046710968 0.0059375763
0.0042266846 0.0058441162
0.0037479401 0.0057659149
0.0032558441 0.0057296753
0.0027675629 0.0057601929
0.0022964478 0.0058727264
0.0018520355 0.0060882568
0.0014438629 0.0064182281
0.0010738373 0.0068492889
0.0007362366 0.0073471069
0.0004215240 0.0078582764
0.0001201630 0.0083236694
-0.0001697540 0.0087108612
-0.0004444122 0.0090217590
-0.0007019043 0.0092658997
-0.0009365082 0.0094680786
-0.0011405945 0.0096511841
-0.0013217926 0.0098419189
-0.0014781952 0.0100708008
-0.0016136169 0.0103530884
-0.0017318726 0.0106868744
-0.0018253326 0.0110378265
-0.0018920898 0.0113334656
-0.0019207001 0.0114994049
-0.0019054413 0.0115013123
-0.0018539429 0.0113430023
-0.0017642975 0.0110607147
-0.0016403198 0.0106983185
-0.0014839172 0.0102882385
-0.0012969971 0.0098686218
-0.0010929108 0.0094814301
-0.0008811951 0.0091629028
-0.0006771088 0.0089397430
-0.0004959106 0.0088100433
-0.0003452301 0.0087509155
-0.0002365112 0.0087089539
-0.0001754761 0.0086174011
-0.0001678467 0.0084533691
-0.0002136230 0.0082302094
-0.0003051758 0.0079727173
-0.0004329681 0.0077133179
-0.0005912781 0.0074863434
-0.0007762909 0.0073146820
-0.0009803772 0.0072212219
-0.0011997223 0.0072231293
-0.0014362335 0.0073223114
-0.0016880035 0.0074939728
-0.0019397736 0.0076885223
-0.0021839142 0.0078582764
-0.0024242401 0.0079746246
-0.0026645660 0.0080451965
-0.0029182434 0.0080890656
-0.0031948090 0.0081291199
-0.0034999847 0.0081863403
-0.0038452148 0.0082778931
-0.0042362213 0.0084266663
-0.0046710968 0.0086441040
-0.0051403046 0.0089302063
-0.0056266785 0.0092658997
-0.0060901642 0.0095939636
-0.0064792633 0.0098419189
-0.0067558289 0.0099563599
-0.0069103241 0.0099239349
-0.0069522858 0.0097618103
-0.0069007874 0.0095062256
-0.0067844391 0.0091934204
-0.0066242218 0.0088558197
-0.0064487457 0.0085239410
-0.0062808990 0.0082302094
-0.0061378479 0.0080032349
-0.0060272217 0.0078430176
-0.0059299469 0.0077285767
-0.0058059692 0.0076103210
-0.0056095123 0.0074253082
-0.0053119659 0.0071315765
-0.0049114227 0.0067253113
-0.0044384003 0.0062370300
-0.0039310455 0.0057144165
-0.0034294128 0.0052013397
-0.0029678345 0.0047302246
-0.0025672913 0.0043315887
-0.0022449493 0.0040283203
-0.0020103455 0.0038242340
-0.0018596649 0.0037136078
-0.0017814636 0.0036754608
-0.0017509460 0.0036716461
-0.0017414093 0.0036678314
-0.0017356873 0.0036373138
-0.0017127991 0.0035724640
-0.0016651154 0.0034790039
-0.0015926361 0.0033702850
-0.0014953613 0.0032634735
-0.0013847351 0.0031700134
-0.0012741089 0.0031051636
-0.0011730194 0.0030899048
-0.0010948181 0.0031280518
-0.0010471344 0.0032157898
-0.0010280609 0.0033359528
-0.0010452271 0.0034656525
-0.0010910034 0.0035877228
-0.0011539459 0.0036830902
-0.0012340546 0.0037498474
-0.0013217926 0.0037975311
-0.0014057159 0.0038299561
-0.0014858246 0.0038566589
-0.0015659332 0.0038967133
-0.0016517639 0.0039691925
-0.0017547607 0.0040950775
-0.0018806458 0.0042781830
-0.0020294189 0.0045185089
-0.0021991730 0.0047969818
-0.0023899078 0.0050888062
-0.0026035309 0.0053939819
-0.0028610229 0.0057258606
-0.0031890869 0.0061130524
-0.0036125183 0.0065822601
-0.0041599274 0.0071659088
-0.0048580170 0.0079002380
-0.0057296753 0.0088195801
-0.0067863464 0.0099430084
-0.0080223083 0.0112724304
-0.0094127655 0.0127735138
-0.0109100342 0.0143718719
-0.0124549866 0.0159988403
-0.0140209198 0.0176124573
-0.0156154633 0.0192203522
-0.0172710419 0.0208606720
-0.0190200806 0.0225772858
-0.0209007263 0.0244178772
-0.0229701996 0.0264492035
-0.0252895355 0.0287590027
-0.0279216766 0.0314216614
-0.0308990479 0.0344753265
-0.0341739655 0.0378780365
-0.0375919342 0.0414638519
-0.0409088135 0.0449638367
-0.0438842773 0.0481147766
-0.0464344025 0.0508155823
-0.0486679077 0.0531711578
-0.0507850647 0.0553894043
-0.0530033112 0.0576953888
-0.0555496216 0.0603179932
-0.0586433411 0.0634822845
-0.0624809265 0.0673866272
-0.0671997070 0.0721530914
-0.0727977753 0.0777626038
-0.0790710449 0.0839824677
-0.0856227875 0.0903606415
-0.0920066833 0.0963973999
-0.0979614258 0.1018009186
-0.1034984589 0.1065654755
-0.1087779999 0.1108493805
-0.1140193939 0.1148777008
-0.1194839478 0.1189289093
-0.1254730225 0.1233196259
-0.1323146820 0.1284027100
-0.1402912140 0.1344985962
-0.1494922638 0.1417388916
-0.1596336365 0.1498985291
-0.1699161530 0.1582679749
-0.1790561676 0.1656875610
-0.1856937408 0.1709194183
-0.1890525818 0.1732769012
-0.1892242432 0.1728878021
-0.1868972778 0.1704006195
-0.1829738617 0.1666412354
-0.1783962250 0.1624717712
-0.1741199493 0.1587429047
-0.1710376740 0.1562652588
-0.1698474884 0.1556739807
-0.1708393097 0.1572246552
-0.1737270355 0.1606559753
-0.1775627136 0.1650886536
-0.1808528900 0.1691474915
-0.1821517944 0.1714859009
-0.1808433533 0.1715164185
-0.1773567200 0.1696090698
-0.1726741791 0.1666488647
-0.1678695679 0.1636390686
-0.1640052795 0.1615962982
-0.1621189117 0.1615390778
-0.1631507874 0.1644134521
-0.1678009033 0.1709365845
-0.1763343811 0.1813907623
-0.1884193420 0.1954479218
-0.2030735016 0.2121047974
-0.2187500000 0.2297763824
-0.2336139679 0.2465667725
-0.2459850311 0.2607154846
-0.2548675537 0.2711715698
-0.2603130341 0.2779941559
-0.2632808685 0.2822151184
-0.2651367188 0.2853012085
-0.2672233582 0.2886810303
-0.2705631256 0.2934379578
-0.2755508423 0.2999668121
-0.2816734314 0.3076820374
-0.2875480652 0.3150539398
-0.2915992737 0.3203449249
-0.2930202484 0.3226966858
-0.2921161652 0.3224811554
-0.2897930145 0.3207321167
-0.2870311737 0.3185749054
-0.2847671509 0.3170738220
-0.2839221954 0.3172626495
-0.2854213715 0.3201847076
-0.2901020050 0.3267669678
-0.2984142303 0.3375034332
-0.3100490570 0.3520298004
-0.3236579895 0.3688068390
-0.3369293213 0.3852043152
-0.3474388123 0.3984432220
-0.3538856506 0.4070167542
-0.3564968109 0.4111385345
-0.3563652039 0.4120025635
-0.3547782898 0.4110355377
-0.3530063629 0.4096603394
-0.3522987366 0.4093132019
-0.3538665771 0.4114112854
-0.3586158752 0.4170265198
-0.3666992188 0.4263782501
-0.3771190643 0.4383506775
-0.3876953125 0.4504489899
-0.3958129883 0.4596710205
-0.3997440338 0.4640254974
-0.3993797302 0.4633827209
-0.3957996368 0.4589824677
-0.3905067444 0.4525470734
-0.3849868774 0.4457893372
-0.3805694580 0.4402408600
-0.3784675598 0.4373016357
-0.3797378540 0.4382076263
-0.3849449158 0.4436302185
-0.3936500549 0.4530830383
-0.4040641785 0.4645175934
-0.4132041931 0.4745311737
-0.4180564880 0.4796657562
-0.4171752930 0.4782714844
-0.4111137390 0.4710063934
-0.4014739990 0.4597167969
-0.3900070190 0.4463977814
-0.3783721924 0.4329452515
-0.3681488037 0.4211483002
-0.3607559204 0.4125995636
-0.3572235107 0.4084453583
-0.3577919006 0.4089202881
-0.3615036011 0.4129085541
-0.3662757874 0.4179763794
-0.3697662354 0.4214038849
-0.3707237244 0.4216957092
-0.3694229126 0.4190635681
-0.3669700623 0.4146728516
-0.3646621704 0.4098892212
-0.3638381958 0.4061164856
-0.3658714294 0.4048423767
-0.3720855713 0.4075012207
-0.3834915161 0.4152221680
-0.4003944397 0.4283905029
-0.4219436646 0.4461479187
-0.4458312988 0.4660873413
-0.4685058594 0.4844932556
-0.4864196777 0.4976997375
-0.4977684021 0.5039215088
-0.5028533936 0.5036315918
-0.5029754639 0.4983482361
-0.4995613098 0.4896697998
-0.4941291809 0.4792289734
-0.4884147644 0.4688415527
-0.4841995239 0.4603157043
-0.4827957153 0.4550132751
-0.4844207764 0.4532432556
-0.4877281189 0.4538230896
-0.4899063110 0.4541969299
-0.4878425598 0.4514694214
-0.4799346924 0.4440612793
-0.4668045044 0.4323692322
-0.4503860474 0.4179878235
-0.4328765869 0.4027481079
-0.4163475037 0.3883514404
-0.4026451111 0.3763580322
-0.3933067322 0.3680763245
-0.3894538879 0.3644599915
-0.3914909363 0.3658599854
-0.3987197876 0.3716049194
-0.4090728760 0.3797416687
-0.4192428589 0.3872070312
-0.4258346558 0.3908843994
-0.4269790649 0.3891372681
-0.4227752686 0.3822212219
-0.4144058228 0.3714141846
-0.4032783508 0.3581886292
-0.3907966614 0.3439674377
-0.3784141541 0.3301544189
-0.3675918579 0.3181037903
-0.3594932556 0.3088760376
-0.3545188904 0.3028450012
-0.3519210815 0.2993850708
-0.3497924805 0.2968673706
-0.3457870483 0.2932548523
-0.3383750916 0.2871589661
-0.3274459839 0.2783889771
-0.3138580322 0.2675743103
-0.2987251282 0.2555923462
-0.2830810547 0.2432670593
-0.2678756714 0.2313880920
-0.2540435791 0.2207527161
-0.2424049377 0.2120590210
-0.2333869934 0.2056655884
-0.2267074585 0.2013130188
-0.2212829590 0.1980361938
-0.2156448364 0.1944961548
-0.2087135315 0.1896781921
-0.2003173828 0.1833572388
-0.1909751892 0.1759147644
-0.1813621521 0.1679000854
-0.1720619202 0.1598396301
-0.1635513306 0.1522102356
-0.1562461853 0.1454772949
-0.1505165100 0.1400871277
-0.1465644836 0.1363601685
-0.1442947388 0.1343269348
-0.1431312561 0.1335716248
-0.1419868469 0.1332130432
-0.1395072937 0.1320838928
-0.1345443726 0.1291809082
-0.1266670227 0.1241264343
-0.1161460876 0.1171569824
-0.1035652161 0.1087722778
-0.0895805359 0.0995140076
-0.0748367310 0.0899009705
-0.0599327087 0.0804214478
-0.0453987122 0.0714874268
-0.0316314697 0.0633659363
-0.0188713074 0.0561294556
-0.0072288513 0.0496063232
0.0032386780 0.0434646606
0.0124511719 0.0374145508
0.0202751160 0.0313644409
0.0265655518 0.0254554749
0.0312118530 0.0199279785
0.0342063904 0.0149650574
0.0356521606 0.0106697083
0.0357475281 0.0070838928
0.0347824097 0.0041999817
0.0330848694 0.0019454956
0.0309524536 0.0002250671
0.0285720825 -0.0010528564
0.0260543823 -0.0019989014
0.0234870911 -0.0027084351
0.0210304260 -0.0032653809
0.0189437866 -0.0037460327
0.0174751282 -0.0042152405
0.0168228149 -0.0047225952
0.0171127319 -0.0053138733
0.0184097290 -0.0060272217
0.0207290649 -0.0068778992
0.0240516663 -0.0078849792
0.0283241272 -0.0090522766
0.0334129333 -0.0103569031
0.0390892029 -0.0117454529
0.0450172424 -0.0131263733
0.0508460999 -0.0144119263
0.0563507080 -0.0155487061
0.0614700317 -0.0165328979
0.0662460327 -0.0173912048
0.0707817078 -0.0181694031
0.0752410889 -0.0189208984
0.0798454285 -0.0197067261
0.0848388672 -0.0205917358
0.0904159546 -0.0216217041
0.0965995789 -0.0228118896
0.1031227112 -0.0240898132
0.1093902588 -0.0253181458
0.1146850586 -0.0263252258
0.1185455322 -0.0269851685
0.1209220886 -0.0272865295
0.1220741272 -0.0272712708
0.1223793030 -0.0270195007
0.1222686768 -0.0266304016
0.1222229004 -0.0262107849
0.1227111816 -0.0258750916
0.1241264343 -0.0257186890
0.1266250610 -0.0257797241
0.1299858093 -0.0260162354
0.1335411072 -0.0263061523
0.1362495422 -0.0264358521
0.1370773315 -0.0262031555
0.1355590820 -0.0255279541
0.1319541931 -0.0244522095
0.1268806458 -0.0231094360
0.1209983826 -0.0216369629
0.1149291992 -0.0201416016
0.1092491150 -0.0187301636
0.1044616699 -0.0174827576
0.1009178162 -0.0164413452
0.0987434387 -0.0156135559
0.0977363586 -0.0149536133
0.0973358154 -0.0143470764
0.0967712402 -0.0136604309
0.0953521729 -0.0127639771
0.0927810669 -0.0116004944
0.0891838074 -0.0101928711
0.0848808289 -0.0085716248
0.0801696777 -0.0067825317
0.0753402710 -0.0048522949
0.0706748962 -0.0028076172
0.0663986206 -0.0006752014
0.0626564026 0.0015449524
0.0593910217 0.0038414001
0.0563125610 0.0061988831
0.0529708862 0.0085983276
0.0489044189 0.0110282898
0.0438804626 0.0135040283
0.0379753113 0.0160751343
0.0313873291 0.0188369751
0.0242996216 0.0218887329
0.0168457031 0.0253295898
0.0091247559 0.0292625427
0.0012016296 0.0337867737
-0.0068855286 0.0389595032
-0.0151023865 0.0447616577
-0.0233917236 0.0510368347
-0.0316200256 0.0574569702
-0.0395965576 0.0635986328
-0.0471191406 0.0690650940
-0.0539970398 0.0736389160
-0.0601043701 0.0773162842
-0.0653839111 0.0802116394
-0.0698127747 0.0824890137
-0.0734329224 0.0843544006
-0.0763664246 0.0860671997
-0.0787887573 0.0879058838
-0.0808067322 0.0900192261
-0.0823326111 0.0923309326
-0.0829963684 0.0944442749
-0.0822105408 0.0956802368
-0.0794372559 0.0953636169
-0.0745391846 0.0931930542
-0.0678939819 0.0893821716
-0.0601158142 0.0843925476
-0.0518150330 0.0786972046
-0.0435295105 0.0727386475
-0.0357131958 0.0669174194
-0.0287246704 0.0615768433
-0.0228233337 0.0569458008
-0.0181579590 0.0530929565
-0.0147819519 0.0498847961
-0.0126571655 0.0469856262
-0.0116195679 0.0440216064
-0.0114364624 0.0407447815
-0.0118103027 0.0371055603
-0.0124282837 0.0331764221
-0.0130233765 0.0290718079
-0.0133781433 0.0249099731
-0.0133514404 0.0207862854
-0.0129051208 0.0168190002
-0.0120925903 0.0131187439
-0.0110015869 0.0097732544
-0.0097312927 0.0068473816
-0.0083541870 0.0043449402
-0.0069236755 0.0022659302
-0.0054893494 0.0006065369
-0.0041389465 -0.0006523132
-0.0030059814 -0.0015258789
-0.0021934509 -0.0020446777
-0.0017585754 -0.0022583008
-0.0017051697 -0.0022239685
-0.0019760132 -0.0020103455
-0.0024948120 -0.0016899109
-0.0031738281 -0.0013237000
-0.0038986206 -0.0009651184
-0.0045585632 -0.0006637573
-0.0050392151 -0.0004653931
-0.0052375793 -0.0003890991
-0.0050888062 -0.0004463196
-0.0045967102 -0.0006217957
-0.0038261414 -0.0008926392
-0.0028457642 -0.0012359619
-0.0017242432 -0.0016250610
-0.0005264282 -0.0020561218
0.0006980896 -0.0025138855
0.0019111633 -0.0029869080
0.0030822754 -0.0034713745
0.0041656494 -0.0039520264
0.0051155090 -0.0044021606
0.0058860779 -0.0047912598
0.0064239502 -0.0050773621
0.0067100525 -0.0052452087
0.0067634583 -0.0053176880
0.0066261292 -0.0053176880
0.0063514709 -0.0052757263
0.0060195923 -0.0052375793
0.0056991577 -0.0052375793
0.0054550171 -0.0053100586
0.0053558350 -0.0054855347
0.0054512024 -0.0057792664
0.0057678223 -0.0061759949
0.0063056946 -0.0066375732
0.0070419312 -0.0071334839
0.0079307556 -0.0076065063
0.0089149475 -0.0080299377
0.0099220276 -0.0083961487
0.0109062195 -0.0086936951
0.0118331909 -0.0089378357
0.0126838684 -0.0091514587
0.0134735107 -0.0093650818
0.0142326355 -0.0096130371
0.0149841309 -0.0099334717
0.0157318115 -0.0103302002
0.0164299011 -0.0107727051
0.0169944763 -0.0112075806
0.0173568726 -0.0115737915
0.0175247192 -0.0118522644
0.0175704956 -0.0120544434
0.0175781250 -0.0121994019
0.0176429749 -0.0123176575
0.0178108215 -0.0124397278
0.0181198120 -0.0125923157
0.0185890198 -0.0128021240
0.0192070007 -0.0130844116
0.0199203491 -0.0134277344
0.0206069946 -0.0137748718
0.0210876465 -0.0140228271
0.0211715698 -0.0140686035
0.0207595825 -0.0138664246
0.0198516846 -0.0134239197
0.0185203552 -0.0127830505
0.0168533325 -0.0120124817
0.0149688721 -0.0111808777
0.0129928589 -0.0103645325
0.0110473633 -0.0096321106
0.0092620850 -0.0090484619
0.0077323914 -0.0086555481
0.0065155029 -0.0084609985
0.0056381226 -0.0084495544
0.0051040649 -0.0085639954
0.0048904419 -0.0087432861
0.0049667358 -0.0089416504
0.0052680969 -0.0091400146
0.0057334900 -0.0093269348
0.0063209534 -0.0094909668
0.0069694519 -0.0096321106
0.0076484680 -0.0097579956
0.0083503723 -0.0098800659
0.0090408325 -0.0100021362
0.0096855164 -0.0101089478
0.0102157593 -0.0101699829
0.0105361938 -0.0101127625
0.0105743408 -0.0098609924
0.0102920532 -0.0094070435
0.0097389221 -0.0087776184
0.0090065002 -0.0080299377
0.0081939697 -0.0072288513
0.0073890686 -0.0064315796
0.0066680908 -0.0056991577
0.0061035156 -0.0050735474
0.0057411194 -0.0045890808
0.0056152344 -0.0042724609
0.0057373047 -0.0041275024
0.0060920715 -0.0041389465
0.0066413879 -0.0042762756
0.0073242188 -0.0045013428
0.0081062317 -0.0047874451
0.0089721680 -0.0051269531
0.0099143982 -0.0055274963
0.0109519958 -0.0059928894
0.0121192932 -0.0065383911
0.0134658813 -0.0071945190
0.0150642395 -0.0079917908
0.0170021057 -0.0089645386
0.0193328857 -0.0101394653
0.0220603943 -0.0115203857
0.0251235962 -0.0130538940
0.0284156799 -0.0146789551
0.0318565369 -0.0163536072
0.0354804993 -0.0180778503
0.0394287109 -0.0199165344
0.0438957214 -0.0219650269
0.0490722656 -0.0243148804
0.0551338196 -0.0270462036
0.0622673035 -0.0302429199
0.0706138611 -0.0339622498
0.0802116394 -0.0382270813
0.0909271240 -0.0429534912
0.1023216248 -0.0479202271
0.1136665344 -0.0527801514
0.1241989136 -0.0571556091
0.1334800720 -0.0608291626
0.1415977478 -0.0638160706
0.1489868164 -0.0663070679
0.1562538147 -0.0685653687
0.1641845703 -0.0709228516
0.1737785339 -0.0738029480
0.1861763000 -0.0776939392
0.2024421692 -0.0830535889
0.2232475281 -0.0901756287
0.2485961914 -0.0990829468
0.2776565552 -0.1094589233
0.3086395264 -0.1206054688
0.3389778137 -0.1315040588
0.3662796021 -0.1412124634
0.3897094727 -0.1493797302
0.4103355408 -0.1563987732
0.4302101135 -0.1630401611
0.4515647888 -0.1701278687
0.4766044617 -0.1784934998
0.5072555542 -0.1888694763
0.5445404053 -0.2016563416
0.5878982544 -0.2166595459
0.6347236633 -0.2329483032
0.6805534363 -0.2489013672
0.7206954956 -0.2627983093
0.7525863647 -0.2737159729
0.7765922546 -0.2817993164
0.7948074341 -0.2878150940
0.8098487854 -0.2927169800
0.8244743347 -0.2975044250
0.8414916992 -0.3031997681
0.8636016846 -0.3107910156
0.8928184509 -0.3210067749
0.9293136597 -0.3339347839
0.9703178406 -0.3485984802
1.0101509094 -0.3629646301
1.0425376892 -0.3748016357
1.0641136169 -0.3829269409
1.0754737854 -0.3875617981
1.0792961121 -0.3896751404
1.0786933899 -0.3903961182
1.0769271851 -0.3908958435
1.0774230957 -0.3924140930
1.0837898254 -0.3962554932
1.0994644165 -0.4036598206
1.1264915466 -0.4153671265
1.1639022827 -0.4310226440
1.2066459656 -0.4487533569
1.2460174561 -0.4653396606
1.2729473114 -0.4774322510
1.2828216553 -0.4833183289
1.2769260406 -0.4834899902
1.2597064972 -0.4796257019
1.2361793518 -0.4736251831
1.2114353180 -0.4674301147
1.1907711029 -0.4630775452
1.1794033051 -0.4625968933
1.1815090179 -0.4676132202
1.1987113953 -0.4787406921
1.2287330627 -0.4950599670
1.2647933960 -0.5138511658
1.2965507507 -0.5309448242
1.3140373230 -0.5422897339
1.3127765656 -0.5460205078
1.2948684692 -0.5429306030
1.2657318115 -0.5351715088
1.2312202454 -0.5251426697
1.1969337463 -0.5152091980
1.1681976318 -0.5076522827
1.1496143341 -0.5044441223
1.1439170837 -0.5067405701
1.1505641937 -0.5142631531
1.1648588181 -0.5248947144
1.1784658432 -0.5348892212
1.1826848984 -0.5403366089
1.1730833054 -0.5392532349
1.1507940292 -0.5321617126
1.1197996140 -0.5208816528
1.0844039917 -0.5073909760
1.0486316681 -0.4935626984
1.0162878036 -0.4811782837
0.9907617569 -0.4718227386
0.9742755890 -0.4665260315
0.9667768478 -0.4652271271
0.9650783539 -0.4663639069
0.9631061554 -0.4669895172
0.9543151855 -0.4639377594
0.9351735115 -0.4554920197
0.9062047005 -0.4418907166
0.8700919151 -0.4244289398
0.8299164772 -0.4045944214
0.7888069153 -0.3838920593
0.7500014305 -0.3638896942
0.7166714668 -0.3461189270
0.6914076805 -0.3318214417
0.6754312515 -0.3215808868
0.6678633690 -0.3149776459
0.6653513908 -0.3104133606
0.6624686718 -0.3053073883
0.6537015438 -0.2970523834
0.6362051964 -0.2843074799
0.6105301380 -0.2673377991
0.5789489746 -0.2472190857
0.5438914299 -0.2250862122
0.5075421333 -0.2019271851
0.4718998671 -0.1786174774
0.4388072491 -0.1559448242
0.4097273350 -0.1345481873
0.3852332830 -0.1147804260
0.3645350933 -0.0965385437
0.3454892635 -0.0792846680
0.3254612684 -0.0623092651
0.3026974201 -0.0451049805
0.2769918442 -0.0275325775
0.2491828203 -0.0096759796
0.2203633785 0.0083465576
0.1915182769 0.0264835358
0.1635000259 0.0447921753
0.1370610744 0.0634155273
0.1127851158 0.0825424194
0.0909457579 0.1023330688
0.0714290291 0.1227359772
0.0537704192 0.1433238983
0.0372838005 0.1632823944
0.0213106498 0.1817092896
0.0054919422 0.1981391907
-0.0101998150 0.2127494812
-0.0256669894 0.2260990143
-0.0408606753 0.2388763428
-0.0558262728 0.2518386841
-0.0706941783 0.2658195496
-0.0856261253 0.2816429138
-0.1006980091 0.2998313904
-0.1157595813 0.3202152252
-0.1303257048 0.3416080475
-0.1435867697 0.3618373871
-0.1547022909 0.3785705566
-0.1632629633 0.3905525208
-0.1694482565 0.3980178833
-0.1737861633 0.4020690918
-0.1769064665 0.4040412903
-0.1794618368 0.4053192139
-0.1821180582 0.4073295593
-0.1855421066 0.4115180969
-0.1903103590 0.4191684723
-0.1966899633 0.4309101105
-0.2043910027 0.4461536407
-0.2124112844 0.4627532959
-0.2191201448 0.4771862030
-0.2228422165 0.4858531952
-0.2227022648 0.4869251251
-0.2188777924 0.4808559418
-0.2121338844 0.4693355560
-0.2033730745 0.4543037415
-0.1935007572 0.4376640320
-0.1833953857 0.4212417603
-0.1738576889 0.4066925049
-0.1654882431 0.3952369690
-0.1585042477 0.3872108459
-0.1525931358 0.3816528320
-0.1469383240 0.3763809204
-0.1405827999 0.3688735962
-0.1329843998 0.3576126099
-0.1242387295 0.3426513672
-0.1148152351 0.3250122070
-0.1052258015 0.3058776855
-0.0959098339 0.2863197327
-0.0872468948 0.2673225403
-0.0795645714 0.2497711182
-0.0731084347 0.2343711853
-0.0679700375 0.2213745117
-0.0640079975 0.2103118896
-0.0608448982 0.1999893188
-0.0580143929 0.1889533997
-0.0551931858 0.1762809753
-0.0523011684 0.1619071960
-0.0494072437 0.1462745667
-0.0466065407 0.1299476624
-0.0439786911 0.1134338379
-0.0415902138 0.0971679688
-0.0394990444 0.0815658569
-0.0377504826 0.0669937134
-0.0363528728 0.0537528992
-0.0352354050 0.0420417786
-0.0342111588 0.0318832397
-0.0329864025 0.0231246948
-0.0312707424 0.0155525208
-0.0289387703 0.0090332031
-0.0260756016 0.0035400391
-0.0228824615 -0.0008964539
-0.0195786953 -0.0042572021
-0.0163648129 -0.0065727234
-0.0134139061 -0.0079383850
-0.0108628273 -0.0085029602
-0.0087976456 -0.0084381104
-0.0072472095 -0.0079231262
-0.0061898232 -0.0071182251
-0.0055673122 -0.0061492920
-0.0052974224 -0.0051345825
-0.0052816868 -0.0041542053
-0.0054187775 -0.0032653809
-0.0056188107 -0.0025177002
-0.0058124065 -0.0019264221
-0.0059523582 -0.0014953613
-0.0060150623 -0.0012245178
-0.0060031414 -0.0010986328
-0.0059404373 -0.0010986328
-0.0058598518 -0.0012054443
-0.0057899952 -0.0013847351
-0.0057432652 -0.0016059875
-0.0057132244 -0.0018348694
-0.0056886673 -0.0020294189
-0.0056712627 -0.0021629333
-0.0056803226 -0.0022163391
-0.0057406425 -0.0021781921
-0.0058710575 -0.0020561218
-0.0060822964 -0.0018615723
-0.0063803196 -0.0015983582
-0.0067677498 -0.0012893677
-0.0072436333 -0.0009536743
-0.0077979565 -0.0006065369
-0.0084009171 -0.0002746582
-0.0089976788 0.0000381470
-0.0095119476 0.0003166199
-0.0098693371 0.0005531311
-0.0100340843 0.0007476807
-0.0100181103 0.0009002686
-0.0098559856 0.0010185242
-0.0095846653 0.0011024475
-0.0092394352 0.0011634827
-0.0088541508 0.0012054443
-0.0084617138 0.0012207031
-0.0080893040 0.0012130737
-0.0077466965 0.0011825562
-0.0074183941 0.0011138916
-0.0070614815 0.0009918213
-0.0066163540 0.0008049011
-0.0060374737 0.0005531311
-0.0053234100 0.0002365112
-0.0045137405 -0.0001296997
-0.0036652088 -0.0005149841
-0.0028316975 -0.0009078979
-0.0020565987 -0.0012893677
-0.0013713837 -0.0016441345
-0.0007953644 -0.0019721985
-0.0003387928 -0.0022697449
-0.0000061989 -0.0025291443
0.0002021790 -0.0027389526
0.0002903938 -0.0028839111
0.0002701283 -0.0029449463
0.0001654625 -0.0029296875
0.0000095367 -0.0028610229
-0.0001618862 -0.0027770996
-0.0003201962 -0.0027084351
-0.0004467964 -0.0026702881
-0.0005316734 -0.0026931763
-0.0005741119 -0.0027847290
-0.0005786419 -0.0029411316
-0.0005512238 -0.0031547546
-0.0004975796 -0.0034065247
-0.0004222393 -0.0036697388
-0.0003297329 -0.0039100647
-0.0002274513 -0.0041046143
-0.0001246929 -0.0042381287
-0.0000314713 -0.0043106079
0.0000424385 -0.0043296814
0.0000894070 -0.0042915344
0.0001029968 -0.0041999817
0.0000772476 -0.0040702820
0.0000107288 -0.0039176941
-0.0000953674 -0.0037612915
-0.0002374649 -0.0036048889
-0.0004105568 -0.0034408569
-0.0006086826 -0.0032653809
-0.0008225441 -0.0030632019
-0.0010392666 -0.0028305054
-0.0012431145 -0.0025825500
-0.0014197826 -0.0023460388
-0.0015575886 -0.0021476746
-0.0016510487 -0.0020027161
-0.0017004013 -0.0019226074
-0.0017096996 -0.0019226074
-0.0016849041 -0.0019989014
-0.0016295910 -0.0021400452
-0.0015428066 -0.0023307800
-0.0014202595 -0.0025444031
-0.0012593269 -0.0027618408
-0.0010662079 -0.0029487610
-0.0008575916 -0.0030937195
-0.0006527901 -0.0031967163
-0.0004694462 -0.0032463074
-0.0003232956 -0.0032463074
-0.0002255440 -0.0032081604
-0.0001831055 -0.0031394958
-0.0001986027 -0.0030555725
-0.0002696514 -0.0029754639
-0.0003910065 -0.0029029846
-0.0005548000 -0.0028266907
-0.0007493496 -0.0027389526
-0.0009601116 -0.0026321411
-0.0011696815 -0.0024909973
-0.0013594627 -0.0023345947
-0.0015144348 -0.0021820068
-0.0016241074 -0.0020408630
-0.0016832352 -0.0019302368
-0.0016927719 -0.0018577576
-0.0016589165 -0.0018196106
-0.0015916824 -0.0018157959
-0.0015010834 -0.0018424988
-0.0013923645 -0.0018806458
-0.0012676716 -0.0019187927
-0.0011310577 -0.0019340515
-0.0009937286 -0.0019111633
-0.0008759499 -0.0018577576
-0.0007994175 -0.0017738342
-0.0007824898 -0.0016555786
-0.0008361340 -0.0015144348


==> data/target_sample53.tex <==
-0.0000877380 0.0000000000
-0.0000305176 -0.0000114441
0.0000076294 -0.0000152588
0.0000305176 -0.0000190735
0.0000457764 -0.0000305176
0.0000495911 -0.0000419617
0.0000457764 -0.0000572205
0.0000419617 -0.0000724792
0.0000381470 -0.0000915527
0.0000381470 -0.0001144409
0.0000419617 -0.0001335144
0.0000457764 -0.0001525879
0.0000534058 -0.0001678467
0.0000610352 -0.0001792908
0.0000648499 -0.0001831055
0.0000762939 -0.0001792908
0.0000877380 -0.0001716614
0.0001068115 -0.0001602173
0.0001258850 -0.0001411438
0.0001373291 -0.0001182556
0.0001449585 -0.0000953674
0.0001373291 -0.0000724792
0.0001258850 -0.0000457764
0.0001068115 -0.0000190735
0.0000801086 0.0000076294
0.0000572205 0.0000267029
0.0000343323 0.0000381470
0.0000076294 0.0000534058
-0.0000267029 0.0000648499
-0.0000648499 0.0000762939
-0.0000991821 0.0000915527
-0.0001296997 0.0001068115
-0.0001602173 0.0001182556
-0.0001869202 0.0001258850
-0.0002021790 0.0001258850
-0.0002098083 0.0001182556
-0.0002098083 0.0001068115
-0.0002059937 0.0000953674
-0.0001983643 0.0000839233
-0.0001907349 0.0000724792
-0.0001869202 0.0000648499
-0.0001754761 0.0000572205
-0.0001640320 0.0000457764
-0.0001525879 0.0000381470
-0.0001411438 0.0000343323
-0.0001296997 0.0000228882
-0.0001068115 0.0000114441
-0.0000801086 0.0000038147
-0.0000534058 -0.0000038147
-0.0000228882 -0.0000152588
0.0000114441 -0.0000228882
0.0000419617 -0.0000267029
0.0000686646 -0.0000305176
0.0000915527 -0.0000305176
0.0001144409 -0.0000305176
0.0001373291 -0.0000228882
0.0001602173 -0.0000152588
0.0001831055 -0.0000114441
0.0001945496 -0.0000038147
0.0002059937 0.0000038147
0.0002098083 0.0000152588
0.0002059937 0.0000305176
0.0002021790 0.0000419617
0.0001907349 0.0000495911
0.0001754761 0.0000572205
0.0001564026 0.0000648499
0.0001258850 0.0000610352
0.0000877380 0.0000534058
0.0000419617 0.0000495911
-0.0000076294 0.0000419617
-0.0000610352 0.0000343323
-0.0001144409 0.0000305176
-0.0001640320 0.0000343323
-0.0002098083 0.0000419617
-0.0002479553 0.0000534058
-0.0002822876 0.0000648499
-0.0003128052 0.0000762939
-0.0003356934 0.0000953674
-0.0003547668 0.0001106262
-0.0003700256 0.0001258850
-0.0003738403 0.0001373291
-0.0003623962 0.0001335144
-0.0003318787 0.0001182556
-0.0002784729 0.0000839233
-0.0001945496 0.0000343323
-0.0000915527 -0.0000267029
0.0000190735 -0.0000991821
0.0001335144 -0.0001678467
0.0002365112 -0.0002212524
0.0003089905 -0.0002670288
0.0003509521 -0.0002937317
0.0003662109 -0.0003013611
0.0003547668 -0.0002975464
0.0003242493 -0.0002784729
0.0002784729 -0.0002593994
0.0002288818 -0.0002326965
0.0001754761 -0.0001983643
0.0001258850 -0.0001716614
0.0000877380 -0.0001449585
0.0000610352 -0.0001220703
0.0000495911 -0.0001068115
0.0000457764 -0.0000953674
0.0000534058 -0.0000877380
0.0000686646 -0.0000762939
0.0000801086 -0.0000648499
0.0000915527 -0.0000534058
0.0001068115 -0.0000457764
0.0001182556 -0.0000381470
0.0001220703 -0.0000267029
0.0001220703 -0.0000228882
0.0001220703 -0.0000228882
0.0001220703 -0.0000152588
0.0001258850 -0.0000038147
0.0001296997 0.0000038147
0.0001335144 0.0000228882
0.0001373291 0.0000495911
0.0001373291 0.0000724792
0.0001373291 0.0000991821
0.0001411438 0.0001296997
0.0001411438 0.0001525879
0.0001335144 0.0001602173
0.0001258850 0.0001564026
0.0001182556 0.0001449585
0.0001068115 0.0001182556
0.0000953674 0.0000877380
0.0000839233 0.0000610352
0.0000686646 0.0000343323
0.0000495911 0.0000228882
0.0000152588 0.0000267029
-0.0000305176 0.0000381470
-0.0000839233 0.0000534058
-0.0001335144 0.0000724792
-0.0001792908 0.0000991821
-0.0002174377 0.0001220703
-0.0002288818 0.0001411438
-0.0002174377 0.0001564026
-0.0001754761 0.0001640320
-0.0000991821 0.0001678467
-0.0000076294 0.0001602173
0.0000915527 0.0001411438
0.0001907349 0.0001106262
0.0002784729 0.0000762939
0.0003509521 0.0000457764
0.0004005432 0.0000152588
0.0004310608 -0.0000114441
0.0004348755 -0.0000267029
0.0004081726 -0.0000267029
0.0003623962 -0.0000114441
0.0003051758 0.0000114441
0.0002441406 0.0000343323
0.0001945496 0.0000648499
0.0001640320 0.0000991821
0.0001411438 0.0001258850
0.0001335144 0.0001525879
0.0001373291 0.0001754761
0.0001411438 0.0001983643
0.0001487732 0.0002174377
0.0001525879 0.0002326965
0.0001487732 0.0002441406
0.0001411438 0.0002517700
0.0001258850 0.0002555847
0.0000991821 0.0002517700
0.0000801086 0.0002517700
0.0000686646 0.0002441406
0.0000648499 0.0002326965
0.0000762939 0.0002212524
0.0000915527 0.0002059937
0.0001182556 0.0001869202
0.0001487732 0.0001716614
0.0001754761 0.0001564026
0.0001945496 0.0001449585
0.0002059937 0.0001449585
0.0002021790 0.0001487732
0.0001831055 0.0001564026
0.0001487732 0.0001716614
0.0001029968 0.0001869202
0.0000495911 0.0001983643
-0.0000076294 0.0002136230
-0.0000610352 0.0002250671
-0.0001106262 0.0002288818
-0.0001487732 0.0002326965
-0.0001792908 0.0002326965
-0.0001945496 0.0002250671
-0.0001945496 0.0002174377
-0.0001792908 0.0002059937
-0.0001525879 0.0001945496
-0.0001106262 0.0001831055
-0.0000610352 0.0001754761
-0.0000152588 0.0001716614
0.0000305176 0.0001640320
0.0000648499 0.0001564026
0.0000877380 0.0001525879
0.0001029968 0.0001449585
0.0001068115 0.0001411438
0.0001029968 0.0001411438
0.0000915527 0.0001411438
0.0000762939 0.0001449585
0.0000534058 0.0001487732
0.0000343323 0.0001564026
0.0000190735 0.0001602173
0.0000038147 0.0001640320
0.0000000000 0.0001602173
0.0000038147 0.0001487732
0.0000114441 0.0001449585
0.0000190735 0.0001335144
0.0000267029 0.0001220703
0.0000343323 0.0001144409
0.0000305176 0.0001068115
0.0000152588 0.0001068115
-0.0000114441 0.0001068115
-0.0000534058 0.0001106262
-0.0001106262 0.0001258850
-0.0001716614 0.0001564026
-0.0002326965 0.0001983643
-0.0002975464 0.0002555847
-0.0003623962 0.0003242493
-0.0004272461 0.0004005432
-0.0004882812 0.0004806519
-0.0005493164 0.0005569458
-0.0006065369 0.0006256104
-0.0006561279 0.0006790161
-0.0006942749 0.0007057190
-0.0007133484 0.0006942749
-0.0007057190 0.0006561279
-0.0006637573 0.0005874634
-0.0005950928 0.0004882812
-0.0005035400 0.0003700256
-0.0003967285 0.0002441406
-0.0002861023 0.0001182556
-0.0001869202 0.0000000000
-0.0000991821 -0.0001068115
-0.0000228882 -0.0001945496
0.0000267029 -0.0002517700
0.0000534058 -0.0002822876
0.0000572205 -0.0002784729
0.0000419617 -0.0002479553
0.0000152588 -0.0001983643
-0.0000114441 -0.0001411438
-0.0000419617 -0.0000915527
-0.0000648499 -0.0000457764
-0.0000839233 -0.0000152588
-0.0001029968 0.0000038147
-0.0001182556 0.0000152588
-0.0001411438 0.0000114441
-0.0001640320 0.0000000000
-0.0001907349 -0.0000190735
-0.0002250671 -0.0000343323
-0.0002555847 -0.0000457764
-0.0002746582 -0.0000610352
-0.0002937317 -0.0000648499
-0.0002975464 -0.0000610352
-0.0002861023 -0.0000572205
-0.0002632141 -0.0000381470
-0.0002288818 -0.0000114441
-0.0001945496 0.0000152588
-0.0001525879 0.0000457764
-0.0001144409 0.0000762939
-0.0000839233 0.0000991821
-0.0000572205 0.0001106262
-0.0000457764 0.0001144409
-0.0000495911 0.0001068115
-0.0000610352 0.0000877380
-0.0000801086 0.0000686646
-0.0001068115 0.0000419617
-0.0001373291 0.0000114441
-0.0001716614 -0.0000114441
-0.0002098083 -0.0000305176
-0.0002517700 -0.0000419617
-0.0002975464 -0.0000457764
-0.0003471375 -0.0000419617
-0.0004005432 -0.0000267029
-0.0004463196 -0.0000038147
-0.0004768372 0.0000267029
-0.0004959106 0.0000572205
-0.0004920959 0.0000801086
-0.0004653931 0.0000991821
-0.0004158020 0.0001106262
-0.0003471375 0.0001144409
-0.0002746582 0.0001106262
-0.0001983643 0.0000953674
-0.0001258850 0.0000724792
-0.0000724792 0.0000534058
-0.0000343323 0.0000381470
-0.0000190735 0.0000267029
-0.0000343323 0.0000267029
-0.0000762939 0.0000381470
-0.0001525879 0.0000572205
-0.0002517700 0.0000877380
-0.0003585815 0.0001296997
-0.0004768372 0.0001678467
-0.0005989075 0.0002059937
-0.0007133484 0.0002517700
-0.0008239746 0.0002899170
-0.0009231567 0.0003166199
-0.0010147095 0.0003356934
-0.0010871887 0.0003395081
-0.0011329651 0.0003204346
-0.0011520386 0.0002861023
-0.0011444092 0.0002403259
-0.0011215210 0.0001907349
-0.0010910034 0.0001525879
-0.0010566711 0.0001220703
-0.0010261536 0.0001029968
-0.0010032654 0.0000991821
-0.0009918213 0.0000991821
-0.0009918213 0.0001068115
-0.0010032654 0.0001220703
-0.0010223389 0.0001373291
-0.0010375977 0.0001487732
-0.0010490417 0.0001564026
-0.0010528564 0.0001640320
-0.0010604858 0.0001678467
-0.0010681152 0.0001754761
-0.0010833740 0.0001831055
-0.0011138916 0.0001907349
-0.0011558533 0.0002059937
-0.0012245178 0.0002212524
-0.0013122559 0.0002441406
-0.0014190674 0.0002746582
-0.0015411377 0.0003128052
-0.0016632080 0.0003547668
-0.0017738342 0.0004005432
-0.0018653870 0.0004501343
-0.0019416809 0.0004997253
-0.0020103455 0.0005531311
-0.0020751953 0.0006027222
-0.0021438599 0.0006523132
-0.0022277832 0.0006980896
-0.0023269653 0.0007400513
-0.0024414062 0.0007820129
-0.0025711060 0.0008201599
-0.0026969910 0.0008544922
-0.0027961731 0.0008850098
-0.0028457642 0.0009002686
-0.0028114319 0.0008926392
-0.0026779175 0.0008621216
-0.0024566650 0.0008125305
-0.0021705627 0.0007514954
-0.0018539429 0.0006752014
-0.0015296936 0.0005912781
-0.0012168884 0.0005111694
-0.0009346008 0.0004272461
-0.0006904602 0.0003471375
-0.0004920959 0.0002822876
-0.0003356934 0.0002212524
-0.0002326965 0.0001716614
-0.0001716614 0.0001373291
-0.0001373291 0.0001068115
-0.0001335144 0.0000877380
-0.0001296997 0.0000686646
-0.0001144409 0.0000495911
-0.0000991821 0.0000343323
-0.0000724792 0.0000076294
-0.0000381470 -0.0000114441
-0.0000114441 -0.0000305176
0.0000076294 -0.0000495911
0.0000114441 -0.0000610352
-0.0000076294 -0.0000648499
-0.0000495911 -0.0000610352
-0.0001144409 -0.0000495911
-0.0002059937 -0.0000228882
-0.0003128052 0.0000114441
-0.0004158020 0.0000534058
-0.0005149841 0.0000991821
-0.0006027222 0.0001449585
-0.0006713867 0.0001792908
-0.0007171631 0.0002059937
-0.0007362366 0.0002212524
-0.0007324219 0.0002174377
-0.0006942749 0.0001983643
-0.0006065369 0.0001564026
-0.0004768372 0.0000915527
-0.0003204346 0.0000152588
-0.0001525879 -0.0000686646
0.0000038147 -0.0001525879
0.0001220703 -0.0002250671
0.0001907349 -0.0002822876
0.0002059937 -0.0003166199
0.0001716614 -0.0003356934
0.0000991821 -0.0003395081
0.0000000000 -0.0003242493
-0.0001106262 -0.0003013611
-0.0002174377 -0.0002746582
-0.0003013611 -0.0002403259
-0.0003547668 -0.0002021790
-0.0003852844 -0.0001602173
-0.0003929138 -0.0001182556
-0.0003890991 -0.0000839233
-0.0003967285 -0.0000610352
-0.0004081726 -0.0000419617
-0.0004348755 -0.0000305176
-0.0004730225 -0.0000305176
-0.0005111694 -0.0000343323
-0.0005455017 -0.0000381470
-0.0005607605 -0.0000419617
-0.0005493164 -0.0000495911
-0.0004959106 -0.0000495911
-0.0003929138 -0.0000419617
-0.0002517700 -0.0000381470
-0.0000915527 -0.0000381470
0.0000839233 -0.0000495911
0.0002555847 -0.0000648499
0.0004158020 -0.0000724792
0.0005569458 -0.0000839233
0.0006752014 -0.0000953674
0.0007667542 -0.0000991821
0.0008316040 -0.0001029968
0.0008697510 -0.0001068115
0.0008697510 -0.0001068115
0.0008354187 -0.0001029968
0.0007705688 -0.0000991821
0.0006866455 -0.0000915527
0.0005874634 -0.0000762939
0.0004844666 -0.0000534058
0.0003814697 -0.0000228882
0.0002784729 0.0000076294
0.0001869202 0.0000457764
0.0001106262 0.0000839233
0.0000495911 0.0001106262
0.0000076294 0.0001335144
-0.0000190735 0.0001449585
-0.0000267029 0.0001411438
-0.0000114441 0.0001258850
0.0000152588 0.0001029968
0.0000534058 0.0000686646
0.0000953674 0.0000343323
0.0001335144 0.0000076294
0.0001716614 -0.0000190735
0.0002021790 -0.0000305176
0.0002212524 -0.0000305176
0.0002326965 -0.0000267029
0.0002326965 -0.0000152588
0.0002212524 0.0000076294
0.0002021790 0.0000267029
0.0001754761 0.0000419617
0.0001449585 0.0000534058
0.0001182556 0.0000572205
0.0001068115 0.0000572205
0.0001029968 0.0000534058
0.0001029968 0.0000572205
0.0001106262 0.0000648499
0.0001220703 0.0000801086
0.0001373291 0.0001106262
0.0001564026 0.0001411438
0.0001754761 0.0001716614
0.0001907349 0.0001983643
0.0001983643 0.0002098083
0.0001945496 0.0002098083
0.0001831055 0.0002021790
0.0001602173 0.0001907349
0.0001258850 0.0001792908
0.0000839233 0.0001754761
0.0000343323 0.0001754761
-0.0000190735 0.0001792908
-0.0000724792 0.0001907349
-0.0001182556 0.0002021790
-0.0001525879 0.0002136230
-0.0001678467 0.0002250671
-0.0001602173 0.0002212524
-0.0001373291 0.0002059937
-0.0000915527 0.0001869202
-0.0000305176 0.0001602173
0.0000228882 0.0001335144
0.0000724792 0.0001068115
0.0001106262 0.0000839233
0.0001335144 0.0000648499
0.0001487732 0.0000495911
0.0001564026 0.0000419617
0.0001564026 0.0000419617
0.0001525879 0.0000457764
0.0001487732 0.0000534058
0.0001411438 0.0000648499
0.0001335144 0.0000801086
0.0001182556 0.0000953674
0.0001029968 0.0001106262
0.0000839233 0.0001220703
0.0000534058 0.0001220703
0.0000152588 0.0001258850
-0.0000305176 0.0001258850
-0.0000877380 0.0001220703
-0.0001487732 0.0001182556
-0.0002059937 0.0001144409
-0.0002632141 0.0001106262
-0.0003051758 0.0001029968
-0.0003204346 0.0000991821
-0.0003166199 0.0000953674
-0.0002937317 0.0000877380
-0.0002555847 0.0000801086
-0.0002174377 0.0000762939
-0.0001716614 0.0000762939
-0.0001258850 0.0000762939
-0.0000915527 0.0000762939
-0.0000610352 0.0000839233
-0.0000305176 0.0000915527
-0.0000038147 0.0000953674
0.0000190735 0.0000991821
0.0000419617 0.0001029968
0.0000610352 0.0000991821
0.0000762939 0.0000877380
0.0000915527 0.0000724792
0.0000991821 0.0000534058
0.0000953674 0.0000343323
0.0000839233 0.0000114441
0.0000724792 -0.0000038147
0.0000534058 -0.0000152588
0.0000267029 -0.0000267029
0.0000000000 -0.0000305176
-0.0000305176 -0.0000267029
-0.0000610352 -0.0000152588
-0.0000877380 0.0000076294
-0.0001068115 0.0000343323
-0.0001220703 0.0000648499
-0.0001335144 0.0000953674
-0.0001411438 0.0001182556
-0.0001487732 0.0001411438
-0.0001640320 0.0001564026
-0.0001792908 0.0001640320
-0.0001907349 0.0001640320
-0.0002021790 0.0001525879
-0.0002021790 0.0001335144
-0.0001792908 0.0001029968
-0.0001335144 0.0000534058
-0.0000610352 -0.0000076294
0.0000343323 -0.0000724792
0.0001449585 -0.0001411438
0.0002593994 -0.0002021790
0.0003662109 -0.0002479553
0.0004577637 -0.0002861023
0.0005187988 -0.0003128052
0.0005569458 -0.0003280640
0.0005760193 -0.0003356934
0.0005683899 -0.0003318787
0.0005416870 -0.0003280640
0.0005035400 -0.0003204346
0.0004463196 -0.0003051758
0.0003814697 -0.0002784729
0.0003204346 -0.0002479553
0.0002670288 -0.0002174377
0.0002250671 -0.0001792908
0.0001945496 -0.0001411438
0.0001716614 -0.0000991821
0.0001602173 -0.0000572205
0.0001525879 -0.0000190735
0.0001525879 0.0000152588
0.0001564026 0.0000419617
0.0001525879 0.0000686646
0.0001487732 0.0000915527
0.0001373291 0.0000991821
0.0001296997 0.0001068115
0.0001258850 0.0001106262
0.0001182556 0.0001068115
0.0001144409 0.0000991821
0.0001144409 0.0000877380
0.0001182556 0.0000724792
0.0001144409 0.0000572205
0.0001068115 0.0000457764
0.0000991821 0.0000267029
0.0000877380 0.0000152588
0.0000724792 0.0000114441
0.0000610352 0.0000038147
0.0000534058 -0.0000038147
0.0000419617 -0.0000076294
0.0000343323 -0.0000152588
0.0000267029 -0.0000228882
0.0000152588 -0.0000305176
0.0000000000 -0.0000381470
-0.0000267029 -0.0000457764
-0.0000610352 -0.0000534058
-0.0000953674 -0.0000572205
-0.0001296997 -0.0000648499
-0.0001564026 -0.0000648499
-0.0001792908 -0.0000610352
-0.0001907349 -0.0000648499
-0.0001831055 -0.0000686646
-0.0001602173 -0.0000801086
-0.0001296997 -0.0001029968
-0.0000839233 -0.0001296997
-0.0000267029 -0.0001640320
0.0000267029 -0.0001983643
0.0000801086 -0.0002288818
0.0001335144 -0.0002517700
0.0001754761 -0.0002708435
0.0002059937 -0.0002746582
0.0002212524 -0.0002593994
0.0002136230 -0.0002365112
0.0001907349 -0.0002021790
0.0001602173 -0.0001640320
0.0001220703 -0.0001258850
0.0000877380 -0.0000915527
0.0000610352 -0.0000686646
0.0000381470 -0.0000572205
0.0000267029 -0.0000572205
0.0000305176 -0.0000648499
0.0000457764 -0.0000801086
0.0000648499 -0.0000991821
0.0000839233 -0.0001182556
0.0001068115 -0.0001335144
0.0001335144 -0.0001373291
0.0001564026 -0.0001411438
0.0001716614 -0.0001373291
0.0001792908 -0.0001220703
0.0001831055 -0.0001106262
0.0001869202 -0.0001029968
0.0001869202 -0.0000915527
0.0001907349 -0.0000801086
0.0001983643 -0.0000724792
0.0002098083 -0.0000648499
0.0002326965 -0.0000534058
0.0002593994 -0.0000381470
0.0002861023 -0.0000267029
0.0003128052 -0.0000152588
0.0003318787 -0.0000038147
0.0003318787 0.0000000000
0.0003128052 0.0000038147
0.0002822876 0.0000076294
0.0002403259 0.0000038147
0.0001831055 -0.0000038147
0.0001296997 -0.0000114441
0.0000801086 -0.0000190735
0.0000343323 -0.0000267029
0.0000038147 -0.0000381470
-0.0000114441 -0.0000457764
-0.0000152588 -0.0000534058
-0.0000076294 -0.0000648499
0.0000114441 -0.0000686646
0.0000381470 -0.0000762939
0.0000648499 -0.0000801086
0.0000915527 -0.0000839233
0.0001220703 -0.0000877380
0.0001449585 -0.0000801086
0.0001678467 -0.0000801086
0.0001945496 -0.0000801086
0.0002098083 -0.0000762939
0.0002212524 -0.0000801086
0.0002288818 -0.0000839233
0.0002250671 -0.0000877380
0.0002250671 -0.0000953674
0.0002288818 -0.0001068115
0.0002403259 -0.0001258850
0.0002670288 -0.0001525879
0.0003089905 -0.0001869202
0.0003662109 -0.0002326965
0.0004348755 -0.0002899170
0.0005149841 -0.0003471375
0.0005950928 -0.0004005432
0.0006637573 -0.0004463196
0.0007133484 -0.0004882812
0.0007438660 -0.0005149841
0.0007553101 -0.0005226135
0.0007476807 -0.0005187988
0.0007324219 -0.0004997253
0.0007057190 -0.0004653931
0.0006637573 -0.0004196167
0.0006217957 -0.0003738403
0.0005760193 -0.0003242493
0.0005226135 -0.0002708435
0.0004692078 -0.0002288818
0.0004158020 -0.0001945496
0.0003585815 -0.0001640320
0.0002937317 -0.0001487732
0.0002288818 -0.0001335144
0.0001678467 -0.0001106262
0.0001029968 -0.0000839233
0.0000419617 -0.0000419617
-0.0000152588 0.0000190735
-0.0000762939 0.0000839233
-0.0001373291 0.0001525879
-0.0001945496 0.0002250671
-0.0002479553 0.0002899170
-0.0002861023 0.0003395081
-0.0003013611 0.0003662109
-0.0002899170 0.0003662109
-0.0002441406 0.0003318787
-0.0001716614 0.0002708435
-0.0000724792 0.0001983643
0.0000457764 0.0001144409
0.0001754761 0.0000305176
0.0002975464 -0.0000419617
0.0004081726 -0.0001106262
0.0004997253 -0.0001640320
0.0005569458 -0.0002021790
0.0005950928 -0.0002288818
0.0006027222 -0.0002326965
0.0005683899 -0.0002212524
0.0005111694 -0.0001945496
0.0004425049 -0.0001640320
0.0003623962 -0.0001411438
0.0002937317 -0.0001258850
0.0002479553 -0.0001182556
0.0002174377 -0.0001144409
0.0002098083 -0.0001182556
0.0002174377 -0.0001220703
0.0002326965 -0.0001220703
0.0002555847 -0.0001182556
0.0002822876 -0.0001144409
0.0002975464 -0.0001144409
0.0002975464 -0.0001144409
0.0002937317 -0.0001220703
0.0002784729 -0.0001335144
0.0002670288 -0.0001373291
0.0002670288 -0.0001411438
0.0002784729 -0.0001449585
0.0003051758 -0.0001449585
0.0003395081 -0.0001411438
0.0003852844 -0.0001373291
0.0004348755 -0.0001296997
0.0004768372 -0.0001220703
0.0005111694 -0.0001144409
0.0005226135 -0.0001068115
0.0005111694 -0.0001068115
0.0004882812 -0.0000991821
0.0004577637 -0.0000839233
0.0004234314 -0.0000724792
0.0003967285 -0.0000610352
0.0003776550 -0.0000457764
0.0003662109 -0.0000381470
0.0003700256 -0.0000305176
0.0003814697 -0.0000228882
0.0003929138 -0.0000190735
0.0004005432 -0.0000152588
0.0004005432 -0.0000114441
0.0003929138 -0.0000038147
0.0003738403 0.0000038147
0.0003433228 0.0000076294
0.0003280640 0.0000076294
0.0003280640 -0.0000038147
0.0003471375 -0.0000228882
0.0003890991 -0.0000457764
0.0004501343 -0.0000801086
0.0005302429 -0.0001182556
0.0006141663 -0.0001602173
0.0007057190 -0.0001983643
0.0007896423 -0.0002288818
0.0008544922 -0.0002479553
0.0008964539 -0.0002517700
0.0009002686 -0.0002403259
0.0008773804 -0.0002136230
0.0008392334 -0.0001792908
0.0007858276 -0.0001373291
0.0007286072 -0.0000915527
0.0006713867 -0.0000572205
0.0006179810 -0.0000267029
0.0005760193 -0.0000038147
0.0005455017 0.0000076294
0.0005264282 0.0000228882
0.0005149841 0.0000305176
0.0005149841 0.0000381470
0.0005226135 0.0000457764
0.0005187988 0.0000495911
0.0005111694 0.0000610352
0.0004959106 0.0000762939
0.0004692078 0.0000877380
0.0004425049 0.0001029968
0.0004081726 0.0001258850
0.0003776550 0.0001449585
0.0003585815 0.0001602173
0.0003471375 0.0001678467
0.0003433228 0.0001678467
0.0003471375 0.0001602173
0.0003585815 0.0001411438
0.0003700256 0.0001144409
0.0003814697 0.0000839233
0.0003929138 0.0000534058
0.0003929138 0.0000267029
0.0003890991 0.0000076294
0.0003776550 -0.0000038147
0.0003585815 -0.0000114441
0.0003395081 -0.0000114441
0.0003242493 -0.0000114441
0.0003166199 -0.0000114441
0.0003128052 -0.0000038147
0.0003128052 -0.0000038147
0.0003242493 -0.0000076294
0.0003471375 -0.0000114441
0.0003776550 -0.0000228882
0.0004119873 -0.0000419617
0.0004463196 -0.0000648499
0.0004882812 -0.0000877380
0.0005226135 -0.0001182556
0.0005569458 -0.0001525879
0.0005989075 -0.0001831055
0.0006408691 -0.0002136230
0.0006828308 -0.0002403259
0.0007247925 -0.0002632141
0.0007629395 -0.0002784729
0.0007896423 -0.0002822876
0.0008087158 -0.0002861023
0.0008125305 -0.0002861023
0.0008010864 -0.0002746582
0.0007743835 -0.0002670288
0.0007400513 -0.0002555847
0.0006980896 -0.0002403259
0.0006484985 -0.0002326965
0.0006103516 -0.0002174377
0.0005760193 -0.0002059937
0.0005455017 -0.0001945496
0.0005226135 -0.0001716614
0.0004997253 -0.0001525879
0.0004806519 -0.0001335144
0.0004653931 -0.0001106262
0.0004539490 -0.0000953674
0.0004348755 -0.0000839233
0.0004119873 -0.0000762939
0.0003929138 -0.0000801086
0.0003585815 -0.0000877380
0.0003166199 -0.0000915527
0.0002746582 -0.0000877380
0.0002174377 -0.0000801086
0.0001525879 -0.0000610352
0.0000877380 -0.0000305176
0.0000190735 0.0000152588
-0.0000457764 0.0000724792
-0.0000915527 0.0001335144
-0.0001258850 0.0001945496
-0.0001525879 0.0002479553
-0.0001716614 0.0002937317
-0.0001869202 0.0003166199
-0.0001945496 0.0003204346
-0.0001945496 0.0003128052
-0.0001831055 0.0002784729
-0.0001487732 0.0002250671
-0.0000877380 0.0001525879
-0.0000114441 0.0000648499
0.0000686646 -0.0000267029
0.0001449585 -0.0001182556
0.0002059937 -0.0001945496
0.0002441406 -0.0002479553
0.0002593994 -0.0002784729
0.0002479553 -0.0002899170
0.0002212524 -0.0002822876
0.0001945496 -0.0002632141
0.0001602173 -0.0002403259
0.0001296997 -0.0002212524
0.0001106262 -0.0002059937
0.0000991821 -0.0001983643
0.0001029968 -0.0002021790
0.0001029968 -0.0002059937
0.0000991821 -0.0002098083
0.0000877380 -0.0002098083
0.0000648499 -0.0001983643
0.0000381470 -0.0001831055
0.0000038147 -0.0001602173
-0.0000381470 -0.0001296997
-0.0000801086 -0.0001029968
-0.0001144409 -0.0000762939
-0.0001449585 -0.0000495911
-0.0001678467 -0.0000343323
-0.0001754761 -0.0000305176
-0.0001754761 -0.0000343323
-0.0001640320 -0.0000457764
-0.0001487732 -0.0000572205
-0.0001335144 -0.0000648499
-0.0001144409 -0.0000724792
-0.0001029968 -0.0000762939
-0.0000953674 -0.0000762939
-0.0000915527 -0.0000762939
-0.0000915527 -0.0000724792
-0.0000953674 -0.0000686646
-0.0001068115 -0.0000724792
-0.0001220703 -0.0000801086
-0.0001335144 -0.0000877380
-0.0001449585 -0.0000915527
-0.0001564026 -0.0000953674
-0.0001678467 -0.0000915527
-0.0001754761 -0.0000724792
-0.0001831055 -0.0000457764
-0.0001945496 -0.0000114441
-0.0002021790 0.0000305176
-0.0002059937 0.0000724792
-0.0002021790 0.0001106262
-0.0001869202 0.0001373291
-0.0001602173 0.0001449585
-0.0001182556 0.0001335144
-0.0000610352 0.0001029968
0.0000000000 0.0000648499
0.0000686646 0.0000190735
0.0001335144 -0.0000267029
0.0001831055 -0.0000648499
0.0002212524 -0.0000953674
0.0002403259 -0.0001106262
0.0002403259 -0.0001106262
0.0002288818 -0.0001029968
0.0002059937 -0.0000877380
0.0001716614 -0.0000534058
0.0001296997 -0.0000152588
0.0000877380 0.0000190735
0.0000534058 0.0000534058
0.0000267029 0.0000724792
0.0000114441 0.0000801086
0.0000114441 0.0000686646
0.0000228882 0.0000343323
0.0000495911 -0.0000152588
0.0000839233 -0.0000762939
0.0001258850 -0.0001411438
0.0001792908 -0.0002059937
0.0002365112 -0.0002670288
0.0002975464 -0.0003128052
0.0003662109 -0.0003471375
0.0004348755 -0.0003738403
0.0005035400 -0.0003890991
0.0005683899 -0.0004081726
0.0006256104 -0.0004386902
0.0006828308 -0.0004844666
0.0007362366 -0.0005416870
0.0007896423 -0.0006217957
0.0008468628 -0.0007171631
0.0009117126 -0.0008201599
0.0009803772 -0.0009307861
0.0010490417 -0.0010375977
0.0011177063 -0.0011329651
0.0011711121 -0.0012092590
0.0012054443 -0.0012664795
0.0012207031 -0.0012969971
0.0012130737 -0.0013008118
0.0011863708 -0.0012817383
0.0011329651 -0.0012397766
0.0010643005 -0.0011825562
0.0009803772 -0.0011177063
0.0008811951 -0.0010452271
0.0007743835 -0.0009574890
0.0006446838 -0.0008583069
0.0004997253 -0.0007476807
0.0003395081 -0.0006217957
0.0001754761 -0.0004806519
0.0000267029 -0.0003318787
-0.0001029968 -0.0001831055
-0.0002136230 -0.0000343323
-0.0003051758 0.0001068115
-0.0003776550 0.0002517700
-0.0004386902 0.0003929138
-0.0004882812 0.0005264282
-0.0005340576 0.0006523132
-0.0005722046 0.0007629395
-0.0005950928 0.0008506775
-0.0006027222 0.0009155273
-0.0005874634 0.0009498596
-0.0005493164 0.0009536743
-0.0004844666 0.0009384155
-0.0003890991 0.0008926392
-0.0002784729 0.0008277893
-0.0001564026 0.0007514954
-0.0000190735 0.0006561279
0.0001182556 0.0005569458
0.0002479553 0.0004615784
0.0003700256 0.0003623962
0.0004730225 0.0002708435
0.0005493164 0.0001907349
0.0005950928 0.0001144409
0.0006027222 0.0000534058
0.0005760193 0.0000114441
0.0005187988 -0.0000152588
0.0004348755 -0.0000267029
0.0003356934 -0.0000190735
0.0002212524 0.0000038147
0.0000991821 0.0000343323
-0.0000228882 0.0000724792
-0.0001373291 0.0001182556
-0.0002403259 0.0001640320
-0.0003356934 0.0002059937
-0.0004119873 0.0002517700
-0.0004730225 0.0002899170
-0.0005226135 0.0003166199
-0.0005455017 0.0003356934
-0.0005378723 0.0003395081
-0.0004997253 0.0003242493
-0.0004234314 0.0002899170
-0.0003128052 0.0002365112
-0.0001792908 0.0001678467
-0.0000381470 0.0000915527
0.0001068115 0.0000114441
0.0002403259 -0.0000724792
0.0003433228 -0.0001525879
0.0004196167 -0.0002212524
0.0004577637 -0.0002670288
0.0004615784 -0.0002937317
0.0004310608 -0.0003013611
0.0003776550 -0.0002899170
0.0003128052 -0.0002632141
0.0002403259 -0.0002250671
0.0001640320 -0.0001792908
0.0000915527 -0.0001220703
0.0000228882 -0.0000648499
-0.0000457764 -0.0000114441
-0.0000991821 0.0000419617
-0.0001449585 0.0000953674
-0.0001907349 0.0001373291
-0.0002288818 0.0001716614
-0.0002555847 0.0002059937
-0.0002746582 0.0002326965
-0.0002861023 0.0002555847
-0.0002861023 0.0002784729
-0.0002708435 0.0002975464
-0.0002403259 0.0003166199
-0.0002021790 0.0003318787
-0.0001525879 0.0003433228
-0.0000991821 0.0003433228
-0.0000457764 0.0003280640
0.0000076294 0.0003013611
0.0000495911 0.0002632141
0.0000839233 0.0002212524
0.0001068115 0.0001792908
0.0001068115 0.0001411438
0.0000953674 0.0001068115
0.0000762939 0.0000724792
0.0000419617 0.0000419617
0.0000000000 0.0000190735
-0.0000381470 0.0000000000
-0.0000762939 -0.0000076294
-0.0001182556 0.0000000000
-0.0001487732 0.0000190735
-0.0001678467 0.0000495911
-0.0001831055 0.0000915527
-0.0001983643 0.0001373291
-0.0002059937 0.0001831055
-0.0002098083 0.0002250671
-0.0002136230 0.0002632141
-0.0002059937 0.0002937317
-0.0001907349 0.0003089905
-0.0001602173 0.0003166199
-0.0001144409 0.0003166199
-0.0000610352 0.0003013611
0.0000114441 0.0002593994
0.0000915527 0.0002021790
0.0001640320 0.0001411438


==> data/target_sample62.tex <==
-0.0034446716 0.0002403259
-0.0033721924 0.0001258850
-0.0033187866 0.0000152588
-0.0032730103 -0.0000915527
-0.0032272339 -0.0002059937
-0.0031661987 -0.0003166199
-0.0030822754 -0.0004158020
-0.0029830933 -0.0005073547
-0.0028686523 -0.0005874634
-0.0027465820 -0.0006523132
-0.0026245117 -0.0006904602
-0.0025100708 -0.0007057190
-0.0024070740 -0.0007095337
-0.0023231506 -0.0007133484
-0.0022659302 -0.0007133484
-0.0022239685 -0.0007057190
-0.0021896362 -0.0007057190
-0.0021476746 -0.0007095337
-0.0020637512 -0.0007019043
-0.0019264221 -0.0006980896
-0.0017318726 -0.0007057190
-0.0014648438 -0.0007324219
-0.0011177063 -0.0007934570
-0.0006752014 -0.0009002686
-0.0001144409 -0.0010719299
0.0005874634 -0.0013351440
0.0014686584 -0.0017051697
0.0025672913 -0.0021934509
0.0039024353 -0.0028266907
0.0054931641 -0.0036125183
0.0073738098 -0.0045585632
0.0095787048 -0.0056953430
0.0121650696 -0.0070610046
0.0152015686 -0.0086975098
0.0187416077 -0.0106468201
0.0228385925 -0.0129318237
0.0275230408 -0.0155754089
0.0328102112 -0.0185890198
0.0386886597 -0.0219650269
0.0450935364 -0.0256652832
0.0518379211 -0.0295829773
0.0585899353 -0.0335235596
0.0649299622 -0.0372467041
0.0704879761 -0.0405387878
0.0751037598 -0.0432968140
0.0787925720 -0.0455436707
0.0816688538 -0.0473747253
0.0839157104 -0.0489273071
0.0857658386 -0.0503768921
0.0874977112 -0.0519332886
0.0894126892 -0.0538215637
0.0917968750 -0.0562362671
0.0947532654 -0.0592651367
0.0980949402 -0.0628204346
0.1013450623 -0.0666198730
0.1039581299 -0.0703430176
0.1056938171 -0.0738296509
0.1066932678 -0.0771522522
0.1072921753 -0.0805130005
0.1078605652 -0.0841407776
0.1087341309 -0.0882568359
0.1101913452 -0.0930519104
0.1124992371 -0.0987205505
0.1158409119 -0.1054191589
0.1201934814 -0.1131324768
0.1251945496 -0.1215400696
0.1301002502 -0.1299819946
0.1340560913 -0.1376838684
0.1365203857 -0.1441993713
0.1374053955 -0.1495513916
0.1368865967 -0.1540260315
0.1352233887 -0.1580009460
0.1327095032 -0.1618995667
0.1296882629 -0.1661949158
0.1265563965 -0.1714019775
0.1237106323 -0.1780395508
0.1214752197 -0.1864852905
0.1199417114 -0.1967468262
0.1188011169 -0.2082290649
0.1173934937 -0.2196998596
0.1149978638 -0.2298164368
0.1112670898 -0.2378578186
0.1063575745 -0.2439231873
0.1006698608 -0.2485580444
0.0945968628 -0.2523880005
0.0884895325 -0.2560920715
0.0826644897 -0.2604007721
0.0774002075 -0.2660484314
0.0728912354 -0.2736568451
0.0691909790 -0.2834510803
0.0661506653 -0.2948875427
0.0633811951 -0.3065338135
0.0603981018 -0.3165531158
0.0568542480 -0.3236598969
0.0526428223 -0.3277034760
0.0478248596 -0.3293590546
0.0425109863 -0.3295383453
0.0367774963 -0.3291606903
0.0307159424 -0.3292198181
0.0244178772 -0.3307991028
0.0179557800 -0.3349418640
0.0113945007 -0.3423538208
0.0047569275 -0.3529834747
-0.0019607544 -0.3656406403
-0.0087814331 -0.3780174255
-0.0157165527 -0.3876152039
-0.0227584839 -0.3931083679
-0.0299034119 -0.3947734833
-0.0371932983 -0.3937625885
-0.0446968079 -0.3913745880
-0.0525131226 -0.3888874054
-0.0607757568 -0.3875656128
-0.0696029663 -0.3886165619
-0.0790939331 -0.3929843903
-0.0892105103 -0.4008865356
-0.0996704102 -0.4113349915
-0.1099395752 -0.4220905304
-0.1193695068 -0.4305019379
-0.1275329590 -0.4348888397
-0.1343727112 -0.4351902008
-0.1400871277 -0.4324111938
-0.1450004578 -0.4278411865
-0.1494789124 -0.4227752686
-0.1539459229 -0.4185047150
-0.1588668823 -0.4163475037
-0.1647109985 -0.4175567627
-0.1718063354 -0.4229412079
-0.1800804138 -0.4323215485
-0.1888885498 -0.4440841675
-0.1970214844 -0.4552516937
-0.2031631470 -0.4626235962
-0.2066192627 -0.4644622803
-0.2075653076 -0.4610424042
-0.2066459656 -0.4537582397
-0.2045974731 -0.4441947937
-0.2021522522 -0.4339103699
-0.2000427246 -0.4245109558
-0.1990089417 -0.4176292419
-0.1996879578 -0.4146900177
-0.2023849487 -0.4164428711
-0.2068405151 -0.4224452972
-0.2120704651 -0.4307727814
-0.2164535522 -0.4382057190
-0.2183189392 -0.4414253235
-0.2168045044 -0.4387378693
-0.2121009827 -0.4305572510
-0.2049446106 -0.4183864594
-0.1961822510 -0.4038639069
-0.1866264343 -0.3885364532
-0.1770668030 -0.3738727570
-0.1682281494 -0.3612213135
-0.1606559753 -0.3515434265
-0.1545295715 -0.3449974060
-0.1494789124 -0.3406009674
-0.1446647644 -0.3362751007
-0.1391525269 -0.3297176361
-0.1324348450 -0.3196449280
-0.1246299744 -0.3061771393
-0.1161804199 -0.2901935577
-0.1075401306 -0.2726726532
-0.0991058350 -0.2545375824
-0.0912361145 -0.2366638184
-0.0842170715 -0.2198581696
-0.0782203674 -0.2047557831
-0.0732498169 -0.1915931702
-0.0690765381 -0.1800136566
-0.0652313232 -0.1690864563
-0.0611915588 -0.1577434540
-0.0566635132 -0.1453952789
-0.0516090393 -0.1321334839
-0.0461502075 -0.1183986664
-0.0404624939 -0.1046352386
-0.0346946716 -0.0912322998
-0.0289726257 -0.0785274506
-0.0234336853 -0.0668048859
-0.0181961060 -0.0562953949
-0.0133323669 -0.0471267700
-0.0088882446 -0.0392799377
-0.0048484802 -0.0325794220
-0.0011901855 -0.0267257690
0.0020980835 -0.0214328766
0.0049858093 -0.0165634155
0.0073966980 -0.0121402740
0.0092735291 -0.0082359314
0.0106010437 -0.0048866272
0.0114021301 -0.0020961761
0.0117073059 0.0001487732
0.0115814209 0.0018844604
0.0111083984 0.0031700134
0.0103797913 0.0040798187
0.0094604492 0.0046825409
0.0083923340 0.0050334930
0.0071907043 0.0051708221
0.0058746338 0.0051212311
0.0045051575 0.0049228668
0.0031776428 0.0046176910
0.0019912720 0.0042457581
0.0010147095 0.0038414001
0.0002899170 0.0034313202
-0.0001792908 0.0030345917
-0.0004119873 0.0026645660
-0.0004425049 0.0023384094
-0.0003242493 0.0020618439
-0.0001106262 0.0018348694
0.0001564026 0.0016517639
0.0004310608 0.0015029907
0.0006752014 0.0013847351
0.0008697510 0.0012912750
0.0010032654 0.0012302399
0.0010833740 0.0011978149
0.0011291504 0.0011882782
0.0011634827 0.0012016296
0.0012016296 0.0012340546
0.0012474060 0.0012760162
0.0013122559 0.0013198853
0.0013961792 0.0013599396
0.0014877319 0.0013790131
0.0015716553 0.0013637543
0.0016403198 0.0013160706
0.0016899109 0.0012454987
0.0017166138 0.0011653900
0.0017280579 0.0010967255
0.0017280579 0.0010490417
0.0017204285 0.0010299683
0.0017204285 0.0010471344
0.0017318726 0.0011005402
0.0017585754 0.0011863708
0.0018119812 0.0013027191
0.0018844604 0.0014419556
0.0019645691 0.0015907288
0.0020484924 0.0017375946
0.0021209717 0.0018730164
0.0021743774 0.0019950867
0.0022125244 0.0021076202
0.0022239685 0.0022182465
0.0022087097 0.0023269653
0.0021705627 0.0024375916
0.0021018982 0.0025577545
0.0020179749 0.0026874542
0.0019187927 0.0028228760
0.0018005371 0.0029582977
0.0016670227 0.0030746460
0.0015106201 0.0031509399
0.0013389587 0.0031814575
0.0011672974 0.0031700134
0.0010223389 0.0031242371
0.0009155273 0.0030612946
0.0008544922 0.0029983521
0.0008506775 0.0029487610
0.0008964539 0.0029239655
0.0009918213 0.0029315948
0.0011291504 0.0029830933
0.0012855530 0.0030765533
0.0014495850 0.0031948090
0.0016059875 0.0033168793
0.0017242432 0.0034179688
0.0018005371 0.0034790039
0.0018386841 0.0034885406
0.0018424988 0.0034484863
0.0018348694 0.0033645630
0.0018196106 0.0032444000
0.0018005371 0.0031013489
0.0017890930 0.0029487610
0.0017967224 0.0028038025
0.0018196106 0.0026760101
0.0018463135 0.0025691986
0.0018653870 0.0024719238
0.0018653870 0.0023784637
0.0018463135 0.0022869110
0.0018043518 0.0022010803
0.0017471313 0.0021324158
0.0016860962 0.0020847321
0.0016174316 0.0020675659
0.0015373230 0.0020847321
0.0014495850 0.0021419525
0.0013504028 0.0022430420
0.0012359619 0.0023937225
0.0010986328 0.0025939941
0.0009384155 0.0028285980
0.0007400513 0.0030765533
0.0004997253 0.0033168793
0.0002212524 0.0035362244
-0.0000801086 0.0037269592
-0.0003776550 0.0038890839
-0.0006599426 0.0040302277
-0.0009155273 0.0041618347
-0.0011291504 0.0042915344
-0.0013008118 0.0044269562
-0.0014343262 0.0045814514
-0.0015258789 0.0047626495
-0.0015792847 0.0049571991
-0.0015945435 0.0051441193
-0.0015640259 0.0052947998
-0.0014839172 0.0053787231
-0.0013656616 0.0053844452
-0.0012168884 0.0053234100
-0.0010604858 0.0052185059
-0.0009117126 0.0050868988
-0.0007858276 0.0049533844
-0.0006980896 0.0048389435
-0.0006446838 0.0047607422
-0.0006332397 0.0047378540
-0.0006599426 0.0047721863
-0.0007133484 0.0048484802
-0.0007858276 0.0049362183
-0.0008697510 0.0049991608
-0.0009498596 0.0050125122
-0.0010070801 0.0049667358
-0.0010414124 0.0048599243
-0.0010452271 0.0047035217
-0.0010147095 0.0045089722
-0.0009498596 0.0042896271
-0.0008506775 0.0040645599
-0.0007324219 0.0038528442
-0.0005989075 0.0036697388
-0.0004463196 0.0035228729
-0.0002861023 0.0034046173
-0.0001220703 0.0032978058
0.0000419617 0.0031909943
0.0001983643 0.0030765533
0.0003433228 0.0029582977
0.0004615784 0.0028400421
0.0005607605 0.0027256012
0.0006370544 0.0026226044
0.0006980896 0.0025367737
0.0007591248 0.0024719238
0.0008201599 0.0024375916
0.0008926392 0.0024356842
0.0009841919 0.0024623871
0.0011024475 0.0025081635
0.0012397766 0.0025596619
0.0013923645 0.0026092529
0.0015640259 0.0026493073
0.0017585754 0.0026855469
0.0019645691 0.0027198792
0.0021896362 0.0027523041
0.0024414062 0.0027904510
0.0027236938 0.0028400421
0.0030479431 0.0029106140
0.0034255981 0.0030097961
0.0038528442 0.0031394958
0.0043106079 0.0032863617
0.0047836304 0.0034294128
0.0052452087 0.0035572052
0.0056838989 0.0036602020
0.0061073303 0.0037403107
0.0065345764 0.0038070679
0.0069808960 0.0038700104
0.0074653625 0.0039424896
0.0080184937 0.0040435791
0.0086822510 0.0041923523
0.0094871521 0.0044097900
0.0104331970 0.0047035217
0.0115127563 0.0050640106
0.0126686096 0.0054702759
0.0138015747 0.0058803558
0.0148200989 0.0062522888
0.0156822205 0.0065650940
0.0164337158 0.0068244934
0.0171394348 0.0070476532
0.0178718567 0.0072612762
0.0187149048 0.0074882507
0.0197334290 0.0077495575
0.0209960938 0.0080623627
0.0225219727 0.0084247589
0.0242614746 0.0088157654
0.0261077881 0.0091819763
0.0279350281 0.0094699860
0.0296821594 0.0096530914
0.0313873291 0.0097351074
0.0331497192 0.0097484589
0.0350685120 0.0097274780
0.0372428894 0.0097064972
0.0397644043 0.0097179413
0.0427284241 0.0097980499
0.0462646484 0.0099868774
0.0504760742 0.0103244781
0.0553474426 0.0108261108
0.0607185364 0.0114765167
0.0662651062 0.0122299194
0.0716018677 0.0130157471
0.0765304565 0.0137939453
0.0811195374 0.0145549774
0.0855827332 0.0152988434
0.0901908875 0.0160388947
0.0952262878 0.0168018341
0.1009902954 0.0176181793
0.1078224182 0.0185356140
0.1160430908 0.0196208954
0.1258239746 0.0209217072
0.1370391846 0.0224399567
0.1491050720 0.0241088867
0.1609916687 0.0257854462
0.1716194153 0.0273208618
0.1803932190 0.0286636353
0.1874084473 0.0298728943
0.1931648254 0.0310649872
0.1982574463 0.0323600769
0.2033195496 0.0338745117
0.2090225220 0.0357112885
0.2160644531 0.0379543304
0.2249908447 0.0406551361
0.2358970642 0.0437736511
0.2481651306 0.0471324921
0.2604255676 0.0504169464
0.2711677551 0.0532894135
0.2796173096 0.0555515289
0.2860336304 0.0572166443
0.2912406921 0.0584316254
0.2962074280 0.0593910217
0.3019866943 0.0603275299
0.3096885681 0.0614986420
0.3204917908 0.0631828308
0.3354682922 0.0656375885
0.3552131653 0.0690212250
0.3793601990 0.0733070374
0.4063072205 0.0782203674
0.4335060120 0.0833053589
0.4585685730 0.0881290436
0.4805488586 0.0925006866
0.5000610352 0.0965042114
0.5184745789 0.1003322601
0.5372657776 0.1041755676
0.5578804016 0.1082191467
0.5817909241 0.1126651764
0.6103820801 0.1177463531
0.6445274353 0.1236495972
0.6838378906 0.1303424835
0.7258224487 0.1374034882
0.7658538818 0.1440200806
0.7990036011 0.1493110657
0.8227386475 0.1528644562
0.8377876282 0.1548805237
0.8466529846 0.1558628082
0.8521537781 0.1563510895
0.8571205139 0.1568603516
0.8644599915 0.1579074860
0.8771781921 0.1600246429
0.8979911804 0.1636962891
0.9282951355 0.1691684723
0.9669723511 0.1762218475
1.0097351074 0.1840534210
1.0498847961 0.1914215088
1.0811538696 0.1971435547
1.1009063721 0.2006721497
1.1105651855 0.2021770477
1.1135559082 0.2021923065
1.1137046814 0.2013301849
1.1149215698 0.2002315521
1.1212348938 0.1995697021
1.1364250183 0.1999721527
1.1630592346 0.2018527985
1.2010726929 0.2051677704
1.2465438843 0.2092113495
1.2917976379 0.2126369476
1.3284645081 0.2139987946
1.3520126343 0.2125473022
1.3628730774 0.2084140778
1.3638534546 0.2021389008
1.3582572937 0.1942996979
1.3499832153 0.1855030060
1.3436126709 0.1764068604
1.3439426422 0.1676826477
1.3551483154 0.1599082947
1.3793201447 0.1533813477
1.4147548676 0.1479358673
1.4551525116 0.1428890228
1.4911499023 0.1372432709
1.5145187378 0.1301193237
1.5221614838 0.1211738586
1.5162391663 0.1105861664
1.5014247894 0.0987625122
1.4828929901 0.0861148834
1.4659290314 0.0730018616
1.4560146332 0.0597419739
1.4586181641 0.0465965271
1.4782123566 0.0337581635
1.5164394379 0.0213241577
1.5702972412 0.0093059540
1.6313762665 -0.0023460388
1.6872844696 -0.0136966705
1.7264442444 -0.0247764587
1.7436294556 -0.0355911255
1.7407264709 -0.0461292267
1.7229652405 -0.0563926697
1.6958055496 -0.0664043427
1.6642837524 -0.0762119293
1.6333112717 -0.0859069824
1.6074991226 -0.0955867767
1.5896883011 -0.1052551270
1.5787429810 -0.1146812439
1.5687851906 -0.1233215332
1.5519981384 -0.1305141449
1.5233988762 -0.1358451843
1.4827227592 -0.1393013000
1.4325537682 -0.1411342621
1.3766236305 -0.1417198181
1.3196377754 -0.1415576935
1.2669215202 -0.1412467957
1.2236602306 -0.1414146423
1.1944497824 -0.1426753998
1.1826974154 -0.1455326080
1.1893368959 -0.1502056122
1.2115007639 -0.1564559937
1.2418363094 -0.1634674072
1.2692521811 -0.1699352264
1.2827808857 -0.1745777130
1.2770172358 -0.1768283844
1.2535712719 -0.1770324707
1.2177336216 -0.1760025024
1.1753127575 -0.1745948792
1.1318023205 -0.1735973358
1.0923538208 -0.1737365723
1.0613374710 -0.1756076813
1.0412769318 -0.1794967651
1.0316610336 -0.1851787567
1.0283646584 -0.1917819977
1.0244774818 -0.1979370117
1.0132818222 -0.2022895813
0.9917221069 -0.2041339874
0.9609737396 -0.2035617828
0.9242553711 -0.2010784149
0.8849945068 -0.1972789764
0.8463068008 -0.1927566528
0.8109674454 -0.1880893707
0.7814197540 -0.1838245392
0.7593708038 -0.1803779602
0.7448959351 -0.1777935028
0.7356348038 -0.1755390167
0.7269353867 -0.1725425720
0.7137689590 -0.1676425934
0.6934537888 -0.1602516174
0.6664333344 -0.1505470276
0.6347579956 -0.1390991211
0.6006698608 -0.1265258789
0.5662727356 -0.1134128571
0.5335798264 -0.1003074646
0.5044670105 -0.0877113342
0.4804306030 -0.0760383606
0.4620761871 -0.0655269623
0.4485893250 -0.0561790466
0.4376888275 -0.0477924347
0.4264869690 -0.0400753021
0.4129924774 -0.0328140259
0.3968944550 -0.0259647369
0.3790454865 -0.0195751190
0.3606262207 -0.0136985779
0.3427639008 -0.0083541870
0.3265171051 -0.0035247803
0.3129100800 0.0008296967
0.3028354645 0.0047760010
0.2968139648 0.0083904266
0.2946491241 0.0117454529
0.2951412201 0.0148849487
0.2961883545 0.0178050995
0.2955684662 0.0204811096
0.2920665741 0.0228977203
0.2858333588 0.0250587463
0.2777366638 0.0269908905
0.2687511444 0.0287265778
0.2598056793 0.0303058624
0.2517871857 0.0317935944
0.2455368042 0.0332832336
0.2417278290 0.0348663330
0.2406044006 0.0365905762
0.2416992188 0.0384197235
0.2437496185 0.0401897430
0.2450256348 0.0416679382
0.2440795898 0.0426845551
0.2403984070 0.0432243347
0.2343368530 0.0434303284
0.2265834808 0.0434894562
0.2177848816 0.0435619354
0.2084827423 0.0437774658
0.1992321014 0.0442466736
0.1906318665 0.0450878143
0.1831359863 0.0463733673
0.1767616272 0.0480728149
0.1709041595 0.0500030518
0.1644058228 0.0518264771
0.1560173035 0.0531921387
0.1450366974 0.0539379120
0.1315021515 0.0541572571
0.1158390045 0.0540771484
0.0985183716 0.0539588928
0.0799751282 0.0540771484
0.0606193542 0.0547180176
0.0408401489 0.0561809540
0.0209827423 0.0587387085
0.0013046265 0.0625820160
-0.0180187225 0.0677299500
-0.0368156433 0.0739707947
-0.0548362732 0.0808334351
-0.0717010498 0.0876064301
-0.0869789124 0.0935840607
-0.1003723145 0.0983943939
-0.1118144989 0.1020889282
-0.1214447021 0.1049671173
-0.1295490265 0.1073875427
-0.1365356445 0.1097202301
-0.1428966522 0.1123256683
-0.1490459442 0.1154479980
-0.1550960541 0.1190738678
-0.1606712341 0.1227931976
-0.1648979187 0.1258163452
-0.1668167114 0.1272926331
-0.1659832001 0.1267662048
-0.1626510620 0.1243438721
-0.1574497223 0.1204357147
-0.1510372162 0.1154975891
-0.1440143585 0.1099624634
-0.1369361877 0.1042423248
-0.1303100586 0.0987262726
-0.1245460510 0.0937385559
-0.1198501587 0.0894451141
-0.1160793304 0.0857582092
-0.1127243042 0.0823268890
-0.1091556549 0.0786991119
-0.1049671173 0.0746021271
-0.1001319885 0.0700550079
-0.0948295593 0.0652256012
-0.0892620087 0.0602951050
-0.0836143494 0.0554237366
-0.0780735016 0.0507583618
-0.0728454590 0.0464439392
-0.0681343079 0.0426082611
-0.0640830994 0.0393276215
-0.0606880188 0.0365772247
-0.0577392578 0.0342006683
-0.0548400879 0.0319328308
-0.0515804291 0.0295009613
-0.0477676392 0.0267677307
-0.0434856415 0.0237655640
-0.0389461517 0.0206108093
-0.0343608856 0.0174293518
-0.0299110413 0.0143299103
-0.0257472992 0.0114040375
-0.0219974518 0.0087261200
-0.0187587738 0.0063552856
-0.0160865784 0.0043296814
-0.0139770508 0.0026626587
-0.0123634338 0.0013465881
-0.0111541748 0.0003662109
-0.0102691650 -0.0003051758
-0.0096683502 -0.0006904602
-0.0093307495 -0.0008163452
-0.0092411041 -0.0007209778
-0.0093917847 -0.0004310608
-0.0097656250 0.0000152588
-0.0103492737 0.0005836487
-0.0111293793 0.0012435913
-0.0120811462 0.0019626617
-0.0131607056 0.0027084351
-0.0142879486 0.0034389496
-0.0153446198 0.0041103363
-0.0162029266 0.0046730042
-0.0167961121 0.0051040649
-0.0171318054 0.0054111481
-0.0172576904 0.0056114197
-0.0172386169 0.0057296753
-0.0171337128 0.0058002472
-0.0170059204 0.0058536530
-0.0169258118 0.0059185028
-0.0169506073 0.0060234070
-0.0171070099 0.0061874390
-0.0173683167 0.0064086914
-0.0176563263 0.0066642761
-0.0178794861 0.0069293976
-0.0179843903 0.0071868896
-0.0179824829 0.0074405670
-0.0179080963 0.0077018738
-0.0178050995 0.0079822540
-0.0177192688 0.0082931519
-0.0176963806 0.0086421967
-0.0177783966 0.0090427399
-0.0180072784 0.0095062256
-0.0184116364 0.0100345612
-0.0189762115 0.0106201172
-0.0196323395 0.0112152100
-0.0202522278 0.0117416382
-0.0207004547 0.0121231079
-0.0209102631 0.0123195648
-0.0209045410 0.0123538971
-0.0207538605 0.0122699738
-0.0205364227 0.0121192932
-0.0203247070 0.0119533539
-0.0201873779 0.0118160248
-0.0201969147 0.0117530823
-0.0204105377 0.0118007660
-0.0208530426 0.0119800568
-0.0214843750 0.0122756958
-0.0221920013 0.0126304626
-0.0228595734 0.0129776001
-0.0234127045 0.0132846832
-0.0238494873 0.0135574341
-0.0242137909 0.0138168335
-0.0245437622 0.0140914917
-0.0248775482 0.0144042969
-0.0252609253 0.0147705078
-0.0257377625 0.0152149200
-0.0263557434 0.0157642365
-0.0271492004 0.0164241791
-0.0280914307 0.0171699524
-0.0290679932 0.0179290771
-0.0298786163 0.0185699463
-0.0303096771 0.0189514160
-0.0302524567 0.0190029144
-0.0297355652 0.0187416077
-0.0288562775 0.0182304382
-0.0277156830 0.0175323486
-0.0264148712 0.0167102814
-0.0250511169 0.0158367157
-0.0237274170 0.0149822235
-0.0225372314 0.0142097473
-0.0215358734 0.0135593414
-0.0207290649 0.0130405426
-0.0200481415 0.0126190186
-0.0193843842 0.0122261047
-0.0186500549 0.0118122101
-0.0178203583 0.0113601685
-0.0169448853 0.0108928680
-0.0160903931 0.0104446411
-0.0153102875 0.0100402832
-0.0146579742 0.0097064972
-0.0141792297 0.0094642639
-0.0139083862 0.0093345642
-0.0138607025 0.0093326569
-0.0140266418 0.0094528198
-0.0143413544 0.0096549988
-0.0146980286 0.0098762512
-0.0149860382 0.0100460052
-0.0151405334 0.0101242065
-0.0151634216 0.0101146698
-0.0150890350 0.0100421906
-0.0149631500 0.0099353790
-0.0148315430 0.0098247528
-0.0147418976 0.0097427368
-0.0147476196 0.0097198486
-0.0148944855 0.0097866058
-0.0152053833 0.0099582672
-0.0156669617 0.0102214813
-0.0162048340 0.0105247498
-0.0167007446 0.0107879639
-0.0170230865 0.0109252930
-0.0170993805 0.0108890533
-0.0169391632 0.0106906891
-0.0165977478 0.0103759766
-0.0161571503 0.0099983215
-0.0156860352 0.0096130371
-0.0152549744 0.0092678070
-0.0149307251 0.0090045929
-0.0147571564 0.0088558197
-0.0147514343 0.0088253021
-0.0148735046 0.0088882446
-0.0150394440 0.0089912415
-0.0151519775 0.0090770721
-0.0151634216 0.0091075897
-0.0150794983 0.0090827942
-0.0149345398 0.0090255737
-0.0147762299 0.0089530945
-0.0146331787 0.0088863373
-0.0145397186 0.0088443756
-0.0145320892 0.0088462830
-0.0146350861 0.0089073181
-0.0148487091 0.0090312958
-0.0151329041 0.0091934204
-0.0154037476 0.0093421936
-0.0155467987 0.0094146729
-0.0154838562 0.0093593597
-0.0152015686 0.0091686249
-0.0147342682 0.0088615417
-0.0141448975 0.0084743500
-0.0134925842 0.0080432892
-0.0128383636 0.0075988770
-0.0122413635 0.0071792603
-0.0117473602 0.0068149567
-0.0113906860 0.0065212250
-0.0111732483 0.0063056946
-0.0110626221 0.0061492920
-0.0109863281 0.0060100555
-0.0108642578 0.0058536530
-0.0106620789 0.0056610107
-0.0103855133 0.0054340363
-0.0100650787 0.0051994324
-0.0097465515 0.0049839020
-0.0094718933 0.0048084259
-0.0092830658 0.0046939850
-0.0092239380 0.0046634674
-0.0093364716 0.0047359467
-0.0096435547 0.0049152374
-0.0101375580 0.0051975250
-0.0107822418 0.0055599213
-0.0114994049 0.0059566498
-0.0121936798 0.0063419342
-0.0128021240 0.0066833496
-0.0133132935 0.0069732666
-0.0137577057 0.0072326660
-0.0141887665 0.0074939728
-0.0146617889 0.0077896118
-0.0152263641 0.0081481934
-0.0159339905 0.0085945129
-0.0168209076 0.0091457367
-0.0178871155 0.0098018646
-0.0190849304 0.0105285645
-0.0203075409 0.0112628937
-0.0214252472 0.0119361877
-0.0223655701 0.0125007629
-0.0231285095 0.0129489899
-0.0237503052 0.0132999420
-0.0242786407 0.0135746002
-0.0247726440 0.0138053894
-0.0253105164 0.0140323639
-0.0259761810 0.0143032074
-0.0268402100 0.0146617889
-0.0279254913 0.0151195526
-0.0291748047 0.0156497955
-0.0304374695 0.0161781311
-0.0315322876 0.0166091919
-0.0323276520 0.0168743134
-0.0328025818 0.0169658661
-0.0330352783 0.0169296265
-0.0331344604 0.0168266296
-0.0332088470 0.0167160034
-0.0333728790 0.0166568756
-0.0337352753 0.0167064667
-0.0343856812 0.0169105530
-0.0353775024 0.0172958374
-0.0366954803 0.0178508759
-0.0382099152 0.0185070038
-0.0396766663 0.0191459656
-0.0408344269 0.0196304321
-0.0415344238 0.0198783875
-0.0417881012 0.0198841095
-0.0416946411 0.0196781158
-0.0413684845 0.0193042755
-0.0409278870 0.0188121796
-0.0405101776 0.0182628632
-0.0402526855 0.0177268982
-0.0402774811 0.0172653198
-0.0406589508 0.0169258118
-0.0413532257 0.0167083740
-0.0421791077 0.0165500641
-0.0428714752 0.0163612366
-0.0432071686 0.0160732269
-0.0431365967 0.0156784058
-0.0427589417 0.0152378082
-0.0422401428 0.0148353577
-0.0417461395 0.0145339966
-0.0414142609 0.0143947601
-0.0413818359 0.0144634247
-0.0417709351 0.0147724152
-0.0426559448 0.0153388977
-0.0440254211 0.0161399841
-0.0457286835 0.0171070099
-0.0474758148 0.0181121826
-0.0489444733 0.0190200806
-0.0499401093 0.0197467804
-0.0504550934 0.0202713013
-0.0505847931 0.0206089020
-0.0504322052 0.0207881927
-0.0501003265 0.0208415985
-0.0497093201 0.0208091736
-0.0493907928 0.0207424164
-0.0492610931 0.0206832886
-0.0493602753 0.0206527710
-0.0495872498 0.0206127167
-0.0496845245 0.0204563141
-0.0493316650 0.0200538635
-0.0483169556 0.0193290710
-0.0466575623 0.0183067322
-0.0445442200 0.0170822144
-0.0422153473 0.0157737732
-0.0399074554 0.0144958496
-0.0378379822 0.0133438110
-0.0362167358 0.0124073029
-0.0352401733 0.0117702484
-0.0350551605 0.0114974976
-0.0357227325 0.0116214752
-0.0371952057 0.0121421814
-0.0393104553 0.0130214691
-0.0418910980 0.0142192841
-0.0448894501 0.0157470703
-0.0484199524 0.0176715851
-0.0526828766 0.0200881958
-0.0578765869 0.0230884552
-0.0641880035 0.0267505646
-0.0717945099 0.0311489105
-0.0808544159 0.0363445282
-0.0914630890 0.0423641205
-0.1035556793 0.0491657257
-0.1167850494 0.0565662384
-0.1304721832 0.0642261505
-0.1437835693 0.0717334747
-0.1560993195 0.0787715912
-0.1672430038 0.0852375031
-0.1773738861 0.0911865234
-0.1867990494 0.0967521667
-0.1959199905 0.1021251678
-0.2052373886 0.1075458527
-0.2153482437 0.1133136749
-0.2268905640 0.1197528839
-0.2403421402 0.1271133423
-0.2556953430 0.1353950500
-0.2721643448 0.1441822052
-0.2881803513 0.1526489258
-0.3020429611 0.1599082947
-0.3129291534 0.1655445099
-0.3212127686 0.1697883606
-0.3279285431 0.1732311249
-0.3342523575 0.1765289307
-0.3413839340 0.1803436279
-0.3505439758 0.1853466034
-0.3628883362 0.1921691895
-0.3792848587 0.2012825012
-0.3999109268 0.2127838135
-0.4238119125 0.2261734009
-0.4487552643 0.2402687073
-0.4718036652 0.2535037994
-0.4906282425 0.2646331787
-0.5045690536 0.2732982635
-0.5144786835 0.2799530029
-0.5218744278 0.2854042053
-0.5284099579 0.2905406952
-0.5358028412 0.2962989807
-0.5458498001 0.3036632538
-0.5602970123 0.3135967255
-0.5804128647 0.3267974854
-0.6062602997 0.3432884216
-0.6360015869 0.3620204926
-0.6659078598 0.3808631897
-0.6918659210 0.3974552155
-0.7116918564 0.4104900360
-0.7258605957 0.4201526642
-0.7362608910 0.4274425507
-0.7449922562 0.4335155487
-0.7540941238 0.4395446777
-0.7656569481 0.4467487335
-0.7818460464 0.4564056396
-0.8045248985 0.4696063995
-0.8343119621 0.4867000580
-0.8694834709 0.5066719055
-0.9056143761 0.5269336700
-0.9369750023 0.5441341400
-0.9593496323 0.5558185577
-0.9718360901 0.5614719391
-0.9761686325 0.5621051788
-0.9751042128 0.5593280792
-0.9715652466 0.5548439026
-0.9685066342 0.5503597260
-0.9689574242 0.5476131439
-0.9758542180 0.5482845306
-0.9913126230 0.5535907745
-1.0153824091 0.5635795593
-1.0449112654 0.5765132904
-1.0736063719 0.5889244080
-1.0945260525 0.5969886780
-1.1037969589 0.5985794067
-1.1018202305 0.5939407349
-1.0913701057 0.5846290588
-1.0757427216 0.5724716187
-1.0583806038 0.5593490601
-1.0429964066 0.5472640991
-1.0334343910 0.5382537842
-1.0329861641 0.5340499878
-1.0431323051 0.5354347229
-1.0622482300 0.5415611267
-1.0852313042 0.5498161316
-1.1051025391 0.5566253662
-1.1163349152 0.5591468811
-1.1172685623 0.5565147400
-1.1096458435 0.5495719910
-1.0967855453 0.5399513245
-1.0824546814 0.5294952393
-1.0704765320 0.5200500488
-1.0644226074 0.5133171082
-1.0672245026 0.5106735229
-1.0806503296 0.5129356384
-1.1043186188 0.5198936462
-1.1344861984 0.5297393799
-1.1640253067 0.5390777588
-1.1852216721 0.5442161560
-1.1940288544 0.5431518555
-1.1913356781 0.5361671448
-1.1805267334 0.5246963501
-1.1651172638 0.5102691650
-1.1482830048 0.4942779541
-1.1333255768 0.4781646729
-1.1238975525 0.4635353088
-1.1233730316 0.4519004822
-1.1334209442 0.4440650940
-1.1525268555 0.4395561218
-1.1753501892 0.4364166260
-1.1938629150 0.4316825867
-1.2007694244 0.4227180481
-1.1930675507 0.4085502625
-1.1723175049 0.3899345398
-1.1421890259 0.3683891296
-1.1065521240 0.3454208374
-1.0690727234 0.3223648071
-1.0333576202 0.3004379272
-1.0029354095 0.2807350159
-0.9805660248 0.2640647888
-0.9668998718 0.2506065369
-0.9593734741 0.2396774292
-0.9523372650 0.2297897339
-0.9393920898 0.2192382812
-0.9168758392 0.2069931030
-0.8851737976 0.1929893494
-0.8471412659 0.1777572632
-0.8062019348 0.1619796753
-0.7655525208 0.1462745667
-0.7280483246 0.1311912537
-0.6962356567 0.1172027588
-0.6721496582 0.1046791077
-0.6567039490 0.0938110352
-0.6489486694 0.0844955444
-0.6456375122 0.0763168335
-0.6417274475 0.0686340332
-0.6323509216 0.0608406067
-0.6152801514 0.0527153015
-0.5914154053 0.0444335938
-0.5631637573 0.0363082886
-0.5330543518 0.0286293030
-0.5033950806 0.0215797424

